Parallel Network Flow Allocation in Repeated Routing Games via LQR Optimal Control

In this article, we study the repeated routing game problem on a parallel network with affine latency functions on each edge. We cast the game setup in a LQR control theoretic framework, leveraging the Rosenthal potential formulation. We use control techniques to analyze the convergence of the game dynamics with specific cases that lend themselves to optimal control. We design proper dynamics parameters so that the conservation of flow is guaranteed. We provide an algorithmic solution for the general optimal control setup using a multiparametric quadratic programming approach (explicit MPC). Finally we illustrate with numerics the impact of varying system parameters on the solutions.

==> new_main.tex <==




%%%%--------------


\usepackage{graphicx}
\usepackage{tikz}
\usepackage{bbm}
\usepackage[ruled, linesnumbered]{algorithm2e}
\SetAlCapNameFnt{\scriptsize}
\SetAlCapFnt{\footnotesize}
\usepackage[fleqn]{amsmath}
\usepackage{algpseudocode}
\usepackage{float}
\usepackage{setspace}
\usepackage[T1]{fontenc}
%\usepackage{subfig}



\usepackage[colorlinks=true,linkcolor=blue,citecolor=blue]{hyperref}
% For TRB version hide links
\usepackage{amsthm,amsmath,amssymb}
\usepackage{mathtools}
\usepackage{cleveref}
%\usepackage[hidelinks]{hyperref}
\usepackage[font=small,labelfont=bf]{caption}
\usepackage{subcaption}

% Theorems and etc.
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}

\usepackage{amsthm}
\usepackage[pagewise]{lineno}
\linenumbers

\let\oldequation\equation
\let\oldendequation\endequation

\renewenvironment{equation}
  {\linenomathNonumbers\oldequation}
  {\oldendequation\endlinenomath}


% Comments Section----------------------------------------
\newcount\Comments  % 1 suppresses notes to selves in text
\Comments=0  % TODO: set to 1 for final version
\newcommand{\kibitz}[2]{\ifnum\Comments=0\textcolor{#1}{#2}\fi}
% \newcommand{\Fangyu}[1]{\kibitz{PineGreen} {[Fangyu: #1]}}
\newcommand{\todoM}[1]{\todo[inline,color=blue!30!white]{\textbf{Marsalis:} #1}}
\newcommand{\todoY}[1]{\todo[inline,color=green!30!white]{\textbf{Yiling:} #1}}
%---------------------------------------------------------
\newcommand{\colorbegin}{\color{black!50!blue}}
\newcommand{\colorproof}{\color{black!80!red}}
% \newcommand{\colorbegin}{\color{black}}
% \newcommand{\colorproof}{\color{black}}
\newcommand{\colorend}{\color{black}}

\newtheorem{principle}{Principle}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{property}{Property}[section]
\newtheorem{notation}{Notation}[section]
\newtheorem*{theorem*}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}{Lemma}[section]
\newtheorem*{conjecture*}{Conjecture}
\newtheorem{assumption}{Assumption}
\numberwithin{equation}{section}
\theoremstyle{remark}
\newtheorem{example}{Example}[section]

\input{macros.tex}

% Put here what will go to headers as author
\AuthorHeaders{Gibson, You, and Bayen}
\title{Parallel Network Flow Allocation in Repeated Routing Games via LQR Optimal Control}
% Change as needed

\author{%
%   \textbf{Author}\\
%   email\\
%   \hfill\break% this is a way to add line numbering on empty line
  \textbf{Marsalis Gibson*}\\
  University of California, Berkeley\\
  652 Sutardja Dai Hall, Berkeley, CA 94720-1710\\
  email: mtgibson@berkeley.edu\\
  \hfill\break
  \textbf{Yiling You*}\\
  University of California, Berkeley\\
  652 Sutardja Dai Hall, Berkeley, CA 94720-1710\\
  email: yiling.you@berkeley.edu \\
  \hfill\break
  \textbf{Alexandre M. Bayen}\\
  University of California, Berkeley\\
  Institute of Transportation Studies\\
  109 McLaughlin Hall, Berkeley CA 94720-1720\\
  email: bayen@berkeley.edu \\
  \hfill\break
}

% If necessary modify the number of words per table or figure default is set to
% 250 words per table and figure
\setcounter{wordspertable}{250}
\setcounter{wordsperfigure}{0}

% If words are counted manually, put that number here. This does not include
% figures and tables. This can also be used to avoid problems with texcount
% program i.e. if one does not have it installed.
\setcounter{textwords}{6677}
%\setcounter{figure}{6}
\setcounter{table}{2}

\usepackage{todonotes}

\begin{document}

\maketitle


\section{Abstract}

In this article, we study the repeated routing game problem on a parallel network with affine latency functions on each edge. We cast the game setup in a LQR control theoretic framework, leveraging the Rosenthal potential formulation. We use control techniques to analyze the convergence of the game dynamics with specific cases that lend themselves to optimal control. We design proper dynamics parameters so that the conservation of flow is guaranteed. We provide an algorithmic solution for the general optimal control setup using a multiparametric quadratic programming approach (explicit MPC). Finally we illustrate with numerics the impact of varying system parameters on the solutions.


% This article applies the existing Markovian traffic assignment framework to novel traffic control strategies.
% In the Markovian traffic assignment framework, transition matrices are used to derive the traffic flow allocation.
% In contrast to the static traffic assignment, the framework only requires flow split ratio at every intersection, bypassing the need of computing path flow allocation.
% %More specifically, the Markovian framework only involves the flow split ratio at every intersection.
% %This leads to an important advantage of the Markovian framework.
% Consequently, compared to static traffic assignment, drivers' routing behaviors can be modeled with fewer variables.
% %fewer variables are required to understand drivers' routing behaviors.
% As a result, it could be used to improve the efficiency of traffic management, especially in large scale applications.
% To begin with, the article introduces Markovian traffic assignment and connects it to the classic static traffic assignment.
% Then, the framework is extended to dynamic traffic assignment using microscopic traffic simulator \textit{Simulation of Urban Mobility} (SUMO).
% %Applying Markovian framework to a benchmark network, optimal routing behaviors are learned using three different reward functions (network outflow, total vehicle hours of travel, and average marginal regret).
% In a case study, the framework is applied to a standard benchmark network, where optimal routing behaviors are independently learned through grid search, random search, and evolution strategies, under three different reward functions (network outflow, total vehicle hours of travel, and average marginal regret).
% % The benchmark network upholds the relevance of learning the optimal flow split ratios instead of learning the optimal path flow allocation, as Markov chain theory supports the ability to scale up to larger networks.
% The case study shows that the this novel traffic control strategy is promising, as Markov chain theory supports the ability to scale up to larger networks.
% % and suggests ways to extend it to large scale traffic scenarios.

\hfill\break%
\noindent\textit{Keywords}: Repeated routing game, Algorithmic Game Theory, Nash Equilibrium, Linear-quadratic Regulator, Multiparametric quadratic programming, Explicit MPC %Network equilibrium modeling, Routing behavior, Nash games, Markov chains

\newpage

\section{Introduction}
%\item General paragraph about routing in transportation (10 lines), Dijkstra, navigational apps etc. Based on all of this, Google, Waze, etc. act as flow allocation mechanisms. 
%-----------
The routing problem -- a problem in which trip-makers route traffic between an origin and destination -- is a central and essential component in the study of urban transportation planning. Emerging as an enabler to this problem over the last decade, navigational apps have used solution from the routing problem to provide shortest paths from origin to destination, or identify the paths with the shortest travel time \cite{Cabannes2018TheIO}. Due to ubiquitous adoption of navigational apps by motorists (commuters, travelers), TNCs (Lyft/Uber), delivery fleets \cite{hwang2015urban}, and many others, these apps are playing even bigger roles in transportation and the significance of their roles are growing \cite{alonso2017demand}. With increased penetration routing app users, navigational apps are starting to "act" as flow allocation mechanisms -- having positive effects on some cities travels and negative on others when users use local neighborhood routes to avoid traffic \cite{thai2016negative}. Thus, it is becoming ever for important to understand the routing game problem, its solutions, and how flow allocation mechanisms (and traffic assignment) are being used in transportation. %\textbf{[cite policy brief] not sure how to cite it}.

The traffic assignment problem is a model framework for aggregated flows of motorists routed through a network from their origins to their destinations. To address the traffic assignment problem, this process has initially been modeled in a static way using notions such as static traffic assignment, for which specific solutions exist like User equilibrium and system optimal \cite{boyles2010traffic} \cite{patriksson2015traffic}. In this static model, we assume the network being studied is close to "steady state", and that the current network capacity is the capacity over the entire analysis period. However, in hopes to move away from this assumption and better model traffic in urban areas, researchers have moved toward dynamic traffic assignment models, which aim to
model time-varying networks and demand interactions and changes \cite{chiu2011dynamic} \cite{shafiei2018calibration} \cite{mahmassani2001dynamic} \cite{boyles2010traffic}. Additionally, within the field of traffic control, researchers have used simulation based approaches \cite{osorio2010simulation} and some are starting to use big data to further analyze travel behavior  \cite{chen2016promises}. 

The traffic assignment problem has been modeled using game theory among many other techniques. Specifically, it has been posed in a game theoretic framework called routing game. A routing game is a game in which the players (non-cooperatively) route traffic between an origin and a destination of a proposed network, where the network models a system of roads. After each player chooses routing strategies, each player will incur a cost on the route they choose \cite{Nisam2007}. One specific kind of game is called "the one-shot" game. The one-shot routing game is a static game\footnote{A static game is played only once with one iteration.}, where the players make their decision simultaneously and therefore no time history is involved. Within the one-shot game framework, multiple equilibrium models and the corresponding equilibria have played an important role in understanding the inefficiencies of networks (e.g. the price of anarchy \cite{10.1145/506147.506153}), for example the user equilibrium or Nash equilibrium \cite{patriksson}. Properties and the characterizations of the equilibrium solutions are also well-studied, for example, the Nash equilibria are known to be the solution set of the convex Rosenthal potential function \cite{Rosenthal1973ACO}. 

Within routing games, one can also study a dynamic game, where the environment is time varying. The analysis of such games is more difficult from a theoretic standpoint: the notion of dynamic equilibria has to be introduced, and extra ingredients like information acquisition and time ordering of the execution of the actions need to be specified \cite{doi:10.1137/1.9781611971132}. Therefore, moving towards more dynamical games, we consider repeated games, i.e. a static game iterated over time, as a model of the evolution of the traffic situation. The iteration here can be naturally interpreted as time discretization (e.g. sometimes where traffic conditions are steady over time intervals). In the case of the present work, we follow previous approaches in which the repeated nature of the game encompasses the process of a routing entity (Google, Waze, etc) to learn from day to day from their previous performances. Oftentimes (and it is the case in our formulation), the repeated version is essentially the sequential appreciation of a static game. A natural question to study is the behavior of the dynamics, when the players repeat a static game using past information. Dynamics in a repeated routing game might not converge, and even if it does, convergence might not be quantifiable (e.g. convergence almost everywhere, convergence in the sense of Cesaro means or of the time-averages, etc.). Even when the dynamics sequence converges itself, the equilibria to which it converges to (Nash equilibrium or social optimum) might not be unique \cite{7479108}. Approaching this question, Krichene et al. estimates the learning dynamics within an online learning model of player dynamics \cite{krichene2018tcps} and studies the traffic dynamics under partial control \cite{7604118}. 

To better understand the routing game in these systems and provide bigger impacts in transportation, we might also want to leverage concepts from other areas of engineering. Modeling and analysis of conflict, the study of systems, and the study of their equilibria are not unique to the routing game. In fact, very similar concepts and analysis shows up in control theory, which oftentimes, similarly to game theory, models interactions between a system of controllers (the "decision-makers") and their environment \cite{recht2019tour}. Unsurprisingly, many influences within game theory show up in many areas of controls (differential games, teams games, and distributed control) \cite{marden2018game}, and many connections can be made between the two. Even though there exists many similarities and influences between game theory and controls, there are many useful control design techniques that exists separate from game theory \cite{goodwin2001control} \cite{alessio2009survey} \cite{bansal2017hamilton}, but are conceptually similar/applicable to designing decision-makers within routing games, especially for routing systems like google. 

Therefore, in this article, contribute to the literature of routing games and draw from other areas of engineering to making deeper connections and make use of control techniques for routing. We specifically introduce a new game design framework for routing games using the linear-quadratic regulator (LQR).


%\item Leverage: huge literature on game theory. Paragraph on game \textbf{theory} Basar book, repeated games (2-3 references), etc. 



%``Because of all of this'' we do the following


%\item This is what was done before (mostly us + other references). Paragraph on prior work: Prior work in routing (Jerome Thai, Theo /Marco (TRB))

%-----
\subsection{Key Contributions}
The present article focuses on transforming the repeated game problem into a control theoretic problem, and studying the  convergence of the game dynamics in this framework. The key contributions of the article include the following:
\begin{itemize}
    \item We provide a  game design scheme for repeated routing games through the Linear Quadratic Regulator (LQR).
    \item We design control dynamics with specific choices of system parameters to respect the conservation of flow and achieve specific convergence results.
    \item We provide a method for producing piecewise affine optimal routing strategies using explicit model predictive control (MPC) techniques.
    \item We derive new theoretical results for specific cases of the new design scheme. 
    \item We illustrate a geometric framework for visualizing optimal routing solutions for every feasible state in the routing game.
    \item We extend the comparison literature between game theory and controls.
\end{itemize}
\subsection{Organization of the article} 
This article, first, explains the new control theoretic game design scheme in \textit{\nameref{Sec:LQR_Scheme_Sec}}, under  which we also build up the intuition and understanding of the framework by illustrating an evolution of the game from a one-shot framing (see \textit{\nameref{Subsec:One-shot}}) to a repeated game framing (see \textit{\nameref{Subsec:Repeated}}), and finally to the new control framing (see \textit{\nameref{Subsec:LQR}}). We further present analogies between the new framework and a classical algorithmic game theory model of routing games within this section (see \textit{\nameref{Subsec:LQR}}); then, we finally talk about how to design the game (see \textit{\nameref{Subsubsec:GameDesign}}) and its interpretation (see \textit{\nameref{Subsubsec:Interp}}). Next, we run through the system analysis and its properties in \textit{\nameref{Sec:SysAnalysis}}, where we additionally describe a few requirements for the system. In \textit{\nameref{Sec:MPC}}, we describe a algorithmic approach to solve the control routing problem using explicit MPC techniques. Finally, in \textit{\nameref{Sec:Results}} we run through a few numerical simulations and present its results with associated discussions. 




\newpage




%------------------------
% A routing game is a game in which players non-cooperatively route traffic between two points of a game network -- origin point $\origin$ and destination point $\destination$, where the network models a system of roads between various origins and destinations. After each player chooses routing strategies, each player will incur a cost on the route they choose \cite{Nisam2007}. This game arises from the context of game theory, which hopes to "study mathematical models of conflict and cooperation between rational decision-makers" (\textbf{REF}). Under game theory, research have used the routing game to study a variety of problems \textbf{(cite)}, and within routing games, researchers have designed "decision-makers" and have studied system equilibria, along with its convergence properties. The time-varying network and demand interaction is also studied in the Dynamic Traffic Assignment (DTA) literature, where behavioral sound models are built to facilitate real-time traffic planning, as well as analysis of the accuracy and fidelity of the the model results (see \cite{Chiu2011DynamicTA}). Furthermore, in recent years, researchers in game theory have also began to develop algorithms for new technologies like google maps that wish to control flows of traffic.
% \begin{itemize}
%     \item Work of Walid, Tim Roughgarden, Patricksson (UE), Jerome Thai, Theo /Marco (TRB)
% \end{itemize}


% Contributions of the article
%\subsubsection{Key contributions}
%The key contributions of the article include:
%\begin{itemize}
%     \item We provide a full fledged game design scheme for repeated routing games through LQR.
%     \item We design control dynamics with specific choice of system parameters to respect the conservation of flow and achieve specific convergence results.
%     \item We provide a numerical method for producing piecewise affine optimal routing strategies using explicit model predictive control (MPC) techniques.
%     \item We derived new theoretical results for a few cases of the new design scheme. 
%     \item We illustrate a geometric framework for visualizing all optimal routing solutions for every feasible state in the routing game.
%     \item We extend the comparison literature between game theory and controls and are amongst the first to have done routing game design from a control theoretic perspective.
% \end{itemize}

% \subsubsection{Organization of the Paper}
% This article, first, explains the new control theoretic game design scheme in \textit{\nameref{Sec:LQR_Scheme_Sec}}. Under  \textit{\nameref{Sec:LQR_Scheme_Sec}} we build up the intuition and understanding of the framework by illustrating an evolution of the game from a one-shot framing (see \textit{\nameref{Subsec:One-shot}}) to a repeated game framing (see \textit{\nameref{Subsec:Repeated}}), and finally to the new control framing (see \textit{\nameref{Subsec:LQR}}). We further present analogies between the new framework and a classical algorithmic game theory model of routing games within this section (see \textit{\nameref{Subsec:LQR}}); then finally talk about how to design the game (see \textit{\nameref{Subsubsec:GameDesign}}) and its interpretation (see \textit{\nameref{Subsubsec:Interp}}). Next, we run through the system analysis and its properties in \textit{\nameref{Sec:SysAnalysis}}, where we additionally describe a few requirements for the system. In \textit{\nameref{Sec:MPC}}, we describe a algorithmic approach to solve the control routing problem using explicit MPC techniques. Finally, in \textit{\nameref{Sec:Results}} we run through a few numerical simulations and present its results with associated discussions. 

\section{Preliminary}

\begin{table}[h]
\footnotesize
\begin{tabular}{|p{1.7cm}||p{6.7cm}|p{6.3cm}|}
\hline
  \textbf{Notation}
  & \textbf{Description} 
  & \textbf{Type}\\
  \hline % Set of edges in network notation
  
  $\network = (\vertexset, \edgeset)$ &A parallel network for the routing game made of a set of edges $\edgeset$ (as roads) and a set of vertices $\vertexset$ (one origin and one destination)&A directed graph\\
  \hline
  $\edgeelem \in \edgeset$&An edge in the edge set&An element of $\edgeset$\\
  \hline
  $\latfunc(\cdot)$&Affine latency function on edge $\edgeelem$
  &$\edgeflowset \mapsto \costset: \latfunc(\edgeflow) = a_e \edgeflow +b_e, a_e, b_e \geq 0$\\
  \hline % latency function for each edge flow
  
  $\numedges$&   Number of parallel edges 
  &$\mathbb{N}$ \\
  \hline % number of parallel edges 
  
  
  $T$&   Time horizon (total number of rounds in game)
  & $\mathbb{N}$ (discrete time)\\
  \hline % number of parallel edges 
  $\flowset$&Probability Simplex
  & $\flowset:=\{ \flow: \sum_{\edgeelem \in \edgeset} \edgeflow = 1, \edgeflow \geq 0 \}$ \\
  \hline %Probability Simplex, Constraints on the flow
 $\flow$
  &Flow allocation vector on the network
  &  $\flowset, \flow = \left(\edgeflow\right)_{\edgeelem \in \edgeset}$\\
  \hline % flow allocation vector
  $\loss$
  & Latency vector incurred on the network
  & $\lossvectorset,\loss = \left(\latfunc(\edgeflow)\right)_{\edgeelem \in \edgeset}$ \\
  \hline 
  $\stateiter$&System state vector at time $t$
  & $\flowset, \stateiter = (x_{1}^{\timesym},\dots, x_{\numedges}^{\timesym})^\top$\\
  \hline % system state vector, f_t
  $\controliter$
  &System input vector at time $t$
  & $\flowset,
\controliter = (u_{1}^\timesym,\dots, u_{\numedges}^{\timesym})^\top$\\
  \hline % system input vector, u_t
  $\state\optimal$&Steady state of the system&$\flowset$\\
  \hline
  $\initstate$&Initial state of the system&$\flowset$\\
  \hline
  $Q_f$
  &Terminal cost matrix
  & $\mathbb{R}^{\numedges\times \numedges}$ positive semi-definite\\
  \hline % terminal cost matrix, Q_f
  $R$
  &Running cost matrix for inputs
  & $\mathbb{R}^{\numedges\times \numedges}$ positive semi-definite\\
  \hline % input cost matrix, R
  $Q$
  &Running cost matrix for states
  & $\mathbb{R}^{\numedges\times \numedges}$ positive semi-definite\\
  \hline % intermediate state cost matrix, Q
  $\gamma$
  & Weight parameter in the dynamics
  & $\gamma \in [0,1]$\\
  \hline % gamma
  $A$
  & Mapping from the memory to decision
  & $\mathbb{R}^{\numedges\times \numedges}$ left stochastic matrix\\
  \hline % A matrix
  $B$
  & Mapping from suggested routing to decision
  & $\mathbb{R}^{\numedges\times \numedges}$ left stochastic matrix\\
  \hline
\end{tabular}
\end{table}
% Definitions and notation
% \begin{itemize}
%     \item Notation
%     \begin{itemize}
%         \item G, r, c
%         \item f, P
%         \item V, E
%         \item $n_e$
%     \end{itemize}
%     \item non-atomic routing game
%     \item routing network definition and notation
%     \item latency function definition and notation
%     \item Nash equilibrium: (general definition) stable state of the system in which....
%     \item Rosenthal potential function
%     \item LQR
%     \item Ricatti equation
%     \item 
% \end{itemize}

\section{LQR Repeated Game Framework for Routing in Parallel Networks}
\label{Sec:LQR_Scheme_Sec}
We consider a specific routing game design problem where the routing game is posed with a parallel network, $\network$. $\network$ is modeled as a directed graph $\network = (\vertexset, \edgeset)$, where $\vertexset$ is a set containing two nodes (an origin $\origin$ and a destination $\destination$), and $\edgeset$ is an edge set containing $\numedges$ edges between each vertex.

\subsection{One-shot Game Framework}
\label{Subsec:One-shot}
We start by introducing the flow allocation problem, which we will use later as a potential equilibrium point for our repeated game. We will also refer to it as a one-shot game (i.e. a repeated game converging in one iteration).

\begin{definition}[Edge flows]
For each edge $\edgeelem \in \edgeset$, the edge flow, $\edgeflow \in \edgeflowset$, represents a large collection of non-atomic drivers using edge $\edgeelem$ on the network. Each edge flow, $\edgeflow$, represents a portion of traffic in the game (and thus has "mass"), while individual drivers themselves do not. They are negligible with respect to the total number of drivers present (i.e. the non-atomic framework). 
\label{Edge flows} 
\end{definition}

In the flow allocation problem, all drivers are allocated along the network's edges, and each allocation incurs a latency (i.e., loss), $\loss$ (this latency is usually labeled as the average travel time each driver took). Each edge's latency $\loss$ is modeled in the present work as an affine function associated with each edge.

\begin{definition}[Latency function] \label{Latency function} Each edge $\edgeelem \in \edgeset$ has an affine latency function $\latfunc(\cdot): \edgeflowset \mapsto \costset, \latfunc(\edgeflow) = a_e \edgeflow +b_e, a_e, b_e \geq 0$ that converts the edge flow $\edgeflow$ into the edge latency. The latency functions are nonnegative, nondecreasing and Lipschitz-continuous functions.
\label{def:latencyrepeated}
\end{definition}

Normally, in the allocation problem, drivers at the origin, $\origin$, are allocated strategically to reduce the total travel time the system will incur. The resulting allocation for all of the drivers of total mass $1$ in $\network$, is represented as a stochastic vector $\flow =  \left(\edgeflow\right)_{\edgeelem \in \edgeset} \in \flowvectorset$, where each $\edgeflow$ tells us the proportion of flow being allocated on edge $\edgeelem$. Specifically, 
\begin{linenomath*}
\begin{align}
    \flow \in \flowset\text{, where } \flowset := \{ \flow: \sum_{\edgeelem \in \edgeset} \edgeflow = 1, \edgeflow \geq 0 \} 
\end{align}
\end{linenomath*}


\subsubsection{Nash Equilibrium}
% Therefore, we can discuss the Nash equilibrium in the same way we do in game theory. 
If we assume that all drivers act rationally and has access to perfect information, we can describe an equilibrium of the game, known as the \textit{\textbf{Nash equilibrium}}.

\begin{definition}[Nash equilibrium]\label{defi:nashrepeated}
A flow allocation $\flow \in \flowset$ is a Nash equilibrium (user equilibrium \cite{patriksson}, non-atomic equilibrium flow \cite{Nisam2007}, or Wardrop equilibrium \cite{Wardrop1952}) if and only if:
\begin{linenomath*}
\begin{equation}
    \forall \edgeelem \in \edgeset \text{ such that }\edgeflow > 0, ~~\latfunc(\edgeflow) =\min_{\otheredge \in \edgeset} \otheredgelatfunc(\otheredgeflow).
\end{equation}
\end{linenomath*}
\end{definition}



\subsection{Repeated Game Framework}
\label{Subsec:Repeated}
\label{section:RepeatedGames}
% References:
% \begin{itemize}
%     \item http://timroughgarden.org/papers/cacm.pdf
%     \item Loads of Walid's work
%     \item [Cesa-Bianchi and Lugosi 2006]: Nicolo Cesa-Bianchi and G ` abor Lugosi. 2006. ´ Prediction, learning, and games. Cambridge University Press.
%     \item citation for recent years part of this section -- [Freund and Schapire 1999; Hart and Mas-Colell 2001; Hart 2005; Fox and Shamma 2013; Marden et al. 2013; Arslan and Shamma 2004]
%      \item citation for specific study on routing games -- [Fischer and Vocking 2004; Blum et al. 2006; Kleinberg et al. 2009; Krichene et al. 2015a; Krichene et al. 2015b]
% \end{itemize}
In order to encompass time-varying changes in the system, one can use "repeated play" or learning models \cite{cesa2006prediction}. In this framework, a flow allocator (i.e. Gooogle maps) makes a decision iteratively, as opposed to one time in the one-shot game, and uses the outcome of each iteration to adjust their next decision. Adding a $\timesym$ dependency for time to the aforementioned notation, $\flowiter \in \flowset$ becomes the flow allocation at time $\timesym$, $\lossiter \in \lossvectorset$ becomes a vector of latencies produced from functions $\latfunc(\cdot)$ at time $\timesym$, and throughout the game, the flow allocator iteratively chooses $\flowiter$ and then observes $\lossiter$. In this framework, designing learning models of player decisions and whether the resulting dynamics asymptotically converges to equilibrium is one of the objectives of our article. Furthermore, we are also interested in situations in which convergence happens in one shot. Previous research has been done to characterize classes of learning algorithms that converge to different sets of equilibria \cite{blum2006routing} \cite{marden2018game} \cite{hart2001general}. Specifically, different models of learning algorithms and their associated convergence guarantees has been studied for the routing game \cite{krichene2018tcps}, \cite{7604118}, \cite{krichene2015congestion}. 



%%%%%%
%%%%%%
% % Notes from Alex is below
% Flow allocation (expand a bit on $x_{t+1}=f_t(x_t,u_t)$ where $u_t$ is the flow allocation per  $\Delta = \{ u \in \mathbb{R}^{n_e}: \sum_{i \in \mathcal{E}} u_i = 1 , u_i \geq 0\} $

% % This below would probably belong to the part about game allocation process at each step. 
% Thus, the set of actions, $u \in \mathcal{R}^{n_e}$, that the player can take will be represented as a vector of flow proportions. This set is mathematically defined over a probability simplex, $\Delta = \{ u \in \mathbb{R}^{n_e}: \sum_{i \in \mathcal{E}} u_i = 1 , u_i \geq 0\} $. 

%%%%%%%
%%%%%%%
\subsection{LQR Framework}
\label{Subsec:LQR}
The following table sets the framework for the proposed work. The right column defines the repeated game framework previously described (using example designs from previous work \cite{NIPS2015_5843}), while the left column defines the classical control framework used later for LQR control. Both frameworks present obvious mathematical analogies \cite{marden2018game} \cite{marden2015game}.\\


\begin{table}[h]
\footnotesize

\begin{tabular}{|p{2.9cm}||p{6.1cm}|p{6.1cm}|}
 \hline
 &\textbf{Control problem} &  \textbf{Repeated game (online learning)}\\
 \hline
 Notation   & $\stateiter$ state, $\controliter$ control at time $\timesym$ & $\flowiter$ flow allocation, $\lossiter$ loss at time $\timesym$\\
  \hline
 Entities involved &\begin{itemize}
     \item Central decision maker: flow allocator
    \item Players: drivers
\end{itemize}& 
\begin{itemize}
    \item Central decision maker: flow allocator
    \item Players: flow allocator
\end{itemize}\\
\hline
 Design   & $\controliter(\cdot)$  s.t. $\stateiterplus = \ctrldyn(\stateiter,\controliter)$ is stable,  where $\ctrldyn(\cdot, \cdot)$ is the recurrence relation defining the dynamics.    &$\flowdyn(\cdot,\cdot)$ s.t. $\flowiterplus = \flowdyn(\flowiter,\lossiter)$ defines the dynamics for the routing game.\\
  \hline
  Example designs &$\controliter(\stateiter) = K\stateiter$ and $g(\stateiter,\controliter) = A\stateiter + B\controliter\implies \stateiterplus = (A+BK)\stateiter$, where $(A, B)$ is stabilizable, and $A+BK$ is asymptotically stable.& $\flowdyn(\flowiter,\lossiter) = \mathrm{argmin}\limits_{\flowstoch \in \flowset} l_t^\top( \flowstoch - \flowiter)+\frac{1}{\eta_t}D_{\Psi}(\flowstoch, \flowiter)$, where $\eta_t$ is the learning rate at time \timesym, $D_{\Psi}(\cdot, \cdot)$ is the Bregman
divergence induced by a strongly
convex function $\Psi$ defined as $D_{\Psi}(x, y) = \Psi(x)-\Psi(y)-\nabla\Psi(y)^\top(x-y)$. This is called the \textbf{mirror descent algorithm} with Bregman divergence $D_{\Psi}$.\\
  \hline
 Objective function (to minimize)&Cumulative cost, $\sum_{t = 0}^{T-1} \costfunciter(\stateiter,\controliter) + \costfunciterT(\state_T) $&Cumulative regret, $\sum_{t = 0}^{T} \flowcostfunciter(\flowiter, \lossiter) - \min_{\flowstoch \in \flowset}\sum_{t = 0}^{T} \flowcostfunciter(\flowstoch, \lossiter)$\\
\hline
Example objective functions &$\costfunciter(\stateiter,\controliter) = \stateiter^\top Q \stateiter + \controliter^\top R \controliter$, 
$\costfunciterT(\stateiter) = \stateiter^\top Q_f \stateiter$, 
$Q,Q_f\succeq0,R\succ0$
& $\flowcostfunciter(\flowiter,\lossiter) = \flowiter^\top \lossiter$ \\
\hline
\end{tabular}
\end{table}

% \color{red}
% Make a table: Comparing repeated games to control
% (1) Objective function = regret function --> what people who are designing these are algorithms are trying to do \\
% (2) The feedback controller can be compared to the learning algorithm in the repeated game \\
% (3) Observations in repeated games is latency; observation of the control system is the flow distribution occurring on the network --> Latency can be calculated separately, but the cost function is not the latency itself. \\
% (Ex. u(t) = Kx(t) --> Update on decision \\
% Say u(t) is the flow distribution given by each player. \\
% --> Repeated games: u(t) = u(t-1)*$e^{(-\eta)*f_i(x(t))}$ for the decision-maker. \\
% --> Controls: u(t) = Kx(t) is the update law for the decision-maker.\\
% \color{black}
We re-frame the routing problem under the repeated game framework into the LQR framework and solve for/analyze player strategies using existing control techniques. We will essentially aim to do the same game theoretical analysis within linear/nonlinear controls. In the right column of the table, we list the setup under the repeated game framework. The goal of the routing problem there is to design algorithms that dictate strategies for players (the flow allocator). At each time step $\timesym$, the algorithm updates the flow allocation $\flowiterplus$ based on the players' memory $\flowiter$ and the loss on the edge $\lossiter$ induced by the traffic \cite{krichene2015congestion} \cite{7604118} \cite{pmlr-v37-krichene15} \cite{roughgarden2010algorithmic}. The goal is to guarantee a sub-linear regret and a convergence to the set
of Nash equilibria.\\

We start from the repeated games setup, and cast the repeated game problem in a control theoretic framework. We keep the authoritative central decision maker $\control$ as the flow allocator, but we differentiate between the "player" and the "decision-maker" as coined in the original game theoretic setup. Here, the "players" will refer to the drivers in the network flow being routed. In our framework, the "players" do not play; they are only considered by the routing system and the model. The central decision maker is what we want to design in this framework. It has full access to the flow allocation $\state$ on the network, and aims to achieve a certain routing goal (e.g., steer the network flow to a target flow distribution, or minimize the average travel time). The central decision maker embeds the routing goal in the cumulative cost function $\sum_{t = 0}^{T-1} \costfunciter(\stateiter,\controliter) + \costfunciterT(\state_T)$. The players now update their routing decision $\stateiterplus$ by leveraging their memory $\stateiter$ and the central decision maker's suggested routing distribution $\controliter$ at each time step. The target flow allocations $\state\optimal$ are characterized as the steady states of the controlled system, and the central decision maker chooses the optimal controls $\{\controliter\}$  to minimize the cumulative cost function and stabilizes the system to its steady states.\\

The choice of LQR is motivated by the observation that a potential game with affine latency and a parallel network can be naturally framed as a \textbf{quadratic} cost and \textbf{linear} dynamic problem, leveraging the convex formulation of the Rosenthal potential:
\begin{linenomath*}
\begin{align}
    \label{sys:lqr}
    &\underset{\controliter, t = 0, \dots, T-1}{\text{minimize}}  &\sum_{t = 0}^{T-1} \left(\stateiter^\top Q \stateiter + \controliter^\top R \controliter\right)
    &+ \state_T^\top Q_f\state_T \\
    &\text{subject to}&
    \stateiterplus &= A\stateiter + B\controliter, t = 0, 1, \dots, T-1\\
    &&\initstate &= \state(0)
\end{align}
\end{linenomath*}
    where $\stateiter \in \statevectorset$ is the state of the system at time $\timesym$ and $\controliter \in \controlvectorset$ is the action of the decision-maker at time $\timesym$, with appropriate matrices $A, B, Q, R, Q_f$. 
Within this framework, we can leverage known optimal control techniques to formulate optimal strategies and inherent known properties for the system. Furthermore, definition \eqref{defi:nashrepeated} for the context here becomes:

\subsubsection{Nash Equilibrium}
\begin{definition}[Nash equilibrium]\label{defi:nash_ctrls}
A state of the system $\state \in \flowset$ is a Nash equilibrium if and only if:
\begin{linenomath*}
\begin{equation}
    \forall \edgeelem \in \edgeset \text{ such that }\edgestate > 0, ~~\latfunc(\edgestate) =\min_{\otheredge \in \edgeset} \otheredgestatelatfunc(\otheredgestate).
\end{equation}
\end{linenomath*}
\end{definition}

We reiterate the key differences between the repeated game framework and our control theoretic framework:

\begin{enumerate}
    % \item In repeated games, the entities involved are the non-atomic players (a flow allocator). In our control theoretic framework, the entities involved are the non-atomic players (drivers) and \textbf{an authoritative central decision maker}.
    % \item In repeated games, the problem is designed in the point of view of non-atomic players (drivers). In our control theoretic framework, the problem is designed \textbf{in the point of view of a central decision maker}.
    \item In repeated games for parallel networks, the two entities involved, the player and the central decision maker are the same (a flow allocator). However, in our control theoretic framework, the two entities are different -- \textbf{players being the drivers} (in the present case aggregated as non-atomic along the edges) and \textbf{the central decision-maker being the flow allocator}.
    \item In repeated games, the players update their flow allocation based on their memory $\flowiter$ and the incurred loss $\lossiter$ on the network. In our control theoretic framework, the players update their flow allocation based on \textbf{their memory} $\stateiter$ and \textbf{the central decision maker's suggested routing decision $\controliter$}.
    \item In repeated games, one possible goal of the non-atomic player, the flow allocator, (see for example \cite{pmlr-v37-krichene15} \cite{krichene2015heterogeneous}) is to update their flow allocation in order to converge to the set of Nash equilibria and to achieve sub-linear regret. In our control theoretic framework, \textbf{the goal of the central decision maker is to steer the flow allocation to a target flow distribution, by inputting suggestions to the system's players (drivers)}.
\end{enumerate}


% In some problems, the design of $f_t$ is the question (for ex. with Walid, we had 3 different $f_t$s for which we proved a few things
% In the following sections, we design specific $f_t$ to cast the repeated game problem in a control theroretic framework. 


% References to site:
% \begin{itemize}
%     \item https://web.ece.ucsb.edu/~jrmarden/files/marsha2017.pdf
%     \item http://walid.krichene.net/papers/TCNS-routing.pdf
%     \item http://walid.krichene.net/papers/TCPS-learning-player-dynamics.pdf
%     \item Optimal Control references/books: ...
% \end{itemize}

% These decision-makers under the perspective of algorithmic game theory are labeled as "players" of the game. In an atomic routing game, the players take the form of individual drivers (\textbf{cite atomic lit}), whereas in a non-atomic routing game, players take the form of entities that control flows of drivers in the network (\textbf{cite nonatomic lit}). Similar connections exist under the perspective of controls, where "decision-makers" take the form of controllers \textbf{(cite lit)}. Here, the goal is similarly to design strategies for decision-makers and analyze performance and their properties, such as stability, observability, and controllability.

%However, a key difference is: \textit{in some game theoretic problems, the design of $u(\cdot)$ is determined before the dynamics of a system, $f(\cdot, \cdot)$, is known, whereas in controls, we'd solve $u(\cdot)$ using a specific design of $f(\cdot, \cdot)$ for the game}. In algorithmic game theory, the "dynamics" of the routing system itself is dependent on decisions made by every player in the network, and this is typically assumed to be unknown (\textbf{cite someone}). Whereas, typically, in controls, we design a controller's strategy assuming we know a bit about the dynamics of the system. If we apply this to repeated games, this would mean that we'd design learning strategies after assuming strategies for other players in the network. Therefore, by transforming the routing game within our framework, we more close tie the link between assumptions made for others players and the optimal control strategy for our system's decision-maker.

\subsubsection{Designing Games with LQR}
\label{Subsubsec:GameDesign}
We now describe our control routing model.\\
%\todo[inline]{N parallel edges -- We should probably say "flows" as per Alex's feedback. Throughout this section, let's change "edge" to flows.}
\begin{enumerate}
    \item States and controls: the \textit{state} of the LQR at time $\timesym$ is the flow vector \stateiter, consisting of the flow on each edge at time $t$, and the \textit{control} at time $\timesym$ is the flow allocation $ \controliter$ given by the decision maker, i.e.,
    \begin{linenomath*}
    \begin{align}
    \stateiter = (x_{1}^{\timesym},\dots, x_{\numedges}^{\timesym})^\top&, t = 0, \dots, T\\
    \controliter = (u_{1}^{\timesym},\dots, u_{\numedges}^{\timesym})^\top&, t = 0, \dots, T-1.
    \end{align}
    \end{linenomath*}
    
    We model both $\stateiter,\controliter \in \flowset$ at each time step \timesym.
    \item Equation for the dynamics: we assume the dynamics of the flow update is described using a linear time invariant difference equation
    \begin{linenomath*}
    \begin{align}
    \stateiterplus = \gamma A \stateiter + (1-\gamma)B \controliter, t = 0, 1, \dots, T-1
    \end{align}
    \end{linenomath*}
    where $\gamma \in [0,1]$ is a design parameter that weights the contribution of $\stateiter$ and $\controliter$ in the update rule, and $A, B \in \mathbb{R}^{\numedges \times \numedges}$ are two design matrices deciding how the flow vectors $\stateiter$ and $\controliter$ will affect the drivers' routing decision in the subsequent time step respectively.
    \item Cost function: the cost function of our control problem is a summation of quadratic functions
    \begin{linenomath*}
    \begin{align}
        \sum_{t = 0}^{T-1} \left(\stateiter^\top Q \stateiter + \controliter^\top R \controliter \right)+ \state_T^\top Q_f \state_T
    \end{align}
    \end{linenomath*}
    where $Q, Q_f, R \succeq 0$.
\end{enumerate}

%\todo[inline]{Yiling: If all of the examples below are R=0, we should consider putting R=0 here. I believe they are right?}

The resulting control problem is
\begin{linenomath*}
\begin{align}  
    &\underset{\controliter, t = 0, \dots, T-1}{\text{minimize}} &\sum_{t = 0}^{T-1} \left(\stateiter^\top Q \stateiter + \controliter^\top R \controliter \right)+ \state_T^\top Q_f \state_T& \label{begin_lqrrouting}\\ 
    &\text{subject to }&\stateiterplus = \gamma A \stateiter + (1-\gamma)B \controliter&, t = 0, 1, \dots, T-1\\
    & & \stateiter \in \flowset&, t = 0, \dots, T \\
    & & \controliter \in \flowset&, t = 0, \dots, T-1 \label{end_lqrrouting}
\end{align}
\end{linenomath*}

\subsubsection{Interpretation of the Framework}
\label{Subsubsec:Interp}
We now provide interpretations for the design of the control system. 
\begin{enumerate}
    \item States $\stateiter$: 
    the interpretation of the state $\mathbf{x}_t$ is twofold: (1) one could interpret it as the routing decision made by the drivers from one day to another, and (2) it is also the \textit{actual flow distribution} on the network, incurred by the drivers. We assume all drivers comply with a routing decision which depends at the same time on the past state, and the control.
    \item Controls $\controliter$: One could interpret the control $\controliter$ as the recommended routing decision from the central decision maker.
    \item The $A\stateiter$ term in the dynamics represents the mapping from the drivers' memory (past state inherited from the day before) to their  flow allocation decision. 
    \item The $B\controliter$ term in the dynamics represents the mapping from the central decision maker's suggested routing distribution to the players' flow allocation decision.
    %between Google maps action and flow allocation
    \item When updating their flow allocation decision, the drivers leverage their memory $\stateitert$ and the suggested routing distribution $\controliter$ from the decision maker. $\gamma\in [0,1]$ is the design parameter that characterizes the trade-off between the two contributions.
    \item (Quadratic) Cost function: the design of the quadratic cost function $\stateiter^\top Q \stateiter + \controliter^\top R \controliter$ is motivated by the observation that the Rosenthal potential function and the cost function associated to social welfare in a potential game are both quadratic for linear latency functions \cite{Rosenthal1973ACO}.\\
    
    \begin{definition}[Rosenthal potential] The Rosenthal potential function of a potential game, with a flow vector $\state$, is defined as
    \begin{linenomath*}
    \begin{align}
        \mathcal{J}_1(\state) = \sum_{\edgeelem \in \edgeset}\int_0^{x_e} \latfunc(y)\,\mathrm{d}y.
    \end{align}
    \end{linenomath*}
    \end{definition}
    
    \begin{definition}[Social Welfare] The cost function associated to social welfare is defined as
    \begin{linenomath*}
    \begin{align*}
        \mathcal{J}_2(\state) = \sum_{\edgeelem\in \edgeset}x_e \cdot \latfunc(x_e),
    \end{align*}
    \end{linenomath*}
    \end{definition}
    \\
    
    The importance of the Rosenthal potential and the social welfare is that the Nash equilibrium and social optimal of the routing game can be characterized as the local minimizers of these functions respectively, respecting the conservation of flow. With linear latency parallel networks,
    \begin{linenomath*}
    \begin{align}
        \mathcal{J}_1(\state) = \sum_{i=1}^{\numedges}\int_0^{x_i} (a_i y+b_i)\,\mathrm{d}y = \sum_{i=1}^{\numedges} \frac{a_ix_i^2}{2} +b_i x_i = \state^\top \tilde{Q} \state + \mathbf{b}^\top \state,
    \end{align}
    \end{linenomath*}
where $\tilde{Q} = \text{diag}(\frac{a_1}{2},\dots, \frac{a_{\numedges}}{2}), \mathbf{b} = (b_1, \dots, b_{\numedges})$ and 
\begin{linenomath*}
    \begin{align}
        \mathcal{J}_2(\mathbf{x}) = \sum_{i = 1}^{\numedges} x_i (a_i x_i +b_i) = \sum_{i=1}^{\numedges} a_ix_i^2 +b_i x_i = 2\state^\top \tilde{Q} \state + \mathbf{b}^\top \state,
    \end{align}
    \end{linenomath*}
    with the $\tilde{Q}, \mathbf{b}$ defined as the same as above. Note that $\tilde{Q}$ and \textbf{b} are used to construct $Q$ and $Q_f$ of the cost function.  
    
    
    \item Design of the matrix $A$ in the dynamics: since the $A\mathbf{x}_t$ is the mapping from the memory to the flow allocation decision, the matrix $A$ should reflect how the drivers take the memory into account when updating their routing decisions.
    \item Design of the matrix $B$ in the dynamics: since the $B\mathbf{u}_t$ is the mapping from the suggested routing distribution to the flow allocation decision, the matrix $B$ should reflect how the drivers take the central decision maker's suggested flow into account when updating their routing decisions.
    %Non-compliance (definitely refer Jerome Thai's paper: $\alpha$ proportion of non-compliant user
\end{enumerate}
%Interpretation 2 for u(t) and x(t) and dynamics:\\
%u(t) is the desired routing distribution from google maps. (Ex. I want to route 1/3 of my users on route 1, 1/3 on route 2, and the rest on route 3).\\
%x(t) is the actual routing observed on the network (even though google told you to go on route 2, you took route 1 and thus, the actual routing distribution in city 1 is different from google's desired). \\
%B*u(t) is the map from google's desired to what the drivers actually do. If driver's already listen to google maps no matter what then B = I, any deviation then B $\neq$ I. Why does this mapping have to be linear. So it doesn't. So in general it could be non-linear. Maybe in our case, we have an example in which which a linear model is sufficient. Just for LQR setting. Let's take another B matrix with slightly smaller diagonal matrices. In the process between what the driver sees on google and what it decides to do, it will weight google heavily. The entries of the diagonals of B is how much the drivers want to follow what google tells them to do, meaning it can be a probability of how likely drivers will take specific routes given that they've been recommended to take another (or the same) route. \\ 
%A*x(t-1): What would this mean if google maps control the whole traffic demand on the network (if all users in the city uses google)? If google doesn't influence the whole city,

%Say $r_u = 4$ is uncontrolled flow and $r_c = 6$ is controlled flow, total flow = 10.
%v(t) is the observed flow distribution of uncontrolled flow and w(t) is the observed flow distribution of controlled flow. 
%Observed flow distribution x(t) = v(t) + w(t)
%x(t+1) = Av(t) + Aw(t)

%Another way to look at it: the drivers each takes 2 things into account - suggestions by google maps and the observed times/flows on the roads by the drivers themselves. Therefore, B*u(t) is how they take this into account (explained a bit above) but then A*x(t) is how they take the observed travel flows/times into account in their decisions. Think about the two cases: A = I, A = 1/3*ONES. If A = I, to make the next decision, players only considers the travel times on the routes they've taken. Whereas, if A = 1/3 * ONES, players observe all travel times/flows on each route and considers it in their decision. They consider all routes equally because drivers have equal preferences on each route. The A matrix can also represent access/lack of access to this information. If A have unbalanced entries, means drivers can have different preferences/access to information. \\
%Question: Is the observed network flow the same as the decisions made by the drivers? I mean once the players makes decision (which is what we're explaining above) are they guaranteed to take this route/will this be the observed flow we see on the network? \\

%Our thoughts: It can be reasonable to assume that the decisions of the players (once they've made them) is what we'll observe on the network). Maybe later we can see how to break this assumption and maybe this relationship in the dynamics.\\

%Since Google maps has control of u(t) and not x(t), then what should the objective function be dependent on - x(t) or u(t)? The objective function represents regret or rosenthal and thus we're trying to reach an equilibrium. Do we want an equilibrium on u(t) or x(t)? \\


%Later problem: If we're Google, how do we learn A & B? What if we assume that the system ID is already done?

%We considered two different cost functions:


\section{System Analysis and System Properties} \label{Sec:SysAnalysis}
One of the contributions of the work is about how to design specific A and B matrices to produce various convergence results.
\begin{enumerate}
    \item Construction of $A, B$: when designing the matrices $A, B$ in the dynamics, we need to take the conservation of flow into account. More specifically, $A, B$ have to be chosen such that the following property holds
    \begin{linenomath*}
    \begin{equation}
        \stateiter, \controliter \in \flowset \quad \implies  \quad \gamma A\stateiter + (1-\gamma)B\controliter = \stateiterplus \in \flowset.
        \label{constraints:flow_cons}
    \end{equation}
    \end{linenomath*}
    One way to ensure the conservation of flow on the network is to construct \textit{left stochastic} $A, B$.\\
    \begin{definition}
    A matrix $P=(\mathbf{p}_1, \dots, \mathbf{p}_{\numedges})\in \mathbb{R}^{\numedges\times \numedges}$ is \textit{left stochastic} if $\mathbf{p}_i \in \Delta, i = 1, \dots, \numedges$.
    \end{definition}
    \begin{lemma}If $A, B\in \mathbb{R}^{\numedges\times \numedges}$ are left stochastic, and $\initstate, \controliter \in\flowset, t = 0, \dots, T-1 $, then $\gamma A\stateiter +(1-\gamma) B\controliter\ = \stateiterplus \in \flowset, t = 0, \dots, T-1$.
    \begin{proof}
    We will show that if $\stateiter, \controliter \in \flowset$, then $\gamma A\stateiter +(1-\gamma) B\controliter = \stateiterplus \in \flowset$. The proof is then complete by induction on $t$. \\
    First observe that $\mathbf{x}_{t+1}$ has non-negative entries due to the non-negativity of the entries in $A, B, \stateiter, \controliter$. 
    Furthermore,
    \begin{linenomath*}
    \begin{align}
        \mathbb{I}^\top \stateiterplus &= \gamma \mathbb{I}^\top A \stateiter + (1-\gamma)\mathbb{I}^\top B \controliter\\
        &= \gamma \mathbb{I}^\top \stateiter + (1-\gamma)\mathbb{I}^\top \controliter\\
        & = \gamma + (1-\gamma) = 1.
    \end{align}
    \end{linenomath*}
    \end{proof}
    \label{lemma:flow_cons}
    \end{lemma}
    \item Examples: the analysis of the LQR problem with probability simplex constraints is in general not tractable. In other words, we are not aware of a way to solve the discrete-time  algebraic  Ricatti equation in a way that preserves \eqref{constraints:flow_cons}. We therefore provide the important special cases where either (1) exact calculations of the steady state and optimal controls are allowed, or (2) interesting behavioral interpretation of the players can be given.
    \begin{example}
    We first consider the special case where
    \begin{equation}
    B=\begin{pmatrix}
        \frac{1}{\numedges}& \frac{1}{\numedges}&\dots &\frac{1}{\numedges}\\
        \frac{1}{\numedges}& \frac{1}{\numedges}&\dots &\frac{1}{\numedges}\\
        \vdots  & \vdots  & \ddots & \vdots  \\
        \frac{1}{\numedges}& \frac{1}{\numedges}&\dots &\frac{1}{\numedges}\\
        \end{pmatrix}\in \mathbb{R}^{\numedges\times \numedges}.
    \end{equation}
        This choice of $B$ matrix in the dynamics can be interpreted as follows: when the players (drivers) leverage the central decision maker's suggested routing distribution $\controliter$ to update their flow allocation on each edge, they simply average the suggested flow at each time step $\timesym$, and take only the average $\frac{1}{\numedges}\sum_{i = 1}^{\numedges} u_i^t$ into account.\\
        We show that when the players (drivers) update their flow allocation in this way, the controller $\controliter$ is essentially ``muted'', and therefore a target state may not be controllable. The state $\stateiter$ will converge to the same equilibrium that is independent of the choice of the cost function.
        \begin{property}
            Consider the control problem \eqref{begin_lqrrouting}-\eqref{end_lqrrouting} with 
            \begin{equation}\label{eq:1_3_B}
               B =
               \begin{pmatrix}
        \frac{1}{\numedges}& \frac{1}{\numedges}&\dots &\frac{1}{\numedges}\\
        \frac{1}{\numedges}& \frac{1}{\numedges}&\dots &\frac{1}{\numedges}\\
        \vdots  & \vdots  & \ddots & \vdots  \\
        \frac{1}{\numedges}& \frac{1}{\numedges}&\dots &\frac{1}{\numedges}\\
        \end{pmatrix},
        \gamma \in [0,1), \text{ and any left stochastic matrix }A, 
        \end{equation}
        then the unique steady state of the system is given by
        \begin{equation}
            \state\optimal = \frac{1-\gamma}{\numedges}(I_{\numedges}-\gamma A)^{-1}\mathbb{I},
        \end{equation}
        where $I_{\numedges}$ is the $\numedges$-dimensional identity matrix, and $\mathbb{I} = (1, 1, \dots, 1)^\top \in \mathbb{R}^{\numedges}$ is the all-ones vector.
        \begin{proof}
        The key observation is, with equation (\ref{eq:1_3_B}), since we have $\controliter \in \flowset, t = 0, \dots, T-1$, 
        \begin{linenomath*}
        \begin{align}
            B\controliter = \frac{1}{\numedges} \mathbb{I},
        \end{align}
        \end{linenomath*}
        therefore
        \begin{linenomath*}
        \begin{align}
            \stateiterplus=\gamma A\stateiter + (1-\gamma)\frac{1}{\numedges} \mathbb{I},
        \end{align}
        \end{linenomath*}
        and the steady state should satisfy
        \begin{equation}
            \state\optimal=\gamma A\state\optimal + (1-\gamma)\frac{1}{\numedges} \mathbb{I}, \quad \implies \quad \state\optimal = \frac{1-\gamma}{\numedges}(I_{\numedges}-\gamma A)^{-1}\mathbb{I}, 
        \end{equation}
        with the invertibility of $I_{\numedges}-\gamma A$ guaranteed by the fact that the spectral radius of any left stochastic matrix is at most $1$, and $\gamma<1$.
        \end{proof}
        \end{property}
        The foregoing property suggests that in the case of equation \eqref{eq:1_3_B}, the flow allocation on the network does converge to an equilibrium, but the equilibrium depends only on the design parameters $A, \gamma$ and the number of edges $\numedges$, which can be different from the Nash equilibrium.
        \end{example}
        \begin{example}
        We next consider the special case where
        \begin{equation}
        A = \begin{pmatrix}
        \frac{1}{\numedges}& \frac{1}{\numedges}&\dots &\frac{1}{\numedges}\\
        \frac{1}{\numedges}& \frac{1}{\numedges}&\dots &\frac{1}{\numedges}\\
        \vdots  & \vdots  & \ddots & \vdots  \\
        \frac{1}{\numedges}& \frac{1}{\numedges}&\dots &\frac{1}{\numedges}\\
        \end{pmatrix}\in \mathbb{R}^{\numedges\times \numedges}.
        \end{equation}
        This choice of $A$ matrix in the dynamics can be interpreted as follows: when the players (drivers) leverage 
        their memory $\stateiter$ to update their flow allocation on each edge, they simply average the past flow at each time step $\timesym$, and take only this average $\frac{1}{\numedges}\sum_{i = 1}^{\numedges} x_i^t$ into account.\\
        We similarly show that when the players (drivers) update their flow allocation in this way, their memory has no impact in the update rule.
        \begin{property} \label{1/N_A}
            Consider the control problem \eqref{begin_lqrrouting}-\eqref{end_lqrrouting} with 
            \begin{equation}\label{eq:1_3_A}
               A =
               \begin{pmatrix}
        \frac{1}{\numedges}& \frac{1}{\numedges}&\dots &\frac{1}{\numedges}\\
        \frac{1}{\numedges}& \frac{1}{\numedges}&\dots &\frac{1}{\numedges}\\
        \vdots  & \vdots  & \ddots & \vdots  \\
        \frac{1}{\numedges}& \frac{1}{\numedges}&\dots &\frac{1}{\numedges}\\
        \end{pmatrix} \text{ and any left stochastic matrix } B,  
        \end{equation}
        then the optimal controller $\controliter, t = 0, \dots, T-2$ is the solution set of the optimization problem
        \begin{linenomath*}
        \begin{align}
    \underset{\control}{\text{minimize}}\quad&\left( \frac{\gamma}{\numedges} \mathbb{I} + (1-\gamma)B\control\right)^\top Q \left( \frac{\gamma}{\numedges} \mathbb{I} + (1-\gamma)B\control\right) + \control^\top R \control\\
    \text{subject to}\quad& \control \in \flowset,
\end{align}
\end{linenomath*}
and the optimal $\control_{T-1}$ is the solution set of the optimization problem
\begin{linenomath*}
\begin{align}
    \underset{\control}{\text{minimize}}\quad&\left( \frac{\gamma}{\numedges} \mathbb{I} + (1-\gamma)B\control\right)^\top Q_f \left( \frac{\gamma}{\numedges} \mathbb{I} + (1-\gamma)B\control\right) + \control^\top R \control\\
    \text{subject to}\quad& \control\in \flowset.
\end{align}
\end{linenomath*}
        \begin{proof}
        The key observation is, with equation (\ref{eq:1_3_A}), since we have $\stateiter \in \flowset, t = 0, \dots, T-1$, 
        \begin{linenomath*}
        \begin{align}
            A\stateiter = \frac{1}{\numedges} \mathbb{I},
        \end{align}
        \end{linenomath*}
        therefore
        \begin{linenomath*}
        \begin{align}
            \stateiterplus=\gamma \frac{1}{\numedges} \mathbb{I} + (1-\gamma)B\controliter.
        \end{align}
        \end{linenomath*}
        Therefore, the optimal control of problem  \eqref{begin_lqrrouting}-\eqref{end_lqrrouting} can be explicitly solved by the optimization problem
        \begin{linenomath*}
        \begin{align}
    \underset{\controliter, t=0,\dots T-1}{\text{minimize}}\quad&\initstate^\top Q \initstate+ \sum_{t = 0}^{T-2} \left(\left( \frac{\gamma}{\numedges} \mathbb{I} + (1-\gamma)B\controliter\right)^\top Q \left( \frac{\gamma}{\numedges} \mathbb{I} + (1-\gamma)B\controliter\right) + \controliter^\top R \controliter \right)+\nonumber\\
    &\left( \left(\frac{\gamma}{\numedges} \mathbb{I} + (1-\gamma)B\mathbf{u}_{T-1}\right)^\top Q_f \left( \frac{\gamma}{\numedges} \mathbb{I} + (1-\gamma)B\control_{T-1}
    \right) + \control_{T-1}^\top R \control_{T-1}\right)\\
    \text{subject to}\quad& \controliter \in \flowset, t = 0, \dots, T-1, 
\end{align}
\end{linenomath*}
which is further equivalent to solving the constrained optimization problems
\begin{linenomath*}
\begin{align}
    \underset{\control}{\text{minimize}}\quad&\left( \frac{\gamma}{\numedges} \mathbb{I} + (1-\gamma)B\control\right)^\top Q \left( \frac{\gamma}{\numedges} \mathbb{I} + (1-\gamma)B\control\right) + \control^\top R \control\\
    \text{subject to}\quad& \control \in \flowset
\end{align}
\end{linenomath*}
and
\begin{linenomath*}
\begin{align}
    \underset{\control}{\text{minimize}}\quad&\left( \frac{\gamma}{\numedges} \mathbb{I} + (1-\gamma)B\control\right)^\top Q_f \left( \frac{\gamma}{\numedges} \mathbb{I} + (1-\gamma)B\control\right) + \control^\top R \control\\
    \text{subject to}\quad& \control \in \flowset.
\end{align}
\end{linenomath*}
If $Q_f=Q$ and the solution of the above optimization problem exists, the minimizer $\control\optimal$ characterizes the steady state $\state\optimal = \frac{\gamma}{\numedges} \mathbb{I} + (1-\gamma)B\control\optimal$.
        \end{proof}
        \end{property}
        Note that in the very specific case where $R = 0$ and $Q, Q_f$ are defined by the Rosenthal potential function, the minimizer of the above optimization problem and steady state of the system $\state\optimal$ is the Nash equilibrium. If the linear equation system $\state\optimal = \frac{\gamma}{\numedges} \mathbb{I} + (1-\gamma)B\control$ has at least one solution $\control\optimal$ (e.g., when $B$ is invertible and $\gamma\neq 1$), then the  optimal controllers are $\controliter = \control\optimal, t = 0, \dots, T-1$. 
         \end{example}
         \begin{example}
         The third special case we would like to analyze is $A = B = I_{\numedges}$. The players update their flow allocation with $\stateiterplus = \gamma \stateiter + (1-\gamma) \controliter$ at each time step $\timesym$, which is the same as the element-wise update $x_i^{t+1} = \gamma x_i^t + (1-\gamma) u_i^t, i = 1, \dots, N, t = 0, \dots, T-1$.\\
         The interpretation of this choice of $A,B$ is that the players update the flow on each edge \textit{independently}: to update the flow on edge $i$, the players leverage their memory and the suggested routing decision on the edge $i$ only.
         \end{example}
\end{enumerate}


% \todo[inline]{Should we prove stability, controllability, feasibility? Any other properties?}

\section{Solutions via Explicit MPC: A Multiparametric Quadratic Programming Approach}
\label{Sec:MPC}
\begin{figure}[h]
\centering
\includegraphics[scale=0.2]{figures/A111_Q111_R0_gamma0.5_traj.png}
\caption{Here, the optimal strategy for our player is space-varying and we visualize solutions with respect to the feasible state space of the routing game. Each colored region of the graph represents a unique affine strategy that is optimal for those points in space. For example, region 1 (in green) has the solution $\controliter\optimal(\stateiter)$ = $\begin{pmatrix} -\frac{2}{3} & \frac{1}{3} & \frac{1}{3}\\ \frac{1}{3} & -\frac{2}{3} & \frac{1}{3} \\
\frac{1}{3} & \frac{1}{3} & -\frac{2}{3} \\
\end{pmatrix} \stateiter + \begin{pmatrix} \frac{1}{3} \\
\frac{1}{3} \\
\frac{1}{3} \end{pmatrix}$.}
\label{fig:example_cr}
\end{figure}

At first glance, one might consider using the discrete-time algebraic Ricatti equation to obtain solutions for system \eqref{begin_lqrrouting}-\eqref{end_lqrrouting}. 
\begin{definition}[Discrete-time Algebraic Ricatti Equation] The discrete-time algebraic Ricatti equation is a nonlinear equation that gives a solution to the LQR problem presented in equation \eqref{sys:lqr}, described as $P_t$ evolving backwards in time from $P_T &= Q_f$ according to
\begin{equation}
    P_{t-1} &= Q + A\transpose P_{t} A - A\transpose P_{t} B(R + B\transpose Q_f B)\inv B\transpose P_{t} A.
    \end{equation}
\end{definition}

However, using the algebraic Riccati equation is not possible in the presence of our flow conservation constraints, as specified in equation \eqref{constraints:flow_cons}. According to lemma \eqref{lemma:flow_cons}, in order to design a flow preserving scheme and guarantee flow conservation, we must be able to guarantee that each $\stateiter$ and $\controliter$ vector given by a chosen controller remains on the probability simplex $\flowset$, while the optimal controller given by the algebraic Riccati equation drives the system to the steady state $\state\optimal = 0$. Therefore, we turn to multiparametric quadratic programming (mpQP), a technique used in explicit MPC to generate explicit piecewise affine controllers. To generate these explicit strategies, we will formulate the LQR problem into a mpQP problem, utilize an mpQP solver proposed in  \cite{bemporad2015multiparametric} to generate piecewise affine functions for $\controliter$ (the player needs to execute different affine controllers depending on the state), and use (within the solver) a geometric algorithm to plot regions, known as \textit{\textbf{critical regions}}, on the state space to visualize when players should use which specific optimal strategies. Optimal strategies produced by this technique will be piecewisely-affine with respect to the state of the game, hence, optimal strategies in this context are space-varying (see figure \eqref{fig:example_cr} for an example).

Algorithm \eqref{alg:mpc_algo} defines the process by which we use mpQP to generate solutions for routing games. Specifically, we consider the optimal control formulation in problem \eqref{begin_lqrrouting}-\eqref{end_lqrrouting}. We take the linear flow and input constraints in \eqref{constraints:flow_cons} and construct them in the form
\begin{linenomath*}
    \begin{align}
       A_u \controliter \leq b_u, \quad A_x \stateiter \leq b_x.
    \end{align}
    \end{linenomath*}
    To solve for the optimal controls $\control_0,\dots, \control_{T-1}$, first we condense the problem into a strictly convex quadratic programming problem
    \begin{linenomath*}
\begin{align}
    \label{sys:begincondenseqp}
    \condenseqpobj\optimal(x) &\triangleq& &\textit{minimize}& &\frac{1}{2} z^\top Pz + (Fx + c)^\top z + \frac{1}{2} x^\top Yx& \\
    &&&\textit{subject to}& & Gz \leq W + Sx&
    \label{sys:endcondenseqp}
\end{align}
\end{linenomath*}
% \begin{align}  
%     &\text{minimize} &\sum_{t = 0}^{T-1} \left(\mathbf{x}_t^\top Q \mathbf{x}_t + \mathbf{u}_t^\top R \mathbf{u}_t \right)+ \mathbf{x}_T^\top Q_f \mathbf{x}_T& \label{begin_lqrrouting}\\ 
%     &\text{subject to }&\mathbf{x}_{t+1} = \gamma A \mathbf{x}_t + (1-\gamma)B \mathbf{u}_t&, t = 0, 1, \dots, T-1\\
%     & & \mathbf{x}_t \in \Delta&, t = 0, \dots, T \\
%     & & \mathbf{u}_t \in \Delta&, t = 0, \dots, T-1 \label{end_lqrrouting}
% \end{align}
and then use the mpQP algorithm from reference \cite{bemporad2015multiparametric} to solve for $z$ where $z := \left( \control_0^\top \dots \control_{T-1}^\top \right)^\top \in \R^{\nmpc}$ is the decision  variable.

$P=P^\top \in \R^{\nmpc \by \nmpc}$, $F \in \R^{\nmpc \by \mmpc}$, $c \in \R^{\nmpc}$, $Y \in \R^{\mmpc \by \mmpc}$ are defined by the cost matrices, and $G \in \R^{\nmpc \by \qmpc}$, $ W \in \R^{\qmpc}$, $S \in \R^{\qmpc \by \mmpc}$ define the constraints imposed by \eqref{begin_lqrrouting}-\eqref{end_lqrrouting} in compact form. The following property guarantees the existence of a (piecewise affine) solution of the condensed problem \eqref{sys:begincondenseqp}-\eqref{sys:endcondenseqp}.

\begin{property}[Existence of a piecewise affine solution \cite{bemporad2015multiparametric}] Consider \eqref{sys:begincondenseqp}-\eqref{sys:endcondenseqp} with $P=P^\top \succ 0$ and let $x\in \stateset=\R^n$.
\begin{enumerate}
    \item The set $\stateset_f$ of states for which the problem is feasible is a polyhedron.
    \item The optimizer function $z\optimal: \stateset_f \to \mathbb{R}^n$ is piecewise affine and continuous over $\stateset_f$.
    \item If 
   $ \begin{pmatrix}
        P &\F^\top\\
        \F &\Y \\
    \end{pmatrix} \succeq 0$ and symmetric, then the value function $\condenseqpobj\optimal$ is continuous, convex, and piecewise quadratic over $\stateset_f$.
\end{enumerate}
\end{property}

\begin{definition}[Critical Region \cite{spjotvold2006facet}] A critical region is a polyhedron in $\stateset$ for which there exists an optimal solution $z\optimal(\cdot)$ that is affine and optimal for the entire region. Each critical region is defined by a unique set of active constraints $\activeset$ that is common for all points in the region. 
\end{definition}

\IncMargin{1em}
\begin{algorithm}
    % \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
    % \SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
    
    % \Input{$Q$,$R$,$Q_f$,$N_c$,$A$,$B$,$Au$,$bu$,$Ax$,$bx$}
    % \Output{Optimal strategy solution {K^\regions , h^\regions , E^\regions , e^\regions }_{\regions \in \stateset}.}
    % \BlankLine
    % \emph{special treatment of the first line}\;
    % \For{$i\leftarrow 2$ \KwTo $l$}{
    %     \emph{special treatment of the first element of line $i$}\;
    %     \For{$j\leftarrow 2$ \KwTo $w$}{\label{forins}
    %         \Left$\leftarrow$ \FindCompress{$Im[i,j-1]$}\;
    %         \Up$\leftarrow$ \FindCompress{$Im[i-1,]$}\;
    %         \This$\leftarrow$ \FindCompress{$Im[i,j]$}\;
    %         \If(\tcp*[h]{O(\Left,\This)==1}){\Left compatible with \This}{\label{lt}
    %             \lIf{\Left $<$ \This}{\Union{\Left,\This}}
    %             \lElse{\Union{\This,\Left}}
    %         }
    %         \If(\tcp*[f]{O(\Up,\This)==1}){\Up compatible with \This}{\label{ut}
    %             \lIf{\Up $<$ \This}{\Union{\Up,\This}}
    %             \tcp{\This is put under \Up to keep tree as flat as possible}\label{cmt}
    %             \lElse{\Union{\This,\Up}}\tcp*[h]{\This linked to \Up}\label{lelse}
    %         }
    %     }
    %     \lForEach{element $e$ of the line $i$}{\FindCompress{p}}
    % }
    \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
    \SetKwData{qp}{$P,F,c,Y,G,W,S$}\SetKwData{input}{$Q$,$R$,$Q_f$,$N_c$,$A$,$B$,$A_u$,$b_u$,$A_x$,$b_x$}
    \SetKwFunction{Condense}{Condense}\SetKwFunction{mpqpAlgo}{MPQPSolver}
    \Input{\input}
    \Output{Optimal strategy solutions: \mpcctrl, \mpcctrladd\\ Critical Regions to apply solutions: \CR, \CRCheckH, \CRCheckK, }
    \BlankLine
    \qp $\leftarrow$ \Condense{\input}\;
    $\textbf{return}$ \mpqpAlgo{\qp}\;
    \caption{disjoint decomposition}\label{algo_disjdecomp}
    \caption{mpQP algorithm}\label{alg:mpc_algo}
\end{algorithm}\DecMargin{1em}

As explained in (\cite{bemporad2015multiparametric}), $\mpqpAlgo(\cdot)$ uses a geometrical algorithm (see \cite{spjotvold2006facet}) to find the critical regions of the feasible state space by understanding when sets of active constraints differs from point to point in the state space. Once it has identified a critical region, the algorithm is able to uncover the optimal solution defined within the region by using KKT conditions (or similar methods) to obtain the piecewise affine solution $z\optimal$. Algorithm \eqref{alg:mpc_algo} produces (1) the critical regions $\CR$, (2) the matrices to check if a state is in specific critical region, $\CRCheckH = \{\CRCheckH_r\}$ and $\CRCheckK = \{\CRCheckK_r\}$, and (3) the matrices that characterizes the affine solution $\mpcctrl = \{\mpcctrl_r\}$ and  $\mpcctrladd = \{\mpcctrladd_r\}$. Therefore, during the routing game, to recover the optimal strategies, the central decision maker executes
\begin{linenomath*}
\begin{align}
    \text{if } \CRCheckH_{\regionelem}\stateiter \leq \CRCheckK_{\regionelem} ~ \text{, then } \controliter\optimal = \mpcctrl_{\regionelem}\stateiter + \mpcctrladd_{\regionelem}
\end{align}
\end{linenomath*}
and \stateiter~belongs to critical region \regionelem. 

% \IncMargin{1em}
% \begin{algorithm}
%     \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
%     \SetKwData{input}{$Q,F,c,Y,G,W,S$}
%     \SetKwFunction{Condense}{Condense}\SetKwFunction{mpqpAlgo}{MPQPSolver}
%     \Input{\input}
%     \Output{Optimal strategy solution:}
%     \BlankLine
%     \qp $\leftarrow$ \Condense{\input}\;
%     $\textbf{return}$ \mpqpAlgo{\qp}\;
%     \caption{disjoint decomposition}\label{algo_disjdecomp}
%     \caption{MPQPSolver}\label{alg:mpc_solver}
% \end{algorithm}\DecMargin{1em}




% Here we go into LQR to mpQP setup. Then from mpQP to linear affine control laws. Might have to also explain polyhedrons.

% \subsection{Formal Analysis of explicit MPC}
% \todo[inline]{Formal analysis of how fast we converge to system equilibrium: Do we still need to show that if we're in same polyhedron will we converge in one step or not. Can we show?}
% \todo[inline]{Can we formally characterize what flow distributions we'll converge to?}

% \subsection{Finding the solutions to game}
% \begin{itemize}
%     \item What are we trying to solve for? What do we want to find?
%     \item What are the solutions given from our control formulations: Ricatti equation; explicit MPC
% \end{itemize}

\section{Illustration on Simple Numerics}
\label{Sec:Results}
In this section, we plan to provide numerical results and discuss
\begin{enumerate}
    \item differences in varying $A$ matrices in the dynamics, and the interpretations,
    \item changes in $\gamma$ and its effect on the converging rate, 
    \item different initial states and its effect on the converging rate,
    \item different cost functions to drive the system towards different stable equilibrium.
\end{enumerate}

More specifically, we will compare between
\begin{enumerate}
    \item $A = \begin{pmatrix}
        \frac{1}{3}& \frac{1}{3}&\frac{1}{3}\\
        \frac{1}{3}& \frac{1}{3}&\frac{1}{3}\\
        \frac{1}{3}& \frac{1}{3}&\frac{1}{3}
        \end{pmatrix}$ and  $A = I_3$,  with all the other parameters fixed as $B = I_3,  Q = Q_f = I_3, R = 0, \gamma = 0.5, \initstate = (0.3, 0.5, 0.2)^\top$. This means we investigate the differences between the players' routing decision process when they ``mute'' their memory, and when they leverage their memory on each edge independently (i.e., when $x_i^{t+1}$ depends only on $x_i^t$ in the past state $\stateiter$ for $i = 1, \dots, \numedges$). 
    \item $\gamma = 0.5$ and $\gamma = 0.7$:  with all the other parameters fixed as $A = B = I_3, Q = Q_f = \begin{pmatrix}
         1 & 0 & 0 \\
         0 & 2 & 0 \\
         0 & 0 & 4
    \end{pmatrix}, R = \begin{pmatrix}
         0 & 0 & 0 \\
         0 & 0 & 0 \\
         0 & 0 & 0
    \end{pmatrix}, \mathbf{x}_0 = (0.3, 0.5, 0.2)^\top$.  This means we investigate the differences between the players' routing decision process when they weight equally the their memory and the suggested flow, and when they weight more their memory (and less the suggestions).
    \item $\initstate = (0.3, 0.5, 0.2)^\top$ and $\initstate = (0, 1, 0)^\top$: with all the other parameters fixed as $A = B = I_3, Q = Q_f = \begin{pmatrix}
         1 & 0 & 0 \\
         0 & 2 & 0 \\
         0 & 0 & 4
    \end{pmatrix},  R = \begin{pmatrix}
         0 & 0 & 0 \\
         0 & 0 & 0 \\
         0 & 0 & 0
    \end{pmatrix}, \gamma = 0.5$. This means we investigate the differences between the players' routing decision process when they start with putting partial flow on each edge, and when they start with putting all flow on the second edge.
    \item $Q = Q_f = I_3$ and $Q = Q_f = \begin{pmatrix}
         1 & 0 & 0 \\
         0 & 2 & 0 \\
         0 & 0 & 4
    \end{pmatrix}$: with all the other parameters fixed as $A = B = I_3, R =\begin{pmatrix}
         0 & 0 & 0 \\
         0 & 0 & 0 \\
         0 & 0 & 0
    \end{pmatrix}, \gamma = 0.5, \initstate = (0.3, 0.5, 0.2)^\top$. This means we investigate the differences between the players' routing decision process when the central decision maker penalizes equally the flow on the three edges, and when it gradually doubles the penalty on the edges.
\end{enumerate}

\\
We also discuss the \textit{reliability of the solver} by showing one example, where the solver outputs the correct steady state solution only with large enough time horizon $T$. This example serves as an alert that in order to get the accurate numerical solution with the $\mpqpAlgo(\cdot)$, one needs to set a large time horizon $T$, at the price of longer computation time.

% \subsubsection{Com} We start with the simple parallel network, where the three paths have equal latency functions
% \begin{equation*}
%     l_i(f_i) = f_i, i = 1,2,3.
% \end{equation*}
% Therefore the running cost and terminal cost matrices corresponding to the states $F_t$ are
% \begin{equation*}
%     Q = P = \begin{pmatrix}
%          1 & 0 & 0 \\
%          0 & 1 & 0 \\
%          0 & 0 & 1
%     \end{pmatrix}
% \end{equation*}
% We first set the parameters
% \begin{equation*}
%     A = \begin{pmatrix}
%          \frac{1}{3} & \frac{1}{3} & \frac{1}{3} \\
%          \frac{1}{3} & \frac{1}{3} & \frac{1}{3} \\
%          \frac{1}{3} & \frac{1}{3} & \frac{1}{3}
%     \end{pmatrix},
%     B = \begin{pmatrix}
%          1 & 0 & 0 \\
%          0 & 1 & 0 \\
%          0 & 0 & 1
%     \end{pmatrix},N = 15,\gamma = 0.5, F_0 = \begin{pmatrix}
%     0.3& 0.5&0.2\end{pmatrix}^\top
%     \\
% \end{equation*}
% Below and in the following examples, we will show the convergence trajectory of the states in the probability simplex space, as well as the convergence of flow, latency function and optimal cost for the constrained LQR problem.

\subsection{Comparisons and Results}
For ease of reference, we list below the detailed choice of parameters in each figure.
In all experiments we assume no penalty on the controller (i.e., the central decision maker has the freedom to pose any suggested routing decision).\\

Figure \eqref{fig:A1:3_Q111_R0_gamma0.5}:
\begin{linenomath*}
\begin{align*}
 Q = Q_f = \begin{pmatrix}
         1 & 0 & 0 \\
         0 & 1 & 0 \\
         0 & 0 & 1
    \end{pmatrix},
    R = \begin{pmatrix}
         0 & 0 & 0 \\
         0 & 0 & 0 \\
         0 & 0 & 0
    \end{pmatrix}, 
A = &\begin{pmatrix}
         \frac{1}{3} & \frac{1}{3} & \frac{1}{3} \\
         \frac{1}{3} & \frac{1}{3} & \frac{1}{3} \\
         \frac{1}{3} & \frac{1}{3} & \frac{1}{3}
    \end{pmatrix},
    B = \begin{pmatrix}
         1 & 0 & 0 \\
         0 & 1 & 0 \\
         0 & 0 & 1
    \end{pmatrix},\\
    &T = 15,\gamma = 0.5, \initstate = \begin{pmatrix}
    0.3& 0.5&0.2\end{pmatrix}^\top
\end{align*}
\end{linenomath*}


Figure \eqref{fig:A111_Q111_R0_gamma0.5}:
\begin{linenomath*}
\begin{align*}
 Q = Q_f = \begin{pmatrix}
         1 & 0 & 0 \\
         0 & 1 & 0 \\
         0 & 0 & 1
    \end{pmatrix},
    R = \begin{pmatrix}
         0 & 0 & 0 \\
         0 & 0 & 0 \\
         0 & 0 & 0
    \end{pmatrix}, 
A = &\begin{pmatrix}
         1 & 0 & 0 \\
         0 & 1 & 0 \\
         0 & 0 & 1
    \end{pmatrix},
    B = \begin{pmatrix}
         1 & 0 & 0 \\
         0 & 1 & 0 \\
         0 & 0 & 1
    \end{pmatrix},\\
    &T = 15,\gamma = 0.5, \initstate = \begin{pmatrix}
    0.3& 0.5&0.2\end{pmatrix}^\top
\end{align*}
\end{linenomath*}

Figure \eqref{fig:A1:3_Q124_R0_gamma0.4}:
\begin{linenomath*}
\begin{align*}
 Q = Q_f = \begin{pmatrix}
         1 & 0 & 0 \\
         0 & 2 & 0 \\
         0 & 0 & 4
    \end{pmatrix},
    R = \begin{pmatrix}
         0 & 0 & 0 \\
         0 & 0 & 0 \\
         0 & 0 & 0
    \end{pmatrix}, 
A =& \begin{pmatrix}
         \frac{1}{3} & \frac{1}{3} & \frac{1}{3} \\
         \frac{1}{3} & \frac{1}{3} & \frac{1}{3} \\
         \frac{1}{3} & \frac{1}{3} & \frac{1}{3}
    \end{pmatrix},
    B = \begin{pmatrix}
         1 & 0 & 0 \\
         0 & 1 & 0 \\
         0 & 0 & 1
    \end{pmatrix},\\
    &T = 15,\gamma = 0.5, \initstate = \begin{pmatrix}
    0.3& 0.5&0.2\end{pmatrix}^\top
\end{align*}
\end{linenomath*}


Figure \eqref{fig:A111_Q124_R0_gamma0.5}:
\begin{linenomath*}
\begin{align*}
 Q = Q_f = \begin{pmatrix}
         1 & 0 & 0 \\
         0 & 2 & 0 \\
         0 & 0 & 4
    \end{pmatrix},
    R = \begin{pmatrix}
         0 & 0 & 0 \\
         0 & 0 & 0 \\
         0 & 0 & 0
    \end{pmatrix}, 
A =& \begin{pmatrix}
         1 & 0 & 0 \\
         0 & 1 & 0 \\
         0 & 0 & 1
    \end{pmatrix},
    B = \begin{pmatrix}
         1 & 0 & 0 \\
         0 & 1 & 0 \\
         0 & 0 & 1
    \end{pmatrix},\\
    &T = 15,\gamma = 0.5, \initstate = \begin{pmatrix}
    0.3& 0.5&0.2\end{pmatrix}^\top
\end{align*}
\end{linenomath*}

Figure \eqref{fig:A111_Q124_R0_gamma0.5_initial}:
\begin{linenomath*}
\begin{align*}
 Q = Q_f = \begin{pmatrix}
         1 & 0 & 0 \\
         0 & 2 & 0 \\
         0 & 0 & 4
    \end{pmatrix},
    R = \begin{pmatrix}
         0 & 0 & 0 \\
         0 & 0 & 0 \\
         0 & 0 & 0
    \end{pmatrix}, 
A =& \begin{pmatrix}
         1 & 0 & 0 \\
         0 & 1 & 0 \\
         0 & 0 & 1
    \end{pmatrix},
    B = \begin{pmatrix}
         1 & 0 & 0 \\
         0 & 1 & 0 \\
         0 & 0 & 1
    \end{pmatrix},\\
    &T = 15,\gamma = 0.5, \initstate = \begin{pmatrix}
    0&1&0\end{pmatrix}^\top
\end{align*}
\end{linenomath*}

Figure \eqref{fig:A111_Q124_R0_gamma0.7}:
\begin{linenomath*}
\begin{align*}
 Q = Q_f = \begin{pmatrix}
         1 & 0 & 0 \\
         0 & 2 & 0 \\
         0 & 0 & 4
    \end{pmatrix},
    R = \begin{pmatrix}
         0 & 0 & 0 \\
         0 & 0 & 0 \\
         0 & 0 & 0
    \end{pmatrix}, 
A =& \begin{pmatrix}
         1 & 0 & 0 \\
         0 & 1 & 0 \\
         0 & 0 & 1
    \end{pmatrix},
    B = \begin{pmatrix}
         1 & 0 & 0 \\
         0 & 1 & 0 \\
         0 & 0 & 1
    \end{pmatrix},\\
    &T = 15,\gamma = 0.7, \initstate = \begin{pmatrix}
    0.3&0.2&0.5\end{pmatrix}^\top
\end{align*}
\end{linenomath*}



\begin{figure}[h]
\includegraphics[width=8cm]{figures/A1:3_Q111_R0_gamma0.5_traj.png}
\includegraphics[width=8cm]{figures/A1:3_Q111_R0_gamma0.5_panel.png}
\caption{Identity $Q, Q_f, B$, $A = (1/3), \gamma=0.5$. "*" denotes the initial state.}
\label{fig:A1:3_Q111_R0_gamma0.5}
\end{figure}

\begin{figure}[h]
\includegraphics[width=8cm]{figures/A111_Q111_R0_gamma0.5_traj.png}
\includegraphics[width=8cm]{figures/A111_Q111_R0_gamma0.5_panel.png}
\caption{Identity $Q, Q_f, A, B$, $\gamma=0.5$. "*" denotes the initial state.}
\label{fig:A111_Q111_R0_gamma0.5}
\end{figure}


\begin{figure}[h]
\includegraphics[width=8cm]{figures/A1:3_Q124_R0_gamma0.4_traj.png}
\includegraphics[width=8cm]{figures/A1:3_Q124_R0_gamma0.4_panel.png}
\caption{Identity $B$, $A = (1/3), Q = Q_f = \mathrm{diag}(1,2,4),\gamma=0.5$. "*" denotes the initial state.}
\label{fig:A1:3_Q124_R0_gamma0.4}
\end{figure}

\begin{figure}[h]
\includegraphics[width=8cm]{figures/A111_Q124_R0_gamma0.5_traj.png}
\includegraphics[width=8cm]{figures/A111_Q124_R0_gamma0.5_panel.png}
\caption{Identity $A,B$, $Q = Q_f = \mathrm{diag}(1,2,4),\gamma=0.5$. "*" denotes the initial state.}
\label{fig:A111_Q124_R0_gamma0.5}
\end{figure}




\begin{figure}[h]
\includegraphics[width=8cm]{figures/A111_Q124_R0_gamma0.5_traj_init.png}
\includegraphics[width=8cm]{figures/A111_Q124_R0_gamma0.5_panel_init.png}
\caption{Identity $A,B$, $Q=Q_f=\mathrm{diag}(1,2,4),\gamma=0.5$, initial $(0,1,0)$. "*" denotes the initial state.}
\label{fig:A111_Q124_R0_gamma0.5_initial}
\end{figure}

\begin{figure}[h]
\includegraphics[width=8cm]{figures/A111_Q124_R0_gamma0.7_traj.png}
\includegraphics[width=8cm]{figures/A111_Q124_R0_gamma0.7_panel.png}
\caption{Identity $A,B$, $Q = Q_f = \mathrm{diag}(1,2,4),\gamma=0.7$. "*" denotes the initial state.}
\label{fig:A111_Q124_R0_gamma0.7}
\end{figure}

\textbf{Discussion:}
In each figure, we present on the left the probability simplex in $\mathbb{R}^3$, the critical regions in it (recall that within each partition the optimal controller takes different affine expression), and the convergence trajectory of the state $\stateiter$ (with the initial state denoted by $*$). On the right we present (1) the value of the flow allocation $\stateiter$ on each edge at each time step $\timesym$, (2) the value of the optimal control (suggested routing decision) $\controliter$ on each edge at each time step $\timesym$, (3) the incurred latency $\lossiter$ on each edge at each time step $\timesym$, and (4) the incurred stage cost $\stateiter^\top Q \stateiter + \controliter^\top R \controliter, t = 0, \dots, T-1$ and the terminal cost $\state_T^\top Q_f \state_T$.
\begin{enumerate}
    \item \textbf{Varying $A$ matrices in the dynamics:} To see the differences in changing $A$, we compare figure \eqref{fig:A1:3_Q111_R0_gamma0.5} and figure \eqref{fig:A111_Q111_R0_gamma0.5}.
    \begin{itemize}
        \item It can be observed that in both scenarios, the controlled system converges to its steady state $\state\optimal = (1/3, 1/3, 1/3)^\top$ in one step. The numerical results suggest that with the choice of cost matrices being $Q = Q_f = I_3, R = 0$ and the specific setup of other parameters in the numerics, the steady state $\state\optimal$ coincides with the Nash equilibrium in the parallel network with latency functions $l_1(y) = l_2(y) = l_3(y) = y$. 
        \item Specifically, the fact that the state $\mathbf{x}_t$ converges in one step to the Nash equilibrium with $A = \begin{pmatrix}
         \frac{1}{3} & \frac{1}{3} & \frac{1}{3} \\
         \frac{1}{3} & \frac{1}{3} & \frac{1}{3} \\
         \frac{1}{3} & \frac{1}{3} & \frac{1}{3}
    \end{pmatrix}$ agrees with our analysis in property (\ref{1/N_A}).
        \item The polyhedral partitions of the feasible state space $\flowset$ are different. In the case of $A = \begin{pmatrix}
         \frac{1}{3} & \frac{1}{3} & \frac{1}{3} \\
         \frac{1}{3} & \frac{1}{3} & \frac{1}{3} \\
         \frac{1}{3} & \frac{1}{3} & \frac{1}{3}
    \end{pmatrix}$ there is no partition of the space, meaning that the optimal controller takes the same affine function over $\flowset$. In the case of $A = I_3$, the feasible state space is partitioned into four polyhedral regions, within each taking different expression of affine optimal controllers.
    \end{itemize}
    \item \textbf{Varying $\gamma$ in the dynamics:} To see the differences in changing $\gamma$, we compare figure \eqref{fig:A111_Q124_R0_gamma0.5} and figure \eqref{fig:A111_Q124_R0_gamma0.7}.
    \begin{itemize}
        \item Both controlled systems converge to the steady state $\state\optimal = (4/7, 2/7, 1/7)^\top$. The numerical results suggest that with the choice of cost matrices being $Q = Q_f = \begin{pmatrix}
         1 & 0 & 0 \\
         0 & 2 & 0 \\
         0 & 0 & 4
    \end{pmatrix}, R = 0$ and the specific setup of other parameters in the numerics, the steady state $\state\optimal$ coincides with the Nash equilibrium in the parallel network with latency functions $l_1(y) = y, l_2(y) = 2y, l_3(y) = 4y$. 
    \item The polyhedral partitions of the feasible state space $\Delta$ are different in the two cases. We observe that with larger $\gamma = 0.7$ (i.e. the players update their flow allocation considering \textbf{more} their memory than the central decision maker's suggested routing decision), the feasible state space has way more polyhedral partitions. This intuitively means that: if the players weight less the suggestions from the central decision maker, in order for the central decision maker to drive the traffic to a target flow allocation, it will have to design more complex routing strategy based on the actual flow on the network.
    \item The convergence rate with larger $\gamma$ is slower: we see that with $\gamma = 0.5$, the state stabilizes with around 5 time steps, while with $\gamma = 0.7$, the state stabilizes with around 10 time steps. This can be intuitively interpreted as: if the players weight less the suggestions from the central decision maker, the steady state of the system is less controllable and therefore it takes longer for the central decision maker to stabilize the system.
    \end{itemize}
    \item \textbf{Varying initial states $\initstate$:} To see the differences in changing $\initstate$, we compare figure \eqref{fig:A111_Q124_R0_gamma0.5} and figure \eqref{fig:A111_Q124_R0_gamma0.5_initial}.
    \begin{itemize}
        \item Both controlled systems converge to the steady state $\state\optimal = (4/7, 2/7, 1/7)^\top$, which again coincides with the Nash equilibrium in the parallel network with latency functions $l_1(y) = y, l_2(y) = 2y, l_3(y) = 4y$. 
        \item We would like to point out that with $\math{x}_0 = [0,1,0]^\top$, the state of the system starts further away from its steady state, and starts within a different polyhedron from where the steady state is located. However with the specific control dynamics in the numerical experiment, the central decision maker still manages to steer the system to the target flow allocation.
    \end{itemize}
    \item \textbf{Varying cost functions:} To see the differences in changing the cost matrices, we compare figure \eqref{fig:A111_Q111_R0_gamma0.5} and figure \eqref{fig:A111_Q124_R0_gamma0.5}.
    \begin{itemize}
        \item Both controlled systems converge, but to the different steady states. More specifically, with $Q = Q_f = I_3$, the steady state is $\state\optimal = (1/3, 1/3, 1/3)^\top$, which coincides with the Nash equilibrium in the parallel network with latency functions $l_1(y) = l_2(y) = l_3(y) = y$; with $Q = Q_f = \begin{pmatrix}
         1 & 0 & 0 \\
         0 & 2 & 0 \\
         0 & 0 & 4
    \end{pmatrix}$, the steady state is $\state\optimal = (4/7, 2/7, 1/7)^\top$, which coincides with the Nash equilibrium in the parallel network with latency functions $l_1(y) = y, l_2(y) = 2y, l_3(y) = 4y$.
    \item This justifies the capability of the central decision maker to design different objective functions and steer the controlled system to different target flow allocations.
    \end{itemize}
\end{enumerate}





\textbf{Reliability of the solver:} with the following setting, we show that it is important to set the time horizon $T$ to be large enough so that the algorithm gives the steady state solution. \\

Let
\begin{linenomath*}
\begin{align*}
 Q = Q_f = \begin{pmatrix}
         1 & 0 & 0 \\
         0 & 2 & 0 \\
         0 & 0 & 4
    \end{pmatrix},
    R = \begin{pmatrix}
         0 & 0 & 0 \\
         0 & 0 & 0 \\
         0 & 0 & 0
    \end{pmatrix},
A =& \begin{pmatrix}
         1 & 0 & 0 \\
         0 & 1 & 0 \\
         0 & 0 & 1
    \end{pmatrix},
    B = \begin{pmatrix}
         \frac{1}{2} & \frac{1}{2} & 0 \\
         0 & \frac{1}{2} & \frac{1}{2} \\
         \frac{1}{2} & 0 & \frac{1}{2}
    \end{pmatrix},
    \\
    &\gamma = 0.6, \initstate = \begin{pmatrix}
    0.3&0.5&0.2\end{pmatrix}^\top
\end{align*}
\end{linenomath*}
If we set the time horizon $T = 15$, we observe in figure \eqref{fig:Non_coverge} that the control system can be oscillating and non-stable, and does not converge to a steady state. However if we set a larger $T = 35$, we see in figure \eqref{fig:coverge} that the controlled system is stabilizing -- the trajectory of the state converges to a steady state.
\begin{figure}[h]
\includegraphics[width=8cm]{figures/No_conv_traj.png}
\includegraphics[width=8cm]{figures/No_conv_panel.png}
\caption{Identity $A$, $B =\begin{pmatrix}
         1/2 & 1/2 & 0 \\
         0 & 1/2 & 1/2 \\
         1/2 & 0 & 1/2
    \end{pmatrix}$, $Q=Q_f=\mathrm{diag}(1,2,4),\gamma=0.6$, $T = 15$. "*" denotes the initial state.}
\label{fig:Non_coverge}
\end{figure}
\\

\begin{figure}[h]
\includegraphics[width=8cm]{figures/Conv_traj.png}
\includegraphics[width=8cm]{figures/Conv_panel.png}
\caption{Identity $A$, $B =\begin{pmatrix}
         1/2 & 1/2 & 0 \\
         0 & 1/2 & 1/2 \\
         1/2 & 0 & 1/2
    \end{pmatrix}$, $Q=Q_f=\mathrm{diag}(1,2,4),\gamma=0.6$, $T = 35$. "*" denotes the initial state.}
\label{fig:coverge}
\end{figure}

%\begin{itemize}
%    \item Results
%    \begin{itemize}
%        \item Nash equilibrium? We only have one player at the entry route. (Q and $Q_f$ corresponds to Rosenthal potential by design) 
%        \item Other 
%    \end{itemize}
%    \item Specific results and algos.
%    \begin{itemize}
%        \item 1 shot 
%        \item Other results (non-flow conservation). 
%        \item Bemporad approach (how to solve the algo. Numerically, with LP)
%    \end{itemize}
%\end{itemize}


%\begin{itemize}
%    \item Results
%    \begin{itemize}
%        \item Nash equilibrium? We only have one player at the entry route. (Q and $Q_f$ corresponds to Rosenthal potential by design) 
%        \item Other 
%    \end{itemize}
%    \item Specific results and algos.
%    \begin{itemize}
%        \item 1 shot 
%        \item Other results (non-flow conservation). 
%        \item Bemporad approach (how to solve the algo. Numerically, with LP)
%    \end{itemize}
%\end{itemize}

\section{Conclusion}
This article transformed the dynamic traffic assignment problem into a control theoretic problem, under a simple scenario using a parallel network with affine latency functions on each edge. We started with the routing problem under the repeated game framework, proposed a game design scheme through LQR within the control theoretic framework, and then leveraged control techniques to analyze convergence/stability of the system with special examples. Within our system analysis, we discovered that the design of $A, B$ in the equation of the dynamics could be chosen to be \textit{left stochastic matrices} so that the conservation of flow is guaranteed. Additionally, the suggested routing allocation $\control$ has to be chosen such that the resulting vector is stochastic, disqualifying certain control technique that can be used in this system (i.e. the algebraic Ricatti equation) and requesting the use of others. Using this fact, we designed an algorithmic solution for the optimal control using a multiparametric quadratic programming approach (explicit MPC), generating explicit strategies and geometric plots to visualize the optimal solutions the central decision maker should take at the feasible states of the game. We discussed the impact of each system parameter on the solution and explained that various structures in $A$ will result in different solution requirements for the central decision maker, while the cost function changes the system's steady state, and $\gamma, \initstate$ influence the rate of convergence. Future work includes studying the region of attraction of the LQR routing system via reachability analysis, extending the present work to more complex network structures (beyond the parallel network), generalizing the analysis of the convergence behavior of the LQR routing system beyond the special cases considered in the present work, and leveraging the Reinforcement Learning techniques to approach general routing problems.


%\section{From LQR to RL: Regions of attraction and special strategies}
%\todo[inline]{Do we want to do this?}

% \subsection{Motivations}
% \subsubsection{Reducing traffic congestion.} 
% In many parts of the world, congestion has swelled to be a difficult dilemma \cite{Teodorovic2017}.
% In 2018, INRIX calculated an annual loss of around \$305 billion in the U.S. due to the direct and indirect impacts of congestion on productivity \cite{INRIX}.
% Left unattended, congestion can amplify the complications that currently come along with it, which include but are not limited to wasted time, excessive noise, unnecessary fuel consumption, and increased greenhouse gas emissions \cite{barth2009traffic}. 
% Researchers and practitioners have tried many ways to reduce fuel consumption and greenhouse gas emissions by improving the quality of vehicles themselves, but this only makes congestion more bearable without solving the problem itself \cite{barth2009traffic}.
% %Many ways that people have tried to reduce fuel consumption and greenhouse gas emissions involve improving the quality of vehicles themselves, but this only makes congestion more bearable without solving the problem itself \cite{barth2009traffic}.

% \subsubsection{The need of models to perform traffic estimation using new data sources.}

% With the rise of smart phones and cloud computing, 
% %there has been a dramatic increase in the number of traffic data sources.
% traditional traffic management has been outpaced by new mobility services, such as transportation network companies and navigational apps \cite{cabannes2018impact}.
% Consequently, current research aims to improve traffic models by leveraging new mobility services, such as real-time, GPS-based, point-speed data from mobile devices \cite{patire2015much}.
% Even so, the data sources required for current traffic models are challenging to collect, as current traffic models need trajectory data, yet traffic data are mainly available as cross-sectional data.
% Therefore, this article focuses on developing Markov chain-based models to utilize link flow data more effectively.

% \subsubsection{Opportunities to improve traffic flow control through network connectivity.}
% Real-time traffic predictions can help reduce congestion by improving traffic control strategies \cite{crisostomi2011google}.
% Additionally, traffic control systems could benefit from the use of navigational apps and autonomous vehicles \cite{wu2017flow}.
% However, controlling every vehicle can be expensive and may lead to ethical issues.
% Therefore, this article considers network traffic control strategies based on controlling vehicle split ratios at every intersection.
% Such a decentralized structure allows for massive parallelization: at every intersection, traffic control can be applied through infrastructure-to-vehicle communications independent of other intersections, which is a significant computational advantage.

% \subsection{Contributions}
% \subsubsection{Markov chains to model traffic assignment}
% In this article, Markov chains are used to model network traffic equilibrium flow.
% This is claimed to be similar to Google's use of Markov chains to model internet congestion in \cite{langville2011google}. 
% In the Markovian traffic assignment framework, transition matrices are used to derive traffic flow allocations. 
% More specifically, for any vehicle arriving at an intersection, the transition matrix indicates its probability to go on any downstream road segments from its current road segment.
% Using the law of large numbers, each element of the transition matrix can be seen as the flow split ratio of every intersection.
% Therefore, Markov chains can extend the static traffic assignment: the Markovian traffic assignment framework.

% \subsubsection{Key contributions}
% The key contributions of the article include:
% \begin{itemize}
% \item \underline{Framing the static traffic assignment into an equivalent Markov chain framework.}
% The classic static traffic assignment (STA) is reframed into an optimization problem on a transition matrix instead of path flows.
% At each intersection, incoming flows are split among the downstream roads according to the split ratios given by the transition matrix of the network.
% This reformulation can be seen as an Eulerian formulation of a Lagrangian problem using fluid mechanics concepts \cite{zhang2007comparison}.

% % Flows arriving at every intersections are split into flows departing from the intersections following the split ratios given by the transition matrix of the network.
% % This helps better calibrate and validate the Markovian model with the available data.
% % Thus, only link flow data are required by the model, and that data can be collected from detectors. 
% % On the other hand, calibrating and validating the classic static traffic assignment needs path flow data, which would be expensive to perform on large networks.
% % Additionally, vehicle identification is necessary to collect path flow data, so the classic STA would be expensive to perform.

% \item \underline{Extending the Markov chain to the dynamic traffic assignment.}
% The Markovian traffic framework is extended to the dynamic traffic assignment using the microscopic simulator SUMO. 
% A benchmark network composed of five links connected by two branches and one merge is set up in SUMO. 
% Every vehicle path is generated by following the probabilities given by the transition matrix of the Markovian framework.

% \item \underline{Learning optimal routing behavior with the dynamic Markovian framework.}
% We demonstrate how to optimize the traffic flow allocation under the Markovian framework in a case study. To begin, three reward functions -- network outflow, total vehicle hours of travel, and average marginal regret -- are designed to measure the effectiveness of traffic flow allocations. 
% Next, grid search, random search, and evolution strategies are performed on the transition matrix to optimize routing behaviors based on the simulation data collected from SUMO. 
% The results show that those three methods are comparable in the case study under all three rewards.



% % \item \underline{Demonstrating the efficiency of the Markovian framework on traffic control.} 
% % For the dynamic traffic case, we perform microscopic simulations using SUMO to show that control system is efficient on the transition matrix framework. The attempt to effectively compute optimal dynamic flow allocation with the help of SUMO gives us confidence in ability to scale up the control to larger system for future research. 
% % \todoJ{Finish this paragraph}
% % \begin{itemize}
% %     \item The attempt to compute optimal dynamic flow allocation with the help of SUMO simulation makes us confidant in ability to scale up the control to larger system for future research.
% %     \begin{itemize}
% %         \item With the transition matrix, we are able to perform dimensionality reduction which explores \dots
% %         \item No need of centralization
% %         \item More resilient and reliable (no overfit, less sensitive  to outliers)
% %     \end{itemize}
% %     \item Results show \dots
% % \end{itemize}
% \end{itemize}

% \subsection{Outline}
% This article first explains the classic traffic assignment \cite{patriksson} and introduces the Markovian static traffic assignment in Section ``Traffic Assignment Dynamics''.
% Second, in order to compare both models, optimal flow allocations are defined according to the notions of user equilibrium and social optimum in Section ``Optimal Static Flow Allocation''.
% Next, the Markovian framework is extended to dynamic traffic assignment with the help of SUMO to compute the flow allocations using transition matrices in Section ``Dynamic Traffic Assignment.''
% In Section ``Learning Optimal Flow Allocation'', we search the decision space of constructed dynamic traffic assignment scenario through grid search, random search, and evolution strategies.


% % In order to better understand the property of problems, a benchmark is created by grid search method.
% % Then, random-search and evolution strategies for analysis are run for analysis. 
% % Benchmark network example gives us confidence on the relevance to learn optimal flow split ratio instead of optimal path flow allocation, while Markov chain theory supports the ability to scale-up such traffic control scheme to bigger networks.


% \section{Traffic assignment dynamics}\label{sec:sta_framework}
% This section introduces the static traffic assignment framework \cite{patriksson} and an equivalent Markovian framework \cite{crisostomi2011google}.
% In the Markovian framework, computation of the optimal link flow allocation is done using transition matrices.
% This bypasses the need of calculating path flows in the static traffic assignment which can be computationally expensive.

% \subsection{Notations}
% This section defines a network, or graph, $\G$ which is composed of nodes, or vertices, $\N$ joined by links, or edges, $\L$.
% The network is assumed to be strongly connected, and the set of paths without cycles is defined as $\P$. 
% For each path $\p$, the flow on the path is denoted as $\hp$. 
% For each link $\l$, the flow on the link is denoted as $\fl$.
% Given a demand matrix $\de$, which indicates the flows that enter and leave the network at each node, we denote the set of feasible path flow allocations as $\Hd$.
% The following notations and definitions are derived from \cite{patriksson}.

% \begin{definition}[Network, paths, and demand]\label{defi:graph}
% Given a finite strongly connected directed graph $\G$ with nodes set $\N$ and links set $\L\subset \N \times \N$, i.e. $\G = (\N, \L)$, for each origin $\o\in\N$ and destination $\d\in\N$:
% \begin{itemize}
% \item Let $\Pod$ be the set of feasible paths without cycles from $\o$ to $\d$.
% \item Let $\dod\geq0$ be the total number of vehicles that make the journey $\o \to \d$, per unit of time. We denote the demand matrix $\de=(\dod)_{\o,\d\in\N}$.
% \end{itemize}
% \end{definition}
% For all of the following definitions and sections, $\G$ is assumed to be given and strongly connected.
% Therefore, for the sake of redundancy, this fact will not be restated every time.

% \begin{remark}[Tails and heads of links]
% For any link $\l\in\L\subset\N\times\N$, because $\L\subset\N\times\N$, there exists unique $t,h\in\N$ such that $\l=(t,h)$.
% We refer to $t$ as the tail of $\l$, and to $h$ as the head of $\l$.
% \end{remark}

% \colorbegin
% We will use the diamond network as a benchmark network to illustrate definitions and notations. Assume that node A is the origin, node D is the destination, and let demand be $\d_{AD}$. This network is shown in Figure~\ref{fig:diamond_network}.
% \begin{figure}[h]
%     \centering
%     \begin{tikzpicture}
%     \tikzset{vertex/.style = {shape=circle,draw,minimum size=1.5em}}
%     \tikzset{edge/.style = {->,> = latex'}}
%     % vertices
%     \node[vertex] (A) at  (0,0) {A};
%     \node[vertex] (B) at  (3,1.5) {B};
%     \node[vertex] (D) at  (6,0) {D};
%     \node[vertex] (C) at  (3,-1.5) {C};
%     %edges
%     \path[->] (A) edge node[above] {$AB$} (B);
%     \path[->] (A) edge node[below] {$AC$} (C);
%     \path[->] (B) edge node[left] {$BC$} (C);
%     \path[->] (B) edge node[above] {$BD$} (D);
%     \path[->] (C) edge node[below] {$CD$} (D);
%     \path[->] (D) edge[bend left = 100] node[below] {$DA$} (A);
%     \end{tikzpicture}
%     \caption{Benchmark network to illustrate definitions and notations.}
%     \label{fig:diamond_network}
% \end{figure}

% Using the network from Figure~\ref{fig:diamond_network}, we have:
% \begin{align*}
%     \N &= \{A,\  B,\  C,\  D\} \\
%     \L &= \{DA,\  AB,\  AC,\  BC,\  BD,\  CD \} &&& \text{ where } DA=(D,A),\ AB=\dots\\
%     \P_{AD} &= \{ABD,\  ABCD,\  ACD\}
%     &&& \text{ where } ABD=(AB,BD),\ ABCD=\dots
%     \\
%     \de &= \begin{pmatrix}
%     0 &0 &0 &d_{AD} \\
%     0 &0 &0 &0 \\
%     0 &0 &0 &0 \\
%     0 &0 &0 &0
%     \end{pmatrix}
% \end{align*}
% \colorend

% \begin{definition}[Path flows, feasible path flow allocation]\label{defi:path_flow}\
% For each path $\p\in\P=\bigcup\limits_{\o,\d\in\N}\Pod$:
% \begin{itemize}
%     \item let $\hp$ be the path flow of path $\p$: the number of vehicles using path $\p$ per unit of time. We denote the path flow vector $\hv=(\hp)_{\p\in\P}$.
% \end{itemize}
% Given a demand matrix $\de\in\R_{+}^{|\N|\times|\N|}$:
% \begin{itemize}
%     \item let $\Hd=\left\{\hv,\
%     \p\in\P:\hp\in\R_{+},\ \o,\d\in\N: 
%     \sum\limits_{\p\in\Pod}\hp=\dod\right\}$ be the set of feasible path flow allocations.
% \end{itemize}
% \end{definition}

% \colorbegin
% In Figure~\ref{fig:diamond_network}, a path flow allocation $\hv=(\hp)_{\p\in\P}$ is feasible if and only if: $h_{ABD} + h_{ABCD} + h_{ACD} = d_{AD}$.
% \colorend

% \begin{definition}[Link flows]\ 

% \begin{itemize}
%     \item For each link $\l\in\L$, let $\fl$ be the link flow of $\l$: the number of vehicles using link $l$ per unit of time.
%     \item We denote the link flow vector $\fv=(\fl)_{\l\in\L}$.
% \end{itemize}
% \end{definition}

% \subsection{Static traffic assignment notation}
% In this section, we define the static traffic assignment assumption that will be relaxed in the section ``Dynamic traffic assignment using SUMO''.
% Following definitions from \cite{patriksson}, link travel times $\tl$ and path travel times $\cp$ are defined.
% Assuming stationary conditions (which are reasonable for periods of time where demand is quasi-static), the link flow allocation $\fv$ can be derived from the path flow allocation $\hp$ using the incidence matrix $\Delta$: $\fv=\Delta \hv$. Similarly, $\cp=\Delta^\top \tv$.

% \begin{definition}[Incidence matrix]\ 

% \begin{itemize}
%     \item For each path $\p\in\P$ and link $\l\in\L$, we define $\depl = \begin{cases} 1 & \text{if } \l\in\p \\ 0 & \text{otherwise} \end{cases}$. 
%     \item We denote $\dep = (\depl)_{\l\in\L}$ the indicator vector of the links included in path $\p$.
%     \item We denote $\Delta = (\depl)_{\l\in\L, \p\in\P}$ the incidence matrix.
% \end{itemize}
% \end{definition}

% \colorbegin
% On the benchmark network of Figure~\ref{fig:diamond_network}, considering $\P=\P_{AD}$, we have:
% \begin{align*}
%     \Delta &= \begin{pmatrix}
%     0 & 0 & 0\\
%     1 & 1 & 0\\ 
%     0 & 0 & 1\\ 
%     0 & 1 & 0\\ 
%     1 & 0 & 0\\ 
%     0 & 1 & 1
%     \end{pmatrix}
% \end{align*}
% \colorend

% \begin{definition}[Travel time]\ 

% \begin{itemize}
%     \item For each link $\l\in\L$, let $\tl$ be the travel time on link $\l$.
%     \item We denote the link travel time vector $\tv=(\tl)_{\l\in\L}$.
%     \item For each path $\p\in\P$, we define $\cp$ as the travel time on path $\p$ as the sum of the travel times on each link that is included in path $\p$, i.e. $\cp=\dep^\intercal\cdot\tv$.
%     \item We denote the path travel time vector $\cv=(\cp)_{\p\in\P}$.
% \end{itemize}
% \end{definition}

% \begin{definition}[Static model, feasible link flow allocation]\label{defi:feasible_flow}
% Static equilibrium conditions are assumed.
% Therefore, for any path $\p$, $\hp$ remains constant over time and $\fv=\Delta\hv$.

% Given a demand matrix $\de\in\R_{+}^{|\N|\times|\N|}$, let $\Fd=\left\{\Delta\hv,\ \hv\in\Hd\right\}$ be the set of feasible link flow allocations.
% \end{definition}

% \begin{definition}[Separability of travel time, travel time function]\label{defi:separability}
% For each $\l\in\L$, $\tl$ is (only) a function of $\fl$: $\tl(\fl)$. We assume that for each $\l\in\L$, $\tl$ is a strictly increasing function, and is positive for $\fl\geq 0$.
% We denote $\tv(\fv)=(\tl(\fl))_{\l\in\L}$.

% For every link flow allocation $\fv\in\Fd$, the travel time of each path $\p\in\P$ is $\cp(\fv)=\dep^\intercal\cdot\tv(\fv)$.
% \end{definition}

% \subsection{Markovian framework for static traffic assignment}
% In this section, the Markovian framework, inspired by \cite{crisostomi2011google, zhao2018markovian}, is presented.
% First, the line graph $\LG$ is defined as the graph where the roles of nodes and links in $\G$ are swapped.
% Next, based on the adjacency matrix of $\LG$, the transition matrix $\Pr$ -- a type of stochastic matrix \cite{Gagniuc2017} -- gives the transition probabilities to go from any link $\l$ to its downstream links.
% Equilibrium flows (in the context of Markov chains) are then defined using the transition matrix $\Pr$ and the demand matrix $\de$.


% \subsubsection{Definitions}
% % First, the concept of line graphs \cite{Godsil2001algebraic} is defined such that for the line graph $\LG$ of $\G$, the roles of nodes and links in $\G$ are swapped.
% % Afterwards, stochastic matrices \cite{Gagniuc2017} and transition matrices $\Pr$ are defined.

% \begin{definition}[Line graph \cite{Godsil2001algebraic}]
% The line graph $\LG=(\N_{\LG}, \L_{\LG})$ is the graph formed from swapping the roles of nodes and links in $\G=(\N,\L)$. 
% Each link in $\G$ is represented as a node in $L(\G)$: $\N_{\LG} = \L$, 
% % and each intersection of two links in $\G$ is a link in $L(\G)$.
% and each pair of links $(\l_1,\l_2)$ in $\G$ such that the head of $\l_1$ is the tail of $\l_2$ is a link in $\LG$.
% \end{definition}

% \begin{remark}[Line graphs vs. dual graphs]
% Such a graph is called a line graph, but some articles -- such as \cite{crisostomi2011google} and \cite{porta2006network} -- use the term dual graph instead. Note that the definition of the dual graph (in \cite{crisostomi2011google} and \cite{porta2006network}) is not equivalent to the definition of dual graphs from a graph theory point of view, where the faces in the original graphs are nodes in the dual graph.
% \end{remark}


% \begin{definition}[Stochastic matrix \cite{Gagniuc2017}]
% For a line graph $\LG$, $S\in\R^{|\L|\times|\L|}$ is defined as a stochastic matrix if and only if:
% \begin{align*}
%     &\forall i,j\in\L, \quad\quad\quad s_{i,j}\geq 0   \\
%     &S \mathbf{1} = \mathbf{1} \\
%     &\forall i,j\in\L, \quad\quad\quad s_{i,j}\neq 0 \implies (i,j)\in\L_{\LG}
% \end{align*}
% \end{definition}

% \begin{definition}[Transition matrix \cite{langville2011google}]
% For a line graph $\LG$, $\Pr\in\R^{|\L|\times|\L|}$ is defined as a transition matrix if and only if:
% \begin{align*}
%     &P \text{ is a stochastic matrix}\\
%     &\forall i_1,i_2,\l\in\L,\quad  \pr{i_1,\l} \neq 0 \text{ and } \pr{i_2,\l}\neq 0 \implies \pr{i_1,\l} = \pr{i_2,\l}
% \end{align*}
% We denote $\SPr$ as the set of transition matrices.
% \end{definition}


% \begin{remark}[Line graphs and Markov chains]\label{rem:stochastic_transition}
% The line graph of the network is used because information about flow lies in the road segments (or links of $\G$), not in the actual locations or intersections (or nodes of $\G$). 
% With this setup, well-studied Markov chain properties can be used \cite{Gagniuc2017} to observe how flow shifts from one road to the next at every timestep.

% While stochastic matrices allow any probability distribution from one link to the next, transition matrices assume that if two links $\l_1,\l_2$ share the same head, then the probability to go from $\l_1$ to a downstream link $\l_f$ is the same as the probability to go from $\l_2$ to the same link $\l_f$.
% \end{remark}

% % \todoT{Re-explain remark 4.4 to be more connected to the Dynamic section. Markov process on every vehicle, aggregation to flow -> we can take the expectation using the law of large numbers. That is why we can also see the transition matrix as a split ratio matrix. And do not introduce probabilistic frameworks. This will be later explain definition 4.13. See with remark 4.5}
% \begin{remark}[Markov chain]
% A Markov chain is a stochastic process in which the probability of changing to a state $j$ from state $i$ depends only on the fact that the current state is $i$ \cite{langville2011google}.
% % Markov chain gives that the expected location $l_{t+1}$ of a single vehicle at time $t+1$ can be derived from its location at time $t$ with the transition matrix: $E[l_{t+1}]=\Pr^\top E[l_{t}]$.
% % Aggregating vehicles into flows, and using the law of large numbers, this gives us that the distribution of flows $\fv_{t+1}$ at time $t + 1$ can be computed from the distribution of flows $\fv_t$ at time $t$: $\fv_{t + 1} = \Pr^\top \fv_t$ \cite{langville2011google}.
% % In this case, the set of states is $\N_{\LG}$.
% % Consequently, with the assumption that previously taken roads have no effect in the decision of the next road to take, this presented model is similar to a Markov chain, so several Markov chain properties will be applied in order to find equilibrium flows of networks. 
% % One of these properties is the transition matrix $\Pr$.
% Markov chain theory describes that the transition matrix can be used to compute the expected distribution of flows $\fv_{t+1}$ at time $t + 1$ from the distribution of flows $\fv_t$ at time $t$: $\fv_{t + 1} = \Pr^\top \fv_t$ \cite{langville2011google}.
% % , the transition matrix can be used to show the expected distribution of flows at time $t + 1$. 
% % This relationship is $\fv_{t + 1} = \Pr^\top \fv_t$ \cite{langville2011google}.
% Therefore, transition probabilities can also be seen as split ratios (see definition \ref{defi:transition_dynamics}).
% % For the remainder of the article, only the stationary distribution of the Markov chain will be studied. 
% \end{remark}

% % \begin{remark}[Transition matrix conventions]
% % In some texts using Markov chains, row vectors are used, so if $\Pr$ is the transition matrix and $\mathbf{x}_t$ is the distribution of flow in the network at time $t$ organized in a row vector, then $\mathbf{x}_{t+1} = \mathbf{x}_t P$. 
% % However, for column vectors, we can take the transpose of both sides to get $\mathbf{y}_{t+1} = P^\top \mathbf{y}_t$ for $\mathbf{y}_t := \mathbf{x}_t^\top$ and $\mathbf{y}_{t+1} := \mathbf{x}_{t+1}^\top$.
% % \end{remark}

% \colorbegin
% On the benchmark network (Figure~\ref{fig:diamond_network}), we have that:
% \begin{align*}
%     \N_{\LG} &= \{DA, AB, AC, BC, BD, CD \} = \L\\
%     \L_{\LG} &= \{(DA, AB), (DA, AC), (AB, BD), (AB, BC), (BC, CD), (AC, CD), (BD, DA), (CD, DA)\}\\
%     \Pr &= \begin{pmatrix}
%         0 &\pr{AB} &\pr{AC} &0 &0 &0 \\
%         0 &0 &0 &\pr{BC} &\pr{BD} &0\\
%         0 &0 &0 &0 &0 &\pr{CD}\\
%         0 &0 &0 &0 &0 &\pr{CD} \\
%         \pr{DA} &0 &0 &0 &0 &0 \\
%         \pr{DA} &0 &0 &0 &0 &0 
%     \end{pmatrix}    
% \end{align*}
% The line graph of the benchmark graph and the corresponding transition matrix are shown in Figure~\ref{fig:line_graph} where nodes are in the approximate positions of the links in the benchmark graph. In this case, demand enters at nodes $AB$ and $AC$.

% \begin{figure} [h]
%     \centering
%     \begin{tikzpicture}
%     \tikzset{vertex/.style = {shape=circle,draw,minimum size=1.5em}}
%     \tikzset{edge/.style = {->,> = latex'}}
%     % vertices
%     \node[vertex] (AB) at  (1,1) {AB};
%     \node[vertex] (AC) at  (1,-1) {AC};
%     \node[vertex] (BC) at  (3,0) {BC};
%     \node[vertex] (BD) at  (5,1) {BD};
%     \node[vertex] (CD) at  (5,-1) {CD};
%     \node[vertex] (DA) at  (3,-3) {DA};
%     %edges
%     \path[->] (AB) edge node[below] {$\pr{BC}$} (BC);
%     \path[->] (AB) edge node[above] {$\pr{BD}$} (BD);
%     \path[->] (AC) edge node[below] {$\pr{CD}$} (CD);
%     \path[->] (BC) edge node[above] {$\pr{CD}$} (CD);
%     \path[->] (BD) edge[bend left = 100] node[right] {$\pr{DA}$} (DA);
%     \path[->] (CD) edge node[left] {$\pr{DA}$} (DA);
%     \path[->] (DA) edge node[right] {$\pr{AC}$} (AC);
%     \path[->] (DA) edge[bend left = 100] node[left] {$\pr{AB}$} (AB);
%     \end{tikzpicture}
%     \caption{The line graph of the benchmark network.}
%     \label{fig:line_graph}
% \end{figure}
% \colorend

% \subsubsection{Static equilibrium using Markov chains}
% Flow movement through networks is described using previously defined line graphs and transition matrices.
% Transition probabilities, or split ratios, are defined as elements of transition matrices.
% Then, using the concept of flow conservation, equilibrium flow can be defined using ideas analogous to limits of Markov chains.
% This is useful later to reframe the current static traffic assignment framework using transition matrices.

% % \todoT{We are here in the careful proofread.}
% \begin{definition}[Transition probability]
% For a transition matrix $\Pr\in\SPr$, we define $\pr{i,\l}$ for every link $i\in\L$ and $\l\in\L$ as the transition probability to go from the link $i$ to the link $\l$.

% Note that, if there is no connection between the two links (i.e.\ $(i,\l)\in\L_{\LG}$), then $\pr{i\l}=0$.

% Because, $\Pr$ is a transition matrix, $\forall i_1,i_2,\l\in\L$, such that $\pr{i_1,\l} \neq 0$ and $\pr{i_2,\l} \neq 0$ implies $\pr{i_1,\l} = \pr{i_2,\l}$ (definition), and $\exists i\in\L $ such that $\pr{i,\l}\neq 0$ ($\Pr\mathbf{1}=\mathbf{1}$), we can uniquely define $\prl=\pr{i,\l}$ (c.f. remark \ref{rem:stochastic_transition}).

% We call $\prl$ the transition probability of the link $\l$.
% \end{definition}

% \paragraph{Node dynamics}\ 

% At a specific node $\n$ of the network $\G$, the conservation flow inside the network tells that the total inflow of vehicles arriving at the node $\n$ added with the demand that arrives at the node is equal to the total outflow of vehicles departing from the node $\n$ added with the demand that exits at the node.

% This can be summarized into one equality:

% \begin{definition}[Flow conservation]\label{defi:flow_conservation}
% Given a demand $\de\in\R_{+}^{|\N|\times|\N|}$, a link flow allocation $\fv$ satisfies the flow conservation if for every node $\n\in\N$:
% \begin{equation*}
%     \sum_{u, (u,\n)\in \L}f_{u, \n} + 
%     \sum_{\tilde{u}\in\N}d_{\n,\tilde{u}} = 
%     \sum_{v, (\n, v)\in \L}f_{\n, v} + 
%     \sum_{\tilde{v}\in\N}d_{\tilde{v},n}
% \end{equation*}
% \end{definition}

% % \begin{figure} [h]
% %     \centering
% %     \begin{tikzpicture}
% %     \tikzset{vertex/.style = {shape=circle,draw,minimum size=1.5em}}
% %     \tikzset{edge/.style = {->,> = latex'}}
    
% %     % vertices
% %     \node[vertex] (n) at  (0,0) {n};
    
% %     %edges
% %     \path[->] (-2, 1) edge node[above left = 0.5] {$\sum_{u, (u,\n)\in \L}f_{u, \n}$} (n);
% %     \path[->] (-2, 0) edge node[left = 0.75] {$\sum_{\tilde{u}\in\N}d_{\n\tilde{u}}$} (n);
% %     \path[<-] (2, 1) edge node [above right = 0.5] {$\sum_{w, (\n w)\in \L}f_{\n w}$} (n);
% %     \path[<-] (2, 0) edge node[right = 0.75] {$\sum_{\tilde{w}\in\N}d_{\tilde{w}n}$} (n);

% %     \end{tikzpicture}
% %     \caption{The intuition behind definition \ref{defi:flow_conservation}. At the node $\n\in\N$ the in-flow ($\sum_{u, (u,\n)\in \L}f_{u, \n}$) and the demand that enter in the network ($\sum_{\tilde{u}\in\N}d_{\n,\tilde{u}}$) is equal to the out-flow ($\sum_{w, (\n, w)\in \L}f_{\n, w}$) and the demand that exit the network ($\sum_{\tilde{w}\in\N}d_{\tilde{w},n}$).}
% %     \label{fig:network}
% % \end{figure}

% \begin{property}[Flow conservation]\label{prop:flow_conservation}
% Given a demand $\de\in\R_{+}^{|\N|\times|\N|}$, if a link flow allocation $\fv$ is feasible (i.e.\ $\fv\in\Fd$) then $\fv$ satisfies the flow conservation.
% \end{property}
% \colorproof
% \proof{
% The proof can be done by showing that:
% \begin{align*}
%      \sum_{u, (u,\n)\in \L}
%      \sum_{v, (\n, v)\in \L}
%      \sum_{\p\in\P} 
%      \hp\delta_{\p, (u,\n)}\delta_{\p, (\n,v)}
%      &= \sum_{u, (u,\n)\in \L}f_{u, \n} - \sum_{\tilde{v}\in\N}d_{\tilde{v},n}
%      \\
%      \text{and} \quad \quad \quad \quad \quad 
%      &= \sum_{v, (\n, v)\in \L}f_{\n, v}
%      - \sum_{\tilde{u}\in\N}d_{\n,\tilde{u}}
%      \\
%      \text{which shows that } \quad 
%      \sum_{u, (u,\n)\in \L}f_{u, \n} + \sum_{\tilde{u}\in\N}d_{\n,\tilde{u}} &= \sum_{v, (\n, v)\in \L}f_{\n, v} + \sum_{\tilde{v}\in\N}d_{\tilde{v},n}
% \end{align*}
% }
% \colorend 

% \colorbegin
% On the benchmark network example (Figure~\ref{fig:diamond_network}), for the node $B$, we have:
% \begin{align*}
%     \sum_{u, (u, B)\in \L}
%      \sum_{v, (B, v)\in \L}
%      \sum_{\p\in\P} 
%      \hp\delta_{\p, (u,B)}\delta_{\p, (B,v)}
%      = 
%      \delta_{AB, ABD} \delta_{BC, ABD} h_{ABD} &+  
%      \delta_{AB, ABD} \delta_{BD, ABD} h_{ABD} \\ +
%      \delta_{AB, ABCD} \delta_{BC, ABCD} h_{ABCD} &+
%      \delta_{AB, ABCD} \delta_{BD, ABCD} h_{ABCD} \\ +
%      \delta_{AB, ACD} \delta_{BC, ACD} h_{ACD}  &+
%      \delta_{AB, ACD} \delta_{BD, ACD} h_{ACD} \\
%      = \delta_{AB, ABD} h_{ABD} + 
%      \delta_{AB, ABCD}  h_{ABCD} = f_{AB} \quad \quad \quad \quad \;\;& \\
%     =  \delta_{BC, ABD} h_{ABD} + \delta_{BC, ABCD} h_{ABCD}
%     + \delta_{BD, ABD} h_{ABD} + &\delta_{BD, ABCD} h_{ABCD}
%     = f_{BC} + f_{BD}
% \end{align*}
% So this gives that $f_{AB}=f_{BC}+f_{BD}$.
% \colorend

% \paragraph{Equilibrium flow}\ 

% Using the flow conservation property and transition probabilities, equilibrium flow allocations can now be defined.
% In fact, it can be shown that the equilibrium flow allocation is a solution to a linear equation involving the transition matrix.

% \begin{definition}[Transition dynamics]\label{defi:transition_dynamics}
% Given a transition matrix $\Pr\in\SPr$ and demand $\de\in\R_{+}^{|\N|\times|\N|}$, a link flow allocation $\fv\in\R^{|\L|}$ is defined as an equilibrium flow allocation if:
% \begin{enumerate}
%     \item $\fv$ satisfies the flow conservation (definition \ref{defi:flow_conservation})
%     \item For every node $\n\in\N$ and every link $\l\in\L$ that has tail $\n$ ($\exists m\in\N$ such that $\l=\n m$), $\fl = \prl f_{\n, out}$, with $f_{\n, out} = \sum_{w, (\n, w)\in \L}f_{\n, w}$
%     \item $\fv\geq 0$
% \end{enumerate}

% \end{definition}

% \begin{notation}[Set of equilibrium flow]Given a transition matrix $\Pr\in\SPr$ and demand $\de\in\R_{+}^{|\N|\times|\N|}$, $\Fdp$ is denoted as the set of equilibrium flows.

% \end{notation}

% \begin{notation}[Origin probability $\Pr_\o$]
% Given $\Pr \in \SPr $, we denote:
% $\Pr_\o = [\Pr_{\o_{\l,\n}}]_{\l\in\L, \n \in \N}$,

% \noindent
% where $\Pr_{\o_{\l,\n}} = 
% \begin{cases} 
%     \prl & \text{if $\l$ has $\n$ for tail}\\
%     0 & \text{else}
% \end{cases}$.
% \end{notation}

% \colorbegin
% For the network described in Figure~\ref{fig:diamond_network}, we have:
% \begin{align*}
%     \Pr_\o = \begin{pmatrix}
%     0 &0 &0 &\pr{DA} \\
%     \pr{AB} &0 &0 &0 \\
%     \pr{AC} &0 &0 &0 \\
%     0 &\pr{BC} &0 &0 \\
%     0 &\pr{BD} &0 &0 \\
%     0 &0 &\pr{CD} &0
%     \end{pmatrix}
% \end{align*}
% \colorend
    
% \begin{property}[Equilibrium flow]\label{defi:eq_flow}
% For a transition matrix $\Pr\in\SPr$, and demand $\de\in\R_{+}^{|\N|\times|\N|}$, $\fv$ is an equilibrium flow if and only if:
% \begin{enumerate}
%     \item[a.] $\fv=\Pr^\top \fv + \Pr_\o(\de - \de^\top)\mathbf{1}$
%     \item[b.] $\fv_l \geq 0 \ \forall l \in \L$ 
% \end{enumerate}
% \end{property}
% \colorproof
% \proof{
% Let $\fv$ be an equilibrium flow, $\n\in\N$, and $\l\in\L$ which has tail $\n$.
% 2. from definition \ref{defi:transition_dynamics} gives that $\fl = \prl f_{\n, out} = \prl \sum_{v, (\n, v)\in \L}f_{\n, v}$.
% 1. from definition \ref{defi:transition_dynamics} gives that $\sum_{v, (\n, v)\in \L}f_{\n, v} = \sum_{u, (u, \n)\in \L} f_{u, \n} + \sum_{\tilde{u}\in\N}d_{\n,\tilde{u}} - \sum_{\tilde{v}\in\N}d_{\tilde{v},n}$.

% Therefore, $\fl = \prl\left(\sum_{u, (u, \n)\in \L} f_{u, \n} + \sum_{\tilde{u}\in\N}d_{\n,\tilde{u}} - \sum_{\tilde{v}\in\N}d_{\tilde{v},n}\right)$.
% This is equivalent to the matrix expression: $\fv=\Pr^\top \fv + \Pr_\o(\de - \de^\top)\mathbf{1}$.
% }
% \colorend

% \colorbegin
% As an example, this equation will be applied to the benchmark network in Figure~\ref{fig:diamond_network}.
% The aim is to show that the equation results in the following system of equations:

% \begin{align*} 
%     f_{DA} &= \pr{DA}\left(f_{BD} + f_{CD} - d_{AD} \right) \\
%     f_{AB} &= \pr{AB}\left(f_{DA} + d_{AD} \right) \\
%     f_{AC} &= \pr{AC}\left(f_{DA} + d_{AD} \right) \\
%     f_{BC} &= \pr{BC} f_{AB}  \\
%     f_{BD} &= \pr{BD} f_{AB} \\
%     f_{CD} &= \pr{CD}\left(f_{AC} + f_{BC} \right)
% \end{align*}

% Using $\fv = \Pr^\top \fv + \Pr_\o(\de - \de^\top)\mathbf{1}$:
% \begin{align*}
%     \begin{pmatrix}
%     f_{DA} \\
%     f_{AB} \\
%     f_{AC} \\
%     f_{BC} \\
%     f_{BD} \\
%     f_{CD}
%     \end{pmatrix}
%     &=\begin{pmatrix}
%     \pr{DA}\left(f_{BD} + f_{CD}\right) \\
%     \pr{AB}f_{DA} \\
%     \pr{AC}f_{DA} \\
%     \pr{BC}f_{AB} \\
%     \pr{BD}f_{AB} \\
%     \pr{CD}\left(f_{AC} + f_{BC}\right)
%     \end{pmatrix} +
%     \begin{pmatrix}
%     -\pr{DA}d_{AD} \\
%     \pr{AB}d_{AD} \\
%     \pr{AC}d_{AD} \\
%     0 \\
%     0 \\
%     0
%     \end{pmatrix} =
%     \begin{pmatrix}
%     \pr{DA}\left(f_{BD} + f_{CD} - d_{AD} \right) \\
%     \pr{AB}\left(f_{DA} + d_{AD} \right) \\
%     \pr{AC}\left(f_{DA} + d_{AD} \right) \\
%     \pr{BC} f_{AB}  \\
%     \pr{BD} f_{AB} \\
%     \pr{CD}\left(f_{AC} + f_{BC} \right)
%     \end{pmatrix}
% \end{align*}
% \colorend


% \begin{remark}[Equilibrium flow]\label{rem:equilibrium_flow}
% The equilibrium flow can be seen as the stationary distribution of the Markov chain described by $\Pr$ with the additional term $\Pr_\o(\de - \de^\top)\mathbf{1}$ that encodes the demand.
% Furthermore, the stationary distribution of a Markov chain can be seen as the limit of the Markov chain described by $\Pr$ as time goes to infinity \cite{Gagniuc2017}.
% % However, the current framework is a little bit different than a Markov chain because of the term $\Pr_\o(\de - \de^\top)\mathbf{1}$. And because the evolution of flow among the network is a more complicated than $\fv_{t+1}=\Pr^\top\fv_{t}+\Pr_\o(\de - \de^\top)\mathbf{1}$
% \end{remark}



% \begin{property}[Existence of an equilibrium flow]\label{prop:existence_markov}
% There is at least one equilibrium flow: 
% \[\forall
% \Pr\in\SPr,\
% \forall \de\in\R_{+}^{|\N|\times|\N|}, \quad \Fdp\neq\emptyset\]
% \end{property}
% % \proof{
% % \todoT{Try to better do this proof, and better organize it. It is hard to read right now.}
% % First let's show that $\exists \fv$ such that $\fv=\Pr^\top \fv + (\Pr_O\de - \Pr_O \de^\top)\mathbf{1}$.

% % \noindent
% % $
% % \fv=\Pr^\top \fv + (\Pr_O\de - \Pr_O \de^\top)\mathbf{1}\iff
% % A\fv=b \quad \text{with } A = I -  \Pr^\top \text{ and } b = (\Pr_O\de - \Pr_O \de^\top)\mathbf{1}
% % $.
% % If $b\in Im(A)$ then $\exists \fv^*$ such that $b = A\fv^*$.
% % $b\in Im(A)\iff b \perp N(A^\top)$ because $Im(A)\bigoplus^\perp N(A^\top)$.
% % In our case $N(A^\top) = N(I-\Pr) = Span(\mathbf{1})$ (Perron-Frobenius theorem with a strongly connected graph \cite{Godsil2001algebraic}).
% % So $b\in Im(A) \iff b\perp \mathbf{1} \iff \mathbf{1}^\top b = 1$.
% % In our case, $\mathbf{1}^\top b = \mathbf{1}^\top(\Pr_O\de - \Pr_O \de^\top)\mathbf{1} = (\mathbf{1}^\top\Pr_O\de - \mathbf{1}^\top\Pr_O \de^\top)\mathbf{1} = \mathbf{1}^\top\de\mathbf{1} - \mathbf{1}^\top\de^\top\mathbf{1} = 0$.

% % \noindent
% % So we have that $\exists \fv$ such that $\fv=\Pr^\top \fv + (\Pr_O\de - \Pr_O \de^\top)\mathbf{1}$. We denote $\fv^*$ such link flow allocation.

% % Now, let's show that $\exists \fv$ such that $\fv=\Pr^\top \fv + (\Pr_O\de - \Pr_O \de^\top)\mathbf{1}$ and $\fv \geq 0$.

% % \noindent
% % The set of solution of $A\fv=b$ is $\fv^* + N(A)$.
% % Perron-Frobenius theorem gives that $N(A) = Span(\fv_0)$ with $\fv_0 > 0$ ($\fv_0$ is the stationary distribution of $\Pr$ \cite{Gagniuc2017}).
% % So any $\fv=\fv^*+\alpha \fv_0$ with $\alpha\in\R$ is solution of $A\fv=b$.
% % If we take, $\alpha=\min_{i}\frac{f^*_i}{f_{0,i}}$ then $\fv \geq 0$ and $\fv=\Pr^\top \fv + (\Pr_O\de - \Pr_O \de^\top)\mathbf{1}$.
% % }

% \colorproof
% \proof{
% The proof can be done by sequentially:
% \begin{enumerate}
%     \item Show that $\exists \fv$ such that $\fv=\Pr^\top \fv + \Pr_\o(\de - \de^\top)\mathbf{1}$.
%     \item Show that $\exists \fv$ such that $\fv=\Pr^\top \fv + \Pr_\o(\de - \de^\top)\mathbf{1}$ and $\fv \geq 0$
% \end{enumerate}

% \noindent
% 1. With the notation $A=I-\Pr^\top$ and $b=\Pr_\o(\de - \de^\top)\mathbf{1}$: 
% \begin{align*}
%     \exists \fv, \fv=\Pr^\top \fv + \Pr_\o(\de - \de^\top)\mathbf{1} &\iff \exists x, Ax=b \quad \text{(linear equation)} \\
%     &\iff b\in Im(A) \\
%     &\iff b\perp N(A^\top) \quad (\text{because } Im(A)\oplus^\perp N(A^\top))
% \end{align*}
% In this case, $N(A^\top) = N(I-P) = \text{Span}(\mathbf{1})$ because of the Perron-Frobenius theorem for irreducible matrices \cite{Godsil2001algebraic} (basically because $\Pr \mathbf{1} = \mathbf{1}$ and the graph is strongly connected).
% Therefore:
% \begin{align*}
%     \exists \fv, \fv=\Pr^\top \fv + \Pr_\o(\de - \de^\top)\mathbf{1} &\iff \mathbf{1}^\top b = 0 \\
%     &\iff \mathbf{1}^\top\Pr_\o(\de - \de^\top)\mathbf{1} = 0
% \end{align*}
% However, $\mathbf{1}^\top\Pr_\o = \mathbf{1}$ because of the definition of $\Pr_\o$ and that $\Pr$ is a transition matrix. Hence, $\mathbf{1}^\top\Pr_\o(\de - \de^\top)\mathbf{1} = 0$ and $\exists \fv, \fv=\Pr^\top \fv + \Pr_\o(\de - \de^\top)\mathbf{1}$.

% \ 

% \noindent
% 2. Let note $\fv^*$ as a flow such that $\fv^*=\Pr^\top \fv^* + \Pr_\o(\de - \de^\top)\mathbf{1}$.
% With linear algebra:
% \begin{align*}
%     \{x, Ax=b\} &= \{x, x = \fv^* + y, \text{ with }, y\in N(A)\} = \fv^*+N(A)
% \end{align*}
% The Perron-Frobenius theorem gives the result $N(A)=N(I-\Pr^\top)=\text{Span}(\fv_0)$, with $\fv_0>0$.

% \noindent
% Therefore, $\{\fv, \fv=\Pr^\top \fv + \Pr_\o(\de - \de^\top)\mathbf{1}\} = \{\fv, \fv=\fv^*+\alpha \fv_0, \alpha\in\R\}$.

% \noindent
% Because $\fv_0\geq=0$, then $\Fdp = \{\fv, \fv=\fv^*+\alpha \fv_0, \alpha\in\R\}\cap \{\fv, \fv\geq 0\}\neq \emptyset$.
% }
% \colorend

% \colorbegin
% Now, $\mathbf{1}^\top\Pr_\o(\de - \de^\top)\mathbf{1}=0$ can be shown on the benchmark example in Figure~\ref{fig:diamond_network}. 

% \begin{align*}
%     \mathbf{1}^\top\Pr_\o(\de - \de^\top)\mathbf{1} &=
%     \begin{pmatrix}
%     1 &1 &1 &1 &1 &1
%     \end{pmatrix}
%     \begin{pmatrix}
%     -\pr{DA}d_{AD} \\
%     \pr{AB}d_{AD} \\
%     \pr{AC}d_{AD} \\
%     0 \\
%     0 \\
%     0
%     \end{pmatrix} & \\
%     &= -\pr{DA}d_{AD} + \pr{AB}d_{AD} + \pr{AC}d_{AD} \\
%     &= -d_{AD} + d_{AD} &\text{ since $\left(\pr{AB} + \pr{AC}\right) = 1$}\\
%     &=0
% \end{align*}
% \colorend

% \begin{remark}[Uniqueness of an equilibrium flow, convergence of Markov chain]
% The equilibrium flow is not unique. However, one can fix some conditions on link flows such that the equilibrium flow will be unique and is the limit of the Markov chain described by $\Pr$ (c.f. remark \ref{rem:equilibrium_flow}).

% \colorbegin
% On the benchmark network example (Figure~\ref{fig:diamond_network}), one possible constraint is $f_{DA}=0$. In this case, the equilibrium will be uniquely defined (and will still satisfy $\fv\geq 0$).
% \colorend
% \end{remark}

% \begin{remark}[Feasibility of an equilibrium flow]\label{rem:feasibility_equilibrium}
% An equilibrium flow (definition \ref{defi:eq_flow}) may not be a feasible flow (definition \ref{defi:feasible_flow}). This is due to the potential presence of cycles in the network, which was only accounted for as a constraint such that paths should not have cycles (see Figure~\ref{fig:example_non_feasible}).

% \colorbegin
% However, on the benchmark example, if one imposes the constraint that $f_{DA}=0$, then the equilibrium flow will be feasible.
% \colorend
% \end{remark}


% \colorbegin
% \begin{figure}[ht]
% \centering
% % \begin{tikzpicture}[scale=0.8]
% %     \path
% %     (-3,0) node(A) [circle, draw] {$O$}
% %     (3,0) node(B) [circle, draw] {$D$};
% %     \draw[very thick,->] (A) to [bend left=20] node[above, midway] {$f_{OD}=110$} node[below, midway] {} (B);
% %     \draw[very thick,<-] (A) to [bend right=20] node[above, midway] {} node[below, midway] {$f_{DO}=10$} (B);
% % \end{tikzpicture}
% \begin{tikzpicture}
%     \tikzset{vertex/.style = {shape=circle,draw,minimum size=1.5em}}
%     \tikzset{edge/.style = {->,> = latex'}}
%     % vertices
%     \node[vertex] (A) at  (0,0) {A};
%     \node[vertex] (B) at  (3,1.5) {B};
%     \node[vertex] (D) at  (6,0) {D};
%     \node[vertex] (C) at  (3,-1.5) {C};
%     %edges
%     \path[->] (A) edge node[above] {$110$} (B);
%     \path[->] (A) edge node[below] {$0$} (C);
%     \path[->] (B) edge node[left] {$0$} (C);
%     \path[->] (B) edge node[above] {$110$} (D);
%     \path[->] (C) edge node[below] {$0$} (D);
%     \path[->] (D) edge[bend left = 100] node[below] {$10$} (A);
% \end{tikzpicture}
% \caption{An equilibrium flow which is not feasible. Given a demand of $d_{AD}=100$, the flow described in the figure is an equilibrium flow but is not a feasible flow. For any feasible flow allocation $f_{DA}=0$.}
% \label{fig:example_non_feasible}
% \end{figure}
% \colorend



% \section{Optimal static flow allocation}
% In this section, the user equilibrium and social optimum flow allocation are defined for the classic static traffic assignment \cite{patriksson} and for the Markovian framework.
% In the case of user equilibrium, vehicles are assumed to try to reduce their travel times as much as possible \cite{perederieieva2013computational}.
% Intuitively, this means that at user equilibrium, no user can switch to a different path and reduce his or her travel time \cite{perederieieva2013computational}.
% In the case of the social optimum allocation, the total of all vehicles' travel times in the network is minimized (given a fixed demand).
% Both the user equilibrium and the social optimum, for the classic static traffic assignment framework and the Markovian framework, can be computed as minimization problems.

% \subsection{Static traffic assignment}
% First, recall the classic static traffic assignment user equilibrium and social optimum \cite{patriksson}.
% % Both the user equilibrium and the social optimum can be computed as solution to a minimization problem \cite{Beckmann1956studies, nagurney1998network}.

% \begin{definition}[User equilibrium] Given a traffic demand \de, a path flow allocation $\hv\in\Hd$ is a user equilibrium if and only if:
% \begin{equation*}\label{ue}
% \forall \o,\d\in\N,\ \forall \p\in\Pod,\ \hp\cdot(\cp(\hv)-\min\limits_{\q\in\Pod}\cq(\hv))=0
% \end{equation*}
% \label{def:UE}
% \end{definition}

% \begin{definition}[Social optimum] Given a traffic demand \de, a link flow allocation $\fv\in\Fd$ is a social optimum if and only if:
% \begin{equation*}\label{so}
% \forall \mathbf{g}\in\Fd,\ \tv(\fv)^\top \fv\leq \tv(\mathbf{g})^\top \mathbf{g}
% \end{equation*}
% \label{def:SO}
% \end{definition}

% \begin{remark}[Wardrop's first condition \cite{wardrop1952road}]
% At a \textbf{user equilibrium}, the travel time on all used paths between an origin-destination pair are equal and less than those which would be experienced by a single vehicle on any unused path in the network.
% \end{remark}

% \begin{property}[Minimization problem to compute user equilibrium]\ 
% Any user equilibrium is the solution of the following a convex optimization problem  \cite{Beckmann1956studies, nagurney1998network}:

% \begin{align*}
% \min_{\fv, \hv} \sum_{\l\in\L}\int_0^{\fl}\tl(s)&ds \\
% \text{subject to }
% \sum\limits_{\p\in\P} \depl \hp&=\fl &&& \forall \l\in\L\\
% \sum_{\p\in\Pod}\hp&=\dod &&& \forall \o,\d\in\N\\
% \hp&\geq 0 &&& \forall \p\in\P
% \end{align*}
% This can be written as:
% \begin{align*}
%     \max_{\fv\in { X}} \rew(\fv)
% \end{align*}
% Where ${ X} = \Fd$ and $\rew(\fv) = -\sum_{\l\in\L}\int_0^{\fl}\tl(s)ds$.
% \end{property}

% \begin{property}[Minimization problem to compute social optimum]\ 
% Any user equilibrium is the solution of the following a convex optimization problem \cite{patriksson}:
% \begin{align*}
%     \min_{\fv,\hv} \tv(\fv)^\top &\fv\\
% \text{subject to }
% \sum\limits_{\p\in\P} \depl \hp&=\fl &&& \forall \l\in\L\\
% \sum_{\p\in\Pod}\hp&=\dod &&& \forall \o,\d\in\N\\
% \hp&\geq 0 &&& \forall \p\in\P
% \end{align*}
% This can be written as:
% \begin{align*}
%     \max_{\fv\in { X}} \rew(\fv)
% \end{align*}
% Where ${ X} = \Fd$ and $\rew(\fv) = -\tv(\fv)^\top \fv$.
% \end{property}


% \subsection{Optimal flow in the Markovian framework}
% The user equilibrium and social optimum notions can be extended to the Markovian framework.
% The idea is to perform the same minimization problems but on the set of equilibrium flows given by the transition matrix, instead of the set of feasible flow allocations.
% The motivation behind the new Markovian formulation is to reduce the number of variables in the static traffic assignment.
% Instead of computing every path flow (which may be expensive), the Markovian framework only requires information on the split ratio at each intersection.
% Therefore, an advantage of the Markovian framework is the ability to perform decentralized traffic control on routing choices.

% \begin{definition}[User equilibrium in Markovian framework] Given a traffic demand \de, a flow allocation $\fv$ is a user equilibrium in the Markov framework if it is solution of:
% \begin{align*}
% \min_{\fv, \Pr} \sum_{\l\in\L}&\int_0^{\fl}\tl(s)ds \\
% \text{subject to }\quad
% \fv&=\Pr^\top \fv + (\Pr_O\de - \Pr_O \de^\top)\mathbf{1}\\
% \fv &\geq 0\\
% \Pr&\in\SPr
% \end{align*}
% \label{def:UE_markov}
% This can be written as:
% \begin{align*}
%     \max_{\fv\in { X}} \rew(\fv)
% \end{align*}
% Where ${ X} = \bigcup\limits_{\Pr\in\SPr}\Fdp$ and $\rew(\fv) = -\sum_{\l\in\L}\int_0^{\fl}\tl(s)ds$.
% \end{definition}
    
% \begin{definition}[Social optimum in Markovian framework] Given a traffic demand \de, a link flow allocation $\fv$ is a social optimum in the Markov framework if it is a solution of:
% \begin{align*}
% \min_{\fv, \Pr}\  &\tv(\fv)^\top\fv \\
% \text{subject to }\quad
% \fv&=\Pr^\top \fv + (\Pr_O\de - \Pr_O \de^\top)\mathbf{1}\\
% \fv &\geq 0\\
% \Pr&\in\SPr
% \end{align*}
% \label{def:SO_markov}
% This can be written as:
% \begin{align*}
%     \max_{\fv\in {X}} \rew(\fv)
% \end{align*}
% Where ${X} = \bigcup\limits_{\Pr\in\SPr}\Fdp$ and $\rew(\fv) = -\tv(\fv)^\top \fv$.
% \end{definition}

% % \todoT{I will remove remark 5.2 and 5.3}
% % \begin{remark}[Well-posedness]
% % Property \ref{prop:existence_markov} gives that the minimization set are non empty.
% % Because the two minimization function are strictly increasing function and $\fv\geq 0$, then the problem is well-posed and the minimum exists.
% % \todoT{Rephrase this remark in a more mathematical way. Maybe it is a property.}
% % \end{remark}

% % \begin{remark}[Convexity]
% % One might want to know if the minimization problems in definition \ref{def:UE_markov} and \ref{def:SO_markov} are convex with respect to any variable $\prl$, $\l\in\L$.
% % This is true on the benchmark network.
% % The general case is not considered in the present article. 
% % \todoT{Rephrase this remark in a more mathematical way. Maybe it is a property.}
% % \end{remark}
% % \todoT{Show for the benchmark network.}


% \begin{remark}[Equivalence between both frameworks]
% The reader may expect the optimal flow allocation of the Markovian framework to be the same as the optimal flow allocation of the classic STA framework. 
% However, remark \ref{rem:feasibility_equilibrium} shows that the set of feasible flow allocations and the set of equilibrium flows over every transition matrix may be different.
% Nevertheless, if the optimal flow allocation in the Markovian framework is a feasible flow allocation and if the optimal flow allocation in the STA framework is an equilibrium flow allocation, then definitions \ref{def:UE} and \ref{def:UE_markov} and definitions \ref{def:SO} and \ref{def:SO_markov} will be equivalent.
% % This is true on the benchmark network. 
% % The general case is not considered in the present article. 
% % \todoT{Rephrase.}
% \end{remark}
% % \todoT{Show for the benchmark network.}

% % \todoT{Add the plots of the static traffic assignment}
% % \subsection{Grid Search on benchmark example}
% % \todoT{To do.}
% % In order to explore the Markovian static traffic assignment framework, experiments are run on the benchmark network.

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=\linewidth]{figures/grid_search_sta.png}
% %     \caption{Grid search on the benchmark network\Fangyu{Emphasize this is theoretical result from STA.}.}
% %     \label{fig:sta_diamond}
% % \end{figure}

% \section{Dynamic traffic assignment}
% In contrast to the static traffic assignment, dynamic models can simulate time-varying networks and establish new equilibria for different departure times.
% Therefore, the previously defined Markovian framework is extended to the dynamic traffic assignment using SUMO.
% Optimization frameworks are developed based on the dynamic notion of the user equilibrium (minimizing average marginal regret) and the social optimum (minimizing the total vehicles hours of travel).
% The benchmark example is then set up in SUMO.

% % This section talks about the limitations of the static traffic assignment and the extension from static models to dynamic models. 
% % This extension includes the ability to simulate time-varying networks and establish new equilibria for different departure times. 
% % Therefore, for dynamic traffic assignment, the section develops the optimization framework and introduces the notion of user-equilibrium and social optimum. 
% % In the end, the setup procedure for SUMO simulation is introduced. 

% % \todoT{Add one line about what we do here. Make sure that notations are consistent with the previous part.}
% % \todoT{Explain that we use the optimization framework to understand what are optimal flow allocations with respect to different reward functions. Explain which learning processes are considered.}
% %Since $\vec{f} = \Delta \vec{h}$, $A\Delta d_{ab}\vec{\rho} = \vec{b}$ 

% \subsection{Limitations of static traffic assignment framework}

% Static models are defined over a relatively long period of time, and the congestion properties of each link are described by a volume-delay function (VDF) that expresses the average link travel time as a function of the traffic volume on that link.
% The travel time on each path would be the summation of the travel time on each link in the path (as described in definition \ref{defi:separability}).
% Moreover, the static model cannot model node dynamics, and for each link, the inflow is always equal to the outflow in the static model (as described in definition \ref{defi:flow_conservation}).
% % Link travel time increases as traffic volume increases.
% Such features cannot capture the dynamics of congestion in each link: how congestion is propagated upstream through the link and spills back to the upstream link \cite{TRB2011dta}. 
% Furthermore, the static traffic assignment assumes that the travel demand for each origin-destination pair is uniformly distributed over time (as defined in definition \ref{defi:graph}) \cite{saw2015literature}. 
% Consequently, the static traffic assignment cannot model scenarios with changing demand. 

% \subsection{Optimization framework for dynamic traffic assignment}
% \subsubsection{Advantages of dynamic traffic assignment}
% Recognizing that traffic networks are generally not in the steady state, 
% extending
% the notion of user equilibrium from the static traffic assignment to dynamic traffic assignment \cite{TRB2011dta} requires: 
% \begin{enumerate}
%     \item Developing efficient ways of describing time-varying network traffic conditions and finding the path with the shortest travel time, considering that link travel times changes over time.
%     \item Establishing a new equilibrium for each departure time. 
% \end{enumerate}
% Compared to static traffic assignment models, dynamic traffic assignment models are able to capture more realistic traffic flow characteristics such as queue spillback, expansion waves, and changing demand \cite{Szeto2006dynamic}. 
% In addition, the traditional travel forecasting models perform simulations on static regional traffic flow while microscopic traffic simulation models focus on dynamic corridor-level traffic analysis \cite{TRB2011dta}. 
% The dynamic traffic assignment models' ability to model at a wide range of scales from the corridor-level to the regional-level fills the gap between travel forecasting models and microscopic traffic simulation models \cite{TRB2011dta}. 
% This can significantly improve the accuracy of traffic estimation. 

% In this article, a simulation-based dynamic traffic assignment model, using a traffic simulator, reproduces the flow dynamics in urban road traffic systems and collects simulation data for optimization \cite{Peeta2001foundation}. 
% A microscopic and open-source simulator SUMO \cite{krajzewicz2002sumo} simulates the traffic flow propagation and spatial-temporal interaction. 
% SUMO is able to handle easy query and traffic control with Python API traci. 

% \subsubsection{User equilibrium and social optimum extensions in the dynamic traffic assignment}
% % Definitions \ref{def:UE_markov} and \ref{def:SO_markov} are easier to extend to the dynamic case than definitions \ref{def:UE} and \ref{def:SO}.
% % The advantage of a Markovian framework for the dynamic traffic assignment over the current static traffic assignment is that the number of variables that need to be controlled do not scale up with time discretization. 
% % Unlike path flows that can change at every time step, this article considers fixed-time transition matrices.


% % Definitions \ref{def:UE_markov} and \ref{def:SO_markov} can be extended to dynamic framework using SUMO by considering flow allocations $\Fdp$ given by SUMO.
% The Markovian framework can be extended using SUMO. 
% First, given a transition matrix, the set of equilibrium flows $\Fdp$ can now be computed.

% \begin{definition}[Flow allocation using SUMO]
% Using SUMO, given a transition matrix $\Pr\in\SPr$ and demand $\de\in\R_{+}^{|\N|\times|\N|}$, we denote $\Fdps$ as the set of corresponding steady-state flow allocations that SUMO computes with $\Pr$ and $\de$ given to the simulator.
% \end{definition}
% \begin{remark}[Steady-state flow allocation]\ 
% Due to the stochastic nature of the simulation process, it generally takes some steps for the flow allocation to achieve a steady state given a fixed transition matrix which encodes the nodes' split ratios. 
% As demonstrated in Figure \ref{fig:grid search}, as the simulation evolves, it takes a certain amount of time steps for the reward distributions (and therefore the flow allocations) to stabilize. 
% % After the network dynamics converge into steady states, it would be more precise and more convenient to run optimization algorithms. 
% \end{remark}

% % Definitions \ref{def:UE_markov} and \ref{def:SO_markov} gives that the user equilibrium and the social optimum for the Markovian framework can be written as:
% % $\max_{\fv\in { X}} \rew(\fv)$
% % where ${X} = \bigcup\limits_{\Pr\in\SPr}\Fdp$ and  $\rew(\fv) = -\tv(\fv)^\top \tv$ or $\rew(\fv) = -\sum_{\l\in\L}\int_0^{\fl}\tl(s)ds$.

% Then, using $\Fdps$, definitions \ref{def:UE_markov} and \ref{def:SO_markov} can be extended to the dynamic case.

% \begin{definition}[Social optimum in Markovian dynamic framework] 
% Given a traffic demand \de, a transition matrix $\Pr$ defines a social optimum in the Markov dynamic framework if it is solution of:
% \begin{align*}
% \max_{\fv, \Pr}\ & \rew(\fv) \\
% \text{subject to }\quad
% \fv&\in\Fdps \\
% \rew(\fv) &=  -\tv(\fv)^\top \fv\\
% \Pr&\in\SPr
% \end{align*}
% Where $\tv(\fv)^\top \fv$ describes the total vehicle hour travelled in the network.
% \end{definition}

% \begin{definition}[User equilibrium in Markovian dynamic framework] 
% Given a traffic demand \de, a transition matrix $\Pr$ defines a user equilibrium in the Markov dynamic framework if it is a solution of:
% \begin{align*}
% \max_{\fv, \Pr}\ & \rew(\fv) \\
% \text{subject to }\quad
% \fv&\in\Fdps \\
% \rew(\fv) &=  -\max_{\mathbf{x}\in\Fd} \tv(\fv)^\top (\fv - \mathbf{x})\\
% \Pr&\in\SPr
% \end{align*}

% $\rew(\fv) =  \max_{\mathbf{x}\in\Fd} \tv(\fv)^\top (\fv - \mathbf{x})$ expresses the average marginal regret of vehicles in the network \cite{Cabannes2019regret}.
% It has been shown that minimizing $\max_{\mathbf{x}\in\Fd} \tv(\fv)^\top (\fv - \mathbf{x})$ and minimizing $\sum_{\l\in\L}\int_0^{\fl}\tl(s)ds$ are equivalent \cite{Cabannes2019regret, nagurney1998network}.
% Furthermore, the average marginal regret can be extended to the dynamic traffic state \cite{cabannes2018measuring}.
% Intuitively, the average marginal regret measures the distance from a traffic flow allocation to a Nash equilibrium, or user equilibrium \cite{Cabannes2019regret}.
% \end{definition}

% \subsubsection{Reward functions}
% Based on the two previous definitions, we experimented with three reward functions: 
% \begin{enumerate} \label{reward_functions}
%     \item \textbf{Average throughput}: maximizing $\fl$ at exit:
% \begin{equation}
%     \rew_{thru} = f_{Exit},
% \end{equation}
%     where $f_{Exit}$ is defined in section ``SUMO Setup''. 
%     \item \textbf{Social optimum}: maximizing the inverse of vehicle hours of travel (VHT), that is, the sum of link flows weighted by average travel time of the edge divided by the sum of link flows:
% \begin{equation}
%     \rew_{VHT} = \frac{1}{VHT}, \quad 
%     VHT = \frac{\sum_{\l \in \L}{(\fl + 1) \cdot \tl}} {\sum_{l \in \L}{\fl + 1}}, \quad
%     t_l = \frac{\lenl}{v_l + 0.1\vlx},
% \end{equation}
%     where $v_l$ is average speed on link $l$ and $\vlx$ is the speed limit on link $l$. Note that addition of one to flow and $0.1v_{l\text{max}}$ to speed is to prevent from division by zero and is not present in the original theoretical definition of those terms.
%     % \item \textbf{User equilibrium}: minimizing the total difference between travel time on any path and the travel time on the path with the shortest travel time divided by the sum of path flows.
%     \item \textbf{User equilibrium}: maximizing inverse of average marginal regret \cite{Cabannes2019regret} divided by the total demand in the network:
%     % total difference between travel time on any path and the travel time on the path with the shortest travel time divided by the sum of path flows.
%     \begin{equation}
%         \rew_{regret} = \frac{\sum_{\p \in \P} {(\hp + 1) (\cp - \min_{\tilde{\p}}c_{\tilde{\p}})}}{\sum_{\p \in \P} {\hp + 1}}, \quad
%         \cp = \frac{\lenp}{\vp + 0.1\vpx},
%     \end{equation}
%     where $\vp$ is the average speed on path $\p$ and $\vpx$ the speed limit on link $p$. Similar to $R_{VHT}$, we add one to $h_p$ and $0.1v_{\p\text{max}}$ to speed for numerical stability. Furthermore, in our case study, we approximate traffic on path $ABD$ with traffic on path $BD$; traffic on path $ABCED$ with traffic on path $BC$, and traffic on path $ACED$ with traffic on path $AC$.
% \end{enumerate}

% \subsection{SUMO setup}
% The road network in Figure~\ref{fig:diamond_network} is simulated in SUMO \cite{SUMO2012}. The goal here is to simulate the traffic states with different split ratios and to provide data for flow allocation optimization. 



% \begin{figure}[H]
% \centering
% \begin{subfigure}[t]{0.45\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{figures/SUMO_network.png}
%   \caption{SUMO Network Setup: A screenshot from SUMO GUI that describes the geometry of nodes and edges. Blue arrows are added to visualize the direction of traffic flow.}
%   \label{fig:network_setup}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.45\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{figures/Merge_zoom.png}
%   \caption{Merge dynamics: A zoom out window that details how the merge at C is designed on the right network. Note that vehicles from the two lanes take turns to merge in a ``first come, first served'' basis.}
%   \label{fig:merge}
% \end{subfigure}
% \caption{SUMO Setup}
% \label{fig:sumo_setup}
% \end{figure}

% The simulated traffic network is illustrated in Figure~\ref{fig:sumo_setup} and the simulation setup is detailed. For source code, please refer to 
% \cite{Learning_matrix2019}.

% % \subsubsection{Initialization of the network}
% % \begin{itemize}[leftmargin=2em]
% %     \item Fix the position of nodes and edges in desired network in Figure~\ref{fig:diamond_network}.
% %     \item Handle merge at $C$ using buffer space with the help of $E$ to prevent congestion from forming due to bottleneck capacity at merge. 
% %     \item Smooth the two-lane buffer zone back to one lane for consistency with other lanes.
% % \end{itemize}
    
% \begin{enumerate}[leftmargin=2em]
%     \item Set time step $\Delta{t} = 0.5 s$. %We denote the set of time step $T = \delta t\Nu$. For the simulation, $\delta t$ is 0.5 seconds.
%     \item Generate a demand profile $d$ using a Poisson distribution with a rate of 1 veh/s.
%     \item Input a transition matrix $\Pr\in\SPr$.
%     \item Initialize the network with no vehicles.
%     \item For every time step $i\in T$:
%     \begin{itemize}
%         \item Generate vehicles $v\in\mathcal{V}_i$ for the time step $i$ given the demand (where $\mathcal{V}_i$ is the set of all vehicles generated at the time step $i$, $|\mathcal{V}_i| = d$).
%         \item For every vehicle generated:
%         \begin{itemize}
%             \item Create vehicle path according to transition matrix.
%             % \begin{itemize}
%             %     \item Initialize $\p_{v}$ as an empty list: $\p_{v}=[]$
%             %     \item Add the first links ($Enter$) to $\p_{v}$
%             %     \item Iteratively add downstream links $\l$ to the path $\p_{v}$ of the vehicle $v$ following the  probability distributions from the transition matrix $\Pr$:
%             %     each downstream link $\l$ is added to the path $\p_v$ with the probability $\prl$.
%             % \end{itemize}
%             \item Add vehicle $v$ to the network following path $\p_{v}$.
%         \end{itemize}
%         %\item Let SUMO takes care of the dynamics of the vehicles already in the network.
%     \end{itemize}
%     %\item At the end of the simulation, store the data for analysis.
% \end{enumerate}


% \section{Learning optimal flow allocation}
% In this section, we describe the three optimization methods, i.e., grid search, random search, and evolution strategies, we used to search for optimal transition matrix under the three aforementioned reward functions, i.e., average throughput, social optimum, and user equilibrium.
% As illustrated in Figure~\ref{fig:sumo_setup}, the road network has two splits at $\n_A$ and $\n_B$. Therefore, we only need to optimize two variables, $\pr{AB}$ and $\pr{BC}$. 

% As a baseline, we start with a very simple learning algorithm grid search. 
% Next, we solve the same optimization problem using random search and then, a more advanced optimizer, evolution strategies, respectively. 
% Finally, we remark on their pros and cons and discuss how to choose among them in practice. 

% \subsection{Grid search}
% Grid search is an optimization procedure that finds an optimal solution by checking the rewards at every point in a discretized search space and selecting the point(s) with the highest reward. 
% Pseudocode of this algorithm is described in Algorithm~\ref{alg:grid_search}\cite{JimÃ©nez2007}

% The results of grid search is illustrated in Figure~\ref{fig:grid search}. To illustrate evolution of the system dynamics, we plot the heatmap of each reward on a meshgrid of $\pr{AB}$ and $\pr{BC}$ with each axis incrementing from 0 to 1 at stepsize of 0.05. Each simulation is designed to execute 1000  steps, i.e., 500 seconds; each column of Figure~\ref{fig:grid search} shows the progression of heatmaps for each reward function throughout the simulation timestamped at 37.5 s, 87.5 s, 287.5 s, and 487.5 s. 

% Reward functions are evaluated in equilibrium states using data between 475 s and 500 s. The resulting optima found by grid search are marked in the last row of the figure with ``$\star$'' symbols.


% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{figures/rewards_1000step_average.pdf}
%     \caption{Grid Search Results: Each column corresponds to the time-varying distribution of each reward function on the meshgrid of $P_{AB}$ and $P_{BC}$ throughout the simulation. The three columns respectively correspond to reward functions for average outflow, inverse of vehicle hours of travel and inverse of average marginal regret. At time 487.5s, when the network has converged to steady state, the point that gives the highest reward is marked as $\star$ for each reward function. }
%     \label{fig:grid search}
% \end{figure}

% The interpretation of plot of average throughput reward is straightforward because in order to maximize the the exit flow, it's reasonable to minimize congestion in every path. 
% As illustrated in Figure~\ref{fig:sumo_setup}, there is a merge at $C$. 
% When a vehicle is about to turn at a sharp angle, there is a speed reduction for all vehicles in the area, which increases the path travel time. 
% When the amount of vehicles trying to merge at $C$ exceeds capacity, the speed reduction would result in spillbacks in $AC$ or/and $BC$ and therefore decrease the flow rate at exit. 
% In consideration of the merge, when $\pr{AB} >= 0.6$ and $\pr{BC} <= 0.4$, congestion is minimized and the exit flow maximized. 

% The plot for social optimum reward is also reasonable because in order to minimize the weighted average flow travel time, we want to keep each $\p\in\P$ that is in use during simulation unsaturated so the average travel time would be minimized.
% Likewise, we should take the speed reduction at sharp turns into account. 
% The turning angle from $AB$ to $BC$ and from $BC$ to $CE$ is larger than that from $AC$ to $CE$, therefore vehicles would be more likely to experience a larger the speed reduction if taking the route of $AB$ than that of $AC$.
% When $\pr{AB}$ is zero, which means all cars are taking the $\p_{Enter\rightarrow A \rightarrow C \rightarrow E \rightarrow D}$, the reward would be maximized. 
% The worst scenario would be about half percentage of incoming vehicles takes $AB$ and most of these vehicles turn into $BC$ at $B$ to merge with the other half of the vehicles taking $AC$ at $C$. 
% Such merge would cause serious spill back that significantly elongate the path travel time, and therefore the weighted average flow travel time.

% The plot for user equilibrium reward is compatible with the characteristics of the network. 
% The user equilibrium achieves when no one in the network could achieve a shorter travel time if switching to a different path. 
% Therefore, when vehicles approximately have equal split at both $A$ and $B$, there would be queues spilling ack upstream to both $BC$ and $AB$. 
% Such congestion delay would balance out the difference in path's free flow travel time and creates the social equilibrium that each user experiences the same travel time. 
% If some paths in the network is congested while one path is unsaturated, some vehicles could always achieve shorter travel time by switching to the other path.
% If one path is under-saturated, some vehicles could always achieve shorter travel time by switching to the other path. Note that the maximum point is slightly biased toward $AB$ and $BD$. Such bias is also an artefact of reduced road capacity at $BC$ and $CD$ induced by sharp turning angles.

% \begin{figure}
% \centering
% \begin{subfigure}[b]{\textwidth}
%   \includegraphics[width=1\linewidth]{figures/random_search.pdf}
%   \caption{Random Search: Random search graph is performed on top of the reward distribution graph at 975 time-steps of simulation. 50 sample points (black dots) are picked to measure the reward function and the optimal point that gives the highest reward is marked by ``+'' symbol. For comparison, the solution found by grid search is marked by ``$\star$'' symbol.}
%   \label{fig:random_search}
% \end{subfigure}

% \begin{subfigure}[b]{\textwidth}
%   \includegraphics[width=1\linewidth]{figures/gradient_ascent.pdf}
%   \caption{Evolution Strategies: Similar to random search, based on the reward distribution at 975 time-steps of simulation, evolution strategies first randomly pick a starting point and then start climbing uphill with gradient ascent demonstrated by the black trace. The algorithm is manually terminated after 50 iterations at location marked by ``+'' symbol. For comparison, the solution found by grid search is marked by ``$\star$'' symbol.}
%   \label{fig:gradient_ascent}
% \end{subfigure}
% \caption{Random Search and Evolution Strategies Results}
% \end{figure}

% \subsection{Random search}
% Random search is an optimization method that finds an optimal solution by checking the rewards at a few random points from search space and selecting the point(s) with the highest reward. 
% Pseudocode of this algorithm is described in Algorithm~\ref{alg:random_search} \cite{Zabinsky2011random}.

% The result is illustrated in Figure~\ref{fig:random_search}. 
% In the figure, 50 random points are sampled, among which the best point is marked by ``+'' symbol. The location marked by ``$\star$'' symbol is the optimal solution found by grid search.
% By visually checking the graph, the solutions found by the two methods are comparable.


% \subsection{Evolution strategies}
% Evolution strategies is an optimization method that finds an optimal solution using gradient ascent, where the gradients are estimated from Gaussian sampling in the neighbourhood of current solution.
% Specifically, for each iteration, a stochastic gradient is computed from rewards of a few points normally distributed around the current solution. 
% The gradient is then added to the current solution to generate the new solution. 
% Pseudocode of this algorithm is described in Algorithm~\ref{alg:evolution_strategies} \cite{salimans2017evolution}. 

% The results of evolution strategies for three different reward functions is illustrated in Figure~\ref{fig:gradient_ascent}. 
% For a fair comparison with the random search method, the trajectories are stopped after 50 iterations.
% All three trajectories, despite being occasionally distracted, are generally climbing uphill toward higher rewards. 
% The termination locations are marked by ``+'' symbol. 
% Comparing them with those marked by ``$\star$'' symbol, the optimal points found by evolution strategies are just as good as the ones found by grid search. 

% \noindent
% \begin{minipage}[t]{0.33\textwidth}
% \vspace{0pt}
% \IncMargin{-1.9em}
% \begin{algorithm}[H]
% \footnotesize
%     Policy $\theta \leftarrow (\pr{AB}, \pr{BC})$\;
%     Reward $R(\theta)$\;
%     Search step size $\Delta$\;
%     Samples per point $n$\;
%     Time horizon $T$\;
%     Warmup time $\tau$\;
%     $\hat{r^*} \leftarrow -\infty$\;
%     \For{$\pr{AB} \leftarrow 0$; $\pr{AB} \leq 1$; $\pr{AB} \leftarrow \pr{AB}+\Delta$} {
%         \For{$\pr{BC} \leftarrow 0$; $\pr{BC} \leq 1$; $i \leftarrow \pr{BC}+\Delta$} {
%             $\bar{\theta} \leftarrow (\pr{AB}, \pr{BC})$\;
%             \For{$i \leftarrow 0$; $i < n$; $i \leftarrow i+1$} {
%                 $r_i \leftarrow 0$\;
%                 \For{$ t \leftarrow 0$; $t < T$; $t \leftarrow t+1$} {
%                     Step simulation\;
%                     \If{$t > \tau$}{
%                         $r_i \leftarrow r_i + R(\bar{\theta})$\;
%                     }
%                 }
%             }
%             $\bar{r} \leftarrow \frac{1}{n}\sum_{i \leftarrow 0}^{n-1}r_{i}$ \\
%             \If{$\bar{r} > \hat{r^*}$} {
%                 $\hat{r^*} \leftarrow \bar{r}$\;
%                 $\hat{\theta^*} \leftarrow \bar{\theta}$\;
%             }    
%         }
%     }
%     \Return $\hat{\theta^*}$
% \caption{Grid Search}
% \label{alg:grid_search}
% \end{algorithm}
% \end{minipage}%
% \hfill
% \begin{minipage}[t]{0.33\textwidth}
% \vspace{0pt} 
% \IncMargin{-1.9em}
% \begin{algorithm}[H]
% \footnotesize
%     Policy $\theta \leftarrow (\pr{AB}, \pr{BC})$\;
%     Reward $R(\theta)$\;
%     Number of random samples $m$\;
%     Samples per point $n$\;
%     Time horizon $T$\;
%     Warmup time $\tau$\;
%     $\hat{r^*} \leftarrow -\infty$\;
%     \For{$j \leftarrow 0$; $j < m$; $j \leftarrow j+1$}{
%         $\bar{\theta} \leftarrow (\pr{AB}, \pr{BC})$ where $\pr{AB}, \pr{BC} \sim \mathcal{U}(0, 1)$\;
%         \For{$i \leftarrow 0$; $i < n$; $i \leftarrow i+1$}{
%             $r_i \leftarrow 0$\;
%             \For{$t \leftarrow 0$; $t < T$; $t \leftarrow t+1$}{
%                 Step simulation\;
%                 \If{$t > \tau$}{
%                     $r_i \leftarrow r_i + R(\bar{\theta})$\;
%                 }
%             }
%         }
%         $\bar{r} \leftarrow \frac{1}{n}\sum_{i \leftarrow 0}^{n-1}r_{i}$ \\
%         \If{$\bar{r} > \hat{r^*}$} {
%             $\hat{r^*} \leftarrow \bar{r}$\;
%             $\hat{\theta^*} \leftarrow \bar{\theta}$\;
%         }    
%     }
%     \Return $\hat{\theta^*}$
% \caption{Random Search}
% \label{alg:random_search}
% \end{algorithm}
% \end{minipage}%
% \hfill
% \begin{minipage}[t]{0.33\textwidth}
% \vspace{0pt}
% \IncMargin{-1.9em}
% \begin{algorithm}[H]
% \footnotesize
%     Policy $\theta \leftarrow (\pr{AB}, \pr{BC})$\;
%     Reward $R(\theta)$\;
%     Number of iterations $m$\;
%     Learning rate $\alpha$\;
%     Noise magnitude $\sigma$\;
%     Samples per iteration $n$\;
%     Time horizon $T$\;
%     Warmup time $\tau$\;
%     Initialize $\hat{\theta^*} \leftarrow (\pr{AB}, \pr{BC})$ where $\pr{AB}, \pr{BC} \sim \mathcal{U}(0, 1)$\;
%     \For{$j \leftarrow 0$; $j < m$; $j \leftarrow j+1$}{
%         \For{$i \leftarrow 0$; $i < n$; $i \leftarrow i+1$}{
%             Sample $\epsilon_i \sim \mathcal{N}(0, \sigma{I})$\;
%             $\theta_i \leftarrow \hat{\theta^*} + \epsilon_i$\;
%             Clip all $\theta_i$ entries to be within [0, 1]\;
%             $r_i \leftarrow 0$\;
%             \For{$t \leftarrow 0$; $t < T$; $t \leftarrow t+1$}{
%                 Step simulation\;
%                 \If{$t > \tau$}{
%                     $r_i \leftarrow r_i + R(\bar{\theta})$\;
%                 }
%         }
%         }
%         $\nabla\hat{\theta^*} \leftarrow  \frac{1}{n\sigma}\sum_{i \leftarrow 0} ^{n-1}{r_i\epsilon_i}$\;
%         $\hat{\theta^*} \leftarrow \hat{\theta^*} + \alpha\nabla\hat{\theta^*}$\;
%     }
%     \Return $\hat{\theta^*}$
% \caption{Evolution Strategies}
% \label{alg:evolution_strategies}
% \end{algorithm}
% \end{minipage}%

% \subsection{Discussion}
% Although grid search can be exhaustive, it does not scale well with the dimension of the problem. This is commonly known as the ``curse of dimensionality.''   
% Compared to grid search, random search is found to be more efficient, both theoretically and empirically \cite{bergstra2012random}.
% Compared to random search, evolution strategies prefers samples nearby and may perform better in problems where local reward topology is constructive to guide gradient ascent.

% In practice, if the dimension of the problem is small, all of the three methods are good choices. For large problems, random search or evolution strategies should be used instead. For problems where it is possible to efficiently compute the exact gradient, vanilla gradient ascent methods may be used instead. However, random search and evolution strategies can be easily parallelized across a large cluster of nodes, which may result in finding a good solution within less wall clock time.

% \section{Conclusion}

% This article first compares the Markovian static traffic assignment to the classic static traffic assignment.
% The notions of user equilibrium and social optimum flow allocations are introduced for the Markovian framework.
% The Markovian framework reduces the number of variables to compute in the static traffic assignment by introducing the Markov property of the traffic system (i.e.\ a traveler does not take into account her/his previous path to decide the next road to take).
% Then, extensions of these notions to the dynamic traffic assignment using the traffic micro-simulator SUMO are made.
% On a benchmark network, the simulator learns optimal routing behavior by finding optimal flow split ratios at every node using grid search, random search, and evolution strategies.
% The results show the ability of the Markovian framework to learn optimal routing behavior using SUMO.

% The work can lead to several potential applications.
% First, the transition matrix framework may be used to perform traffic estimation through data assimilation using regression with cross-sectional data.
% Second, decentralized traffic control strategies may be developed by learning optimal transition matrices.
% Third, Markov chain theory and graph theory can be used to better understand the resiliency of the traffic network.
% Lastly, time-varying transition matrices in which the optimal split ratios may be learned through reinforcement learning will be considered.
% Another direction will be to consider split ratios that depend on the destinations of the vehicles, where every possible destination has a transition matrix associated with it.

\\
\bibliographystyle{trb}
\bibliography{trb_template}
\end{document}

==> old_stuff.tex <==
\section{Stuff to add or for another article}

%%%%%%%%%%% OLD DESCRIPTION BY HARRY %%%%%%%%%%%%% 
Both $\G$ and $L(\G)$ can be viewed as Markov chains.
In $\G$, the nodes are intersections and links are roads between intersections with transition probabilities determining the likelihood that a commuter chooses one road over others at an intersection. 
In $L(\G)$, the nodes are links in $\G$, and links are every possible intersection of two roads where the direction of the link is from the road before the intersection to the road after the intersection.
Thus, transition probabilities determine the likelihood of going from one road to another.
In fact, transition probabilities in $L(\G)$ come from transition probabilities in $\G$.
The transition probability of a link in $L(\G)$ is the same as the probability going from the previous road to the current road.
To make this more concrete, let us use the diamond example.
The probability associated with link $l \in L(\L)$ that joins nodes $b$ and $d$ is the probability of going from the road represented by $b$ in $\G$ to the road represented by $d$ in $\G$.
This probability is the same as the probability of taking road $d$ after reaching the intersection from taking road $b$.

Another point of clarification is the demand matrix $\de$. 
In our model, there are no commuters in the network at the beginning.
Then, the demand $\sum_{j \in \N}d_{ij}$ enters the network at node $i \in \N$ at each timestep.
Demand leaving the network is slightly different.
A maximum of $\sum_{i \in \N}d_{ij}$ leaves the network from node $j \in \N$ at  at each timestep.
However, since there cannot be a negative number of commuters, the demand leaving the network never exceeds the total flow into $j$.
More formally, the demand that that leaves the network at node $j$ is $min\{ \sum_{i \in \N}d_{ij}, \sum_{i \in \N}f_{ij} \}$.
Consequently, the number of commuters in the network monotonically increases until $\sum_{i \in \N}f_{ij} \geq \sum_{i \in \N}d_{ij}$ for all $j$.
At equilibrium, the flows on all roads do not change with time, implying demand entering the network is equal to the demand leaving the network.

The reason $L(\G)$ is useful is that by representing roads as nodes rather than links, we can use Markov chains to calculate how flow shifts from one node to the next, or from one road to the next, instead of flow of an intersection which is captured in $\G$.

There are several advantages of using Markov chains.
Under this model, we can use properties of Markov chains which will be handy in the next several sections, most notably, the properties of irreducibility and periodicity.
Additionally, this model allows us to combine different modes of transportation   into one network \cite{faizrahnemoon2016real}.
For instance, cars, trains, and other forms of travel can be placed in the same network without having to treat them differently.
Markov chains can also extend to larger networks, so scaling is not a significant issue \cite{crisostomi2011google}.
Furthermore, another benefit is the transition matrix, which captures a nontrivial amount of information about the network which we will explore.

The limitations of this model are that we make time discrete and that we assume that at each timestep, commuters travel from one node to the next. 
Additionally, we assume that each commuter acts independently, meaning commuters choose routes without considering other commuters' choices and without considering previous road choices \cite{crisostomi2011google}.
Another limitation is that we treat demand and transition probabilities as constants, an inherent weakness with the static traffic assignment model.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% ACYCLIC GRAPH %%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{remark}[Existence of an equilibrium flow for acyclic graph]
If the graph is acyclic, then the graph is not strongly connected. Some row of $\Pr$ will be equal to zero, but an equilibrium flow will still exist.

Indeed, for an acyclic graph $I-\Pr^\top$ is invertible, $(I-\Pr^\top)^{-1} = \sum_{i=0}^{|\L|}\Pr^{i}$
\end{remark}

For a connected acyclic, we can define the flow at equilibrium $\fv_{eq}$ as:

\begin{equation}
    \fv_{eq} = L(\Pr)^\top \fv_{eq} + diag(\prv) \O \de \mathbbm{1}
\end{equation} 

\begin{remark}[Transition matrices conventions]
In some texts using Markov chains, row vectors are used, so if $P$ is the transition matrix and $\mathbf{x}_t$ is the distribution of commuters in the network at time $t$ organized in a row vector, then $\mathbf{x}_{t+1} = \mathbf{x}_t P$. 
However, for column vectors, we can take the transpose of both sides to get $\mathbf{y}_{t+1} = P^\top \mathbf{y}_t$ for $\mathbf{y}_t := \mathbf{x}_t^\top$ and $\mathbf{y}_{t+1} := \mathbf{x}_{t+1}^\top$.
\end{remark}

\begin{equation}
\begin{split}
    diag(\prv) O
    &= \begin{bmatrix}
        p_a    &0       &\dots  &0\\
        0      &p_b     &       &\vdots\\
        \vdots &        &\ddots &0\\ 
        0      &\dots   &0      &p_{\epsilon} 
    \end{bmatrix}
    \begin{bmatrix}
        0 &\dots &1 &\dots &0 \\
        0 &\dots &1 &\dots &0 \\
        & &\vdots \\
        0 &\dots &1 &\dots &0
    \end{bmatrix} 
    = \begin{bmatrix}
        0 &\dots &p_a &\dots &0 \\
        0 &\dots &p_b &\dots &0 \\
        & &\vdots \\
        0 &\dots &p_{\epsilon} &\dots &0
    \end{bmatrix}
\end{split}
\end{equation}

\begin{equation}
\begin{split}
    diag(\prv) O \de \mathbbm{1} &= \begin{bmatrix}
        p_a\sum_{\tilde{u}\in\N}d_{k_a\tilde{u}} \\
        p_b\sum_{\tilde{u}\in\N}d_{k_b\tilde{u}} \\
        \vdots \\
        p_\epsilon\sum_{\tilde{u}\in\N} d_{k_\epsilon\tilde{u}}
    \end{bmatrix}
\end{split}
\end{equation}

Now, let us make sure that entries in the above vector sum to zero:
\begin{equation}
\begin{split}
    \begin{bmatrix}
        1 &1 &\dots &1
    \end{bmatrix}
    \begin{bmatrix}
        p_a\left[\sum_{\tilde{u}\in \N}d_{k_a\tilde{u}} - \sum_{\tilde{w}\in \N}d_{\tilde{w}k_a}\right] \\
        p_b\left[\sum_{\tilde{u}\in \N}d_{k_b\tilde{u}} - \sum_{\tilde{w}\in \N}d_{\tilde{w}k_b}\right] \\
        \vdots \\
        p_\epsilon\left[\sum_{\tilde{u}\in \N}d_{k_\epsilon\tilde{u}} - \sum_{\tilde{w}\in \N}d_{\tilde{w}k_\epsilon}\right]
    \end{bmatrix}
    %&= \sum_{l \in\L} \sum_{\tilde{u}\in \N}p_ld_{k_l\tilde{u}} - \sum_{m \in\L} \sum_{\tilde{w} \in \N} p_ld_{\tilde{w}k_l} \\
    &= \sum_{\tilde{u}\in \N}\sum_{l \in\L} p_ld_{k_l\tilde{u}} - \sum_{\tilde{w} \in \N}\sum_{m \in\L}  p_ld_{\tilde{w}k_l} \\
    &= \sum_{\tilde{u}\in \N}\sum_{\tilde{v}\in \N} d_{\tilde{v}\tilde{u}} - \sum_{\tilde{w} \in \N}\sum_{\tilde{x}\in \N} d_{\tilde{x}\tilde{w}} = 0
\end{split}
\end{equation}

The third equality comes from the fact that the sum of outgoing probabilities of any node equals 1:

\begin{equation}
\begin{split}
    \sum_{\tilde{u}\in \N}\sum_{l \in\L} p_ld_{k_l\tilde{u}} &= \sum_{\tilde{u}\in \N}\sum_{\tilde{v} \in \N}\sum_{\tilde{w} \in \N} p_{\tilde{v}\tilde{w}}d_{\tilde{v}\tilde{u}} = \sum_{\tilde{u}\in \N}\sum_{\tilde{v} \in \N}\left[d_{\tilde{v}\tilde{u}}\sum_{\tilde{w} \in \N} p_{\tilde{v}\tilde{w}}\right] = \sum_{\tilde{u}\in \N}\sum_{\tilde{v} \in \N}d_{\tilde{v}\tilde{u}}
\end{split}
\end{equation}


Rearranging terms and letting $I_{|\L|}$ be a $|\L| \times |\L|$ identity matrix, we get:

\begin{equation}
    \fv_{eq} = (I_{|\L|} - L(\Pr)^\top)^{-1} diag(\prv) \O \de \mathbbm{1}
\end{equation}

If $\G$ is acyclic, then $L(\G)$ is also acyclic which implies $L(\Pr)$ can be constructed such that $L(\Pr)$ has 0's on and below the diagonal.
This means $L(\Pr)^\top$ is also nilpotent, and as a consequence, $I - L(\Pr)^\top$ is invertible.


\subsection{Acyclic graph}

For a connected acyclic, we can define the flow at equilibrium $\fv_{eq}$ as:

\begin{equation}
    \mathbf{f}_{eq} = L(P)^\top \mathbf{f}_{eq} + daig(\prv) \O [\de-\de^\top] \mathbf{1}
\end{equation}

\begin{remark}[Transition matrices conventions]
In some texts using Markov chains, row vectors are used, so if $P$ is the transition matrix and $\mathbf{x}_t$ is the distribution of commuters in the network at time $t$ organized in a row vector, then $\mathbf{x}_{t+1} = \mathbf{x}_t P$. 
However, for column vectors, we can take the transpose of both sides to get $\mathbf{y}_{t+1} = P^\top \mathbf{y}_t$ for $\mathbf{y}_t := \mathbf{x}_t^\top$ and $\mathbf{y}_{t+1} := \mathbf{x}_{t+1}^\top$.
\end{remark}

\proof
If we want the flow $f_{vn}$ of the link from $v$ to $n \in\N$, we can rearrange the above equation and multiply both sides by $\pr{vn}$ to find $f_{vn}$:

\begin{equation}
\begin{split}
p_{vn}\sum_{w}f_{vw} &= p_{vn}\left[\sum_{u}f_{uv} + \sum_{\tilde{u}}d_{v\tilde{u}} - \sum_{\tilde{w}}d_{\tilde{w}v}\right] \\
f_{vn} &= p_{vn}\left[\sum_{u}f_{uv} + \sum_{\tilde{u}}d_{v\tilde{u}} - \sum_{\tilde{w}}d_{\tilde{w}v}\right] &\text{since $p_{vn} = \frac{f_{vn}}{\sum_{w}f_{vw}}$}\\
\end{split}
\end{equation}

Notice that $L(\Pr)^\top\fv$ is represented by $p_{vn}\sum_{u}f_{uv} \forall v \in \L$ since this is a transfer of flow in one timestep. 
Similarly, we can make a connection to $p_{vn}\left[\sum_{\tilde{u}}d_{v\tilde{u}} - \sum_{\tilde{w}}d_{\tilde{w}v}\right]$ as $diag(\prv) \O [\de-\de^\top]\mathbf{1}$.
The connection is made more clear below. 
Note that entries equal to 1 in $\O$ are not all lined up (refer to the definition of the origin matrix). 
Let $a, b, \dots,\epsilon$ represent links, $n$ be the number of nodes, and $k_a, k_b, \dots, k_\epsilon$ are origin nodes of links $a, b, \dots,\epsilon$ where $1 \leq k_a, k_b, \dots, k_\epsilon \leq n$:

\begin{equation}
\begin{split}
    diag(\prv) \O [\de-\de^\top]\mathbf{1} &= \begin{bmatrix}
        p_a\sum_{\tilde{u}\in\N}\left(d_{k_a\tilde{u}} - d_{\tilde{u}k_a}\right) \\
        p_b\sum_{\tilde{u}\in\N}\left(d_{k_b\tilde{u}} - d_{\tilde{u}k_b}\right) \\
        \vdots \\
        p_\epsilon\sum_{\tilde{u}\in\N}\left(d_{k_\epsilon\tilde{u}} - d_{\tilde{u}k_\epsilon}\right)
    \end{bmatrix}  = \begin{bmatrix}
        p_a\left[\sum_{\tilde{u}\in\N}d_{k_a\tilde{u}} - \sum_{\tilde{w}\in\N}d_{\tilde{w}k_a}\right] \\
        p_b\left[\sum_{\tilde{u}\in\N}d_{k_b\tilde{u}} - \sum_{\tilde{w}\in\N}d_{\tilde{w}k_b}\right] \\
        \vdots \\
        p_\epsilon\left[\sum_{\tilde{u}\in \N}d_{k_\epsilon\tilde{u}} - \sum_{\tilde{w}\in \N}d_{\tilde{w}k_\epsilon}\right]
    \end{bmatrix}
\end{split}
\end{equation}


Thus, all entries in the resulting vector is what we wanted. Now, let us make sure that entries in the above vector sum to zero:
\begin{equation}
\begin{split}
    \begin{bmatrix}
        1 &1 &\dots &1
    \end{bmatrix}
    \begin{bmatrix}
        p_a\left[\sum_{\tilde{u}\in \N}d_{k_a\tilde{u}} - \sum_{\tilde{w}\in \N}d_{\tilde{w}k_a}\right] \\
        p_b\left[\sum_{\tilde{u}\in \N}d_{k_b\tilde{u}} - \sum_{\tilde{w}\in \N}d_{\tilde{w}k_b}\right] \\
        \vdots \\
        p_\epsilon\left[\sum_{\tilde{u}\in \N}d_{k_\epsilon\tilde{u}} - \sum_{\tilde{w}\in \N}d_{\tilde{w}k_\epsilon}\right]
    \end{bmatrix}
    %&= \sum_{l \in\L} \sum_{\tilde{u}\in \N}p_ld_{k_l\tilde{u}} - \sum_{m \in\L} \sum_{\tilde{w} \in \N} p_ld_{\tilde{w}k_l} \\
    &= \sum_{\tilde{u}\in \N}\sum_{l \in\L} p_ld_{k_l\tilde{u}} - \sum_{\tilde{w} \in \N}\sum_{m \in\L}  p_ld_{\tilde{w}k_l} \\
    &= \sum_{\tilde{u}\in \N}\sum_{\tilde{v}\in \N} d_{\tilde{v}\tilde{u}} - \sum_{\tilde{w} \in \N}\sum_{\tilde{x}\in \N} d_{\tilde{x}\tilde{w}} = 0
\end{split}
\end{equation}

\subsection{Proofs}

% \todoT{
% \begin{itemize}
%     \item Feasible path flow allocation with the transition matrix [Harry]
%     \item Feasible link flow allocation with the transition matrix [Harry]
%     \item Minimization problem for the transition matrix framework
%     \item Convexity of the minimization problem [Theo]
% \end{itemize}}
\todoT{Path flow allocation. Link flow allocation. Equilibrium flow. }


\paragraph{Assumptions}\ 

\todoT{To do:  unique destination. no cycle that does not include the destination. $\pr{ii}=0$.}

\begin{definition}[Path flow with transition matrix]\label{defi:path_transition}
Given a transition matrix $\Pr$, a demand matrix $\de\in\R^{|\N|\times|\N|}_{+}$, and a path $\p$, we define the path flow of the path $\p$, $\hp = \dod \prod\limits_{i=1}^{|\p|}\pr{
p_i, p_{i+1}}$
\end{definition}

\begin{property}[Feasibility of path flow with transition matrix]
Given a transition matrix $\Pr$ and a demand matrix $\de\in\R^{|\N|\times|\N|}_{+}$, the path flow allocation $\hv$ defined in definition \ref{defi:path_transition} is a feasible path flow allocation $\hv\in\Hd$ which $\Hd$ defined in definition \ref{defi:path_flow}.
\end{property}
\proof{
\todoT{To do. Show that $\sum_{\p\in\Pod}\hp=\dod$}
}

\begin{property}[Path flow with transition matrix defines a equilibrium flow]
Given a transition matrix $\Pr$ and a demand matrix $\de\in\R^{|\N|\times|\N|}_{+}$, the path flow allocation $\hv$ defined in definition \ref{defi:path_transition} is aa feasible path flow allocation $\hv\in\Hd$ which $\Hd$ defined in definition \ref{defi:path_flow}.
\end{property}
\proof{
\todoT{To do. Show that $\fl = \sum_{\p}\depl \hp = \prl \sum_{\p} \depl \frac{\hp}{\prl}$}
}

\todoT{Path flow allocation. Link flow allocation as equilibrium flow. Uniqueness of the equilibrium flow under conditions.}
\begin{remark}[In case of several destinations.]
\todoT{To do}
\end{remark}

\begin{remark}[In case of cycles.]
\todoT{To do}
\end{remark}



Instead of link flows, we can choose to focus on path flows as well. We first define the path probabilities $\rho$ as:
\begin{equation}
    \rho = [\Delta^\top diag(p)_{ln}^\top \mathbbm{1}]_e
\end{equation}

\todo[inline]{Try to show that $\mathbf{1}^\top \rho = 1$ when there is only one origin destination pair.}

Let $\delta_k$ be row in the incidence matrix corresponding to link $k$, $P_j$ be the set of links in path $j$, and $\beta$ be number of paths:

\begin{equation}
\begin{split}
    \rho &= 
    \left[
    \begin{bmatrix}
        \delta_a^\top &\delta_b^\top &\dots &\delta_\epsilon^\top
    \end{bmatrix}
    \begin{bmatrix}
        ln(p_a)    &0       &\dots  &0\\
        0      &ln(p_b)     &       &\vdots\\
        \vdots &        &\ddots &0\\ 
        0      &\dots   &0      &ln(p_{\epsilon}) 
    \end{bmatrix}
    \begin{bmatrix}
        1 \\
        \vdots \\
        1
    \end{bmatrix}
    \right]_e \\
    &= \begin{bmatrix}
        ln(p_a)\delta_a^\top + ln(p_b)\delta_b^\top + \dots + ln(p_\epsilon)\delta_\epsilon^\top
    \end{bmatrix}_e \\
    &= \begin{bmatrix}
        e^{\sum_{l \in P_1}ln(p_l)} \\
        \vdots \\
        e^{\sum_{l \in P_\beta}ln(p_l)}
    \end{bmatrix} \\
    &= \begin{bmatrix}
        \prod_{l \in P_1}p_l \\
        \vdots \\
        \prod_{l \in P_\beta}p_l
        \end{bmatrix}
\end{split}
\end{equation}

For one origin-destination pair, we can show that $\mathbf{1}^\top \rho = 1$:

\begin{equation}
    \begin{split}
        \mathbf{1}^\top \vec{\rho} &=
        \begin{bmatrix}
            1 &\dots &1
        \end{bmatrix}
        \begin{bmatrix}
            \prod_{l \in P_1}p_l \\
            \vdots \\
            \prod_{l \in P_\beta}p_l
        \end{bmatrix} \\ 
        &= \sum_{j = 1}^\beta \prod_{l \in P_j}p_l 
    \end{split}
\end{equation}

\todo[inline]{If there is a cycle then $s_{od}=\infty$ (which is not well defined)}

We can prove that $\sum_{j = 1}^\beta \prod_{l \in P_j}p_l$ sums to 1 using strong induction. 
Let distance be defined as the max number of links between two nodes, and let $s_{od}$ be the distance between the origin to the destination.

\textbf{Base case:} When $s_{od}=1$, we know that there is only one link from the origin to the destination. 
Thus, there is one path and the probability of traveling on that path is 1.

\textbf{Inductive hypothesis:} Assume this is true for $s_{od} = k$.

\textbf{Induction step:} Let $s_{od} = k+1$, $n$ be the origin node, $n_1, \dots, n_m$ be the nodes that can be reached from the origin in one step, $p_1, \dots, p_m$ be the probabilities from the origin to the respective nodes, $\beta_1, \dots, \beta_m$ as the number of paths for the respective nodes to the destination, $\beta$ be the number of paths for the entire graph, and $P_{n_i d, j}$ be path $j$ from node $n_i$ to the destination.
We know that the distance from nodes $n_1, \dots, n_m$ to the destination is at most $k$ which we know $\sum_{j = 1}^{\beta_i} \prod_{l \in P_{n_i d, j}}p_l = 1$ is true for $1\leq i \leq m$ by the inductive hypothesis.
Thus, we can rewrite $\sum_{j = 1}^\beta \prod_{l \in P_{n d, j}}p_l$ as:
\begin{equation}
    \sum_{i=1}^m p_i  \sum_{j = 1}^{\beta_i} \prod_{l \in P_{n_i d, j}}p_l = \sum_{i=1}^m p_i = 1 
\end{equation}



%Suppose the above equation does not equal 1. Since the sum of path probabilities should be 1 since all commuters must be on one of those paths. 
%This means that there is at least one path that is not included in the summation above. 
%However, we sum over all paths, so this is a contradiction. Thus, $\sum_{j = 1}^\beta \prod_{l \in P_j}p_l$ = 1. 
Now that we have found $\rho$, we can define the expected path flows $\hv$ for acyclic networks with one origin-destination pair as 
\begin{equation}
    \mathbb{E}[\hv] = d_{o,d}\rho
\end{equation}

This is an expectation since we are assuming a proportion $\rho_p$ of the demand travel on path $p$ even though there is the possibility to deviate from $d_{o, d} \rho_p$.

\begin{remark}[Expected path flow]
The flow on path $p$ is similar to the binomial distribution $Bin(d_{o,d}, \rho_p)$ in the acyclic and single demand case. Considering all paths, this would make the multinomial distribution. 
\end{remark}

\subsection{Equivalence between both methods}
\begin{remark}[Equivalence between both methods]
One might want to know if definition \ref{def:UE} and \ref{def:UE_markov} are equivalent (same for definition \ref{def:SO} and \ref{def:SO_markov}).
This is true on the diamond network. 

One might show that this is true in the general case. This is not done here as it is not the primary goal of the present article.
However to show that \ref{def:UE} and \ref{def:UE_markov} are equivalent, we recommend to first show that the user equilibrium in the Markov framework is a feasible flow (this can be done using contradiction and it is true all the time).
Then, we recommend to try to show that $\Fd\subset\bigcup_{\Pr\in\SPr}\Fdp$ using properties (like ergodicity) of Markov chains.

To show that Markov is bigger than UE, take the UE solution and define $\prl = \frac{\fl}{\sum f_e}$. Show that $\prl$ is well define. Show that $f_{ue}$ is a solution of the equation $\fv=\Pr^\top\fv + \P_\o(\de-\de^\top)\mathbf{1}$.

To show that UE is bigger than Markov, take the Markov solution, assume one destination, show that there is no cycle. 
Then try to extend to case with multiple destinations (similar idea).
\todoT{Rephrase.}
\end{remark}

\end{document}



% \subsection{Limitation of static traffic assignment framework}
% \begin{itemize}
%     \item Not realistic if demand changes
%     \item No congestion spill back
% \end{itemize}
% \subsection{Optimization framework for dynamic traffic assignment}
% \begin{itemize}
%     \item Different reward function
%     \item Math formulation based on transition matrix framework \cite{Cabannes2019regret}
% \end{itemize}

% \subsection{SUMO set-up [Jiayi]}

% \section{Optimal dynamic flow allocation using SUMO}
% \begin{itemize}
%     \item grid search method
%     \begin{itemize}
%         \item Heat map plots
%     \end{itemize}
    % \item Convex optimization methods
    % \item Optimal control methods
    % \item Reinforcement learning method
% \end{itemize}




% \section{Introduction}
% \section{Context}
% \subsection{Definitions}
% \begin{itemize}
%     \item STA
%     \item DTA
%     \item Transition matrix
%     \item line graph
% \end{itemize}
% \subsection{Motivations}
% \subsection{The diamond example}
% \section{Flow dynamics in the static case}
% \subsection{STA framework}
% \subsection{Transition matrix framework}
% \section{Optimal flow allocation in the static case}
% \subsection{STA}
% \subsection{Transition matrix}
% \subsection{Equivalence between both}
% \section{Dynamic traffic assignment}
% \begin{itemize}
%     \item Given the transition matrix SUMO compute the flow allocation
% \end{itemize}
% \section{Applications}

% \subsection{New traffic assignment framework using RL}
% \subsection{Data assimilation using regression}

\newpage

\section{Static equilibrium using Markov chains}
\subsection{Node dynamics and dynamical system equation}

covered in later section

\subsection{Equilibrium for a-cyclic graph
Remark on strongly connected graph}



(Perron-Frobenius theorem) [Harry]

\subsection{Example on diamond network}





\section{Introduction}

\todo[inline]{What has been done? What are we doing? Where are we doing it (sections)?}

There has been a considerable amount of work done for traffic flow in terms of both theory and application. 
A couple of the most notable contributions are the Wardrop conditions which describe the conditions for user and social equilibria \cite{wardrop1952road}. 
Using the Wardrop conditions, the static traffic assignment (STA) relates the path flows and links flows to create an optimization problem that minimizes the regret of the network to find a user equilibrium \cite{patriksson}.
Our article finds an equivalent formulation to the STA by using transition matrices and Markov chain properties to find an equilibrium.
For the dynamic traffic case, we will use simulators to aid in our calculations.
 
In our article, we use Markov chains to help us model traffic flow on strongly connected networks. 
This is similar to Google's use of Markov chains to aid in modeling internet congestion \cite{langville2011google}. 
A considerable advantage of using Markov chains is that they can be easily created from data while simultaneously allowing us to exploit properties of Markov chains to identify characteristics of the traffic network \cite{crisostomi2011google}.
For context, we first define all the necessary terms in the beginning, including the diamond graph example.
Next, we outline the STA framework which is explained in \cite{patriksson} in "Flow Dynamics in the Static Case".
Then, we outline the transition matrix framework that we developed and explore some of its properties.
For both, we will then find the optimal flow allocation on a network in which we will then show the equivalence of the two frameworks in "Optimal Flow Allocation in the Static Case".
Next, we move to dynamic models with the help of SUMO to compute the flow allocation from a transition matrix in "Dynamic Traffic Assignment".
Lastly, we combine these ideas in the form of real-world applications.

\subsection{Motivations}
\todo[inline]{Why are we doing this?}
Congestion is a growing modern problem that has monumental social impacts, both directly and indirectly.
Some externalities that come with congestion include but are not limited to loss of time, noise, excessive fuel consumption, and greenhouse gas emissions \cite{barth2009traffic}. 
Although many ways that people have tried to reduce fuel consumption and greenhouse gas emissions involve improving the vehicles themselves, this only makes congestion more bearable without solving the problem \cite{barth2009traffic}.
Our article focuses on an alternative way of addressing this problem by managing traffic networks instead. 
With systems that can predict traffic flow using real-time data, congestion can be dramatically reduced if not avoided \cite{crisostomi2011google}.
Such a system would also reduce pollution from traffic as well \cite{crisostomi2011google}.
These systems could be in the form of navigation apps and autonomous vehicles.  
Furthermore, understanding the flow of traffic can help engineers improve current road networks and design better road networks in the future \cite{perederieieva2013computational}. 
This could be the network itself or strategies such as tolls, speed bumps, and traffic signs.
In all cases, 


\section{Static network flow dynamics}
% \begin{figure}
% \begin{center}
% \begin{tikzpicture}
%  \colorlet{darkgreen}{green!50!black}
% \path (0,0) node(A) [circle,draw]{\vi}
%       (2,-2) node(B) [circle,draw]{\vii}
%       (4,0) node(C) [circle,draw]{\viii};
% \draw[thick,->,color=black] (A) -- (B) node[above,pos=0.5]{\ei};
% \draw[thick,->,color=black] (A) -- (C) node[below,pos=0.5]{\eii};
% \draw[thick,->,color=black] (B) -- (C) node[left,pos=0.5]{\eiii};
% \end{tikzpicture}
% \end{center}
% \caption{Illustration of the framework on a specific road network. 
% $\N=\lb\vi,\vii,\viii\rb$.
% $\L=\lb\ei,\eii,\eiii\rb$ where $\ei=(\vi,\vii),\ \eii=(\vi,\viii)$ and $\eiii=(\vii,\viii)$.
% $\P_{\vi,\viii}=\lb(\ei,\eiii),(\eii)\rb$.
% If $\p=(\ei,\eiii)\in\P_{\vi,\viii}$ then $\dep=(1,0,1)$.
% $\P=\P_{\vi,\vi}\times\P_{\vi,\vii}\times\P_{\vi,\viii}\times
% \P_{\vii,\vi}\times\P_{\vii,\vii}\times\P_{\vii,\viii}\times
% \P_{\viii,\vi}\times\P_{\viii,\vii}\times\P_{\viii,\viii}=
% \lb(\ei),(\eii),(\eiii),(\ei,\eiii)\rb$. If 100 travelers want to go from $\vi$ to $\viii$ then $\Fd = \lb(x,100-x,x),\ x\in[0,100]\rb$.
% }
% \end{figure}

\subsection{Road network flow as Markov chain.}

\todo[inline]{Put a small explication of what we are doing}

In this article, we will be modeling networks as Markov chains and using their connection with graph theory to understand flow in networks.
Several necessary concepts that we will use are defined below.

\begin{definition}[Stochastic process \cite{langville2011google}]
A stochastic process is a set $\{X_t\}_{t = 0}^\infty$ where each $X_t$ is a random variable whose range is $\{S_i\}_{i \in A}$ where $A$ is a set.
\end{definition}

\begin{remark}
In this article, we define the set $\{S_i\}_{i \in A}$ as $\N$ for graphs which we will start to use in the next definition.
\end{remark}

\begin{definition}[Markov chain \cite{langville2011google}]
Markov chains are stochastic processes that satisfies the following property for $i_0, \dots, i_{t+1}, j \in \N$:
\begin{equation}
    P(X_{t+1} = j | X_{t} = i_t, X_{t-1} = i_{t-1}, \dots, X_0 = i_0) = P(X_{t+1} = j | X_{t} = i_t)
\end{equation}
\end{definition}

% \begin{definition}[Node]
% Nodes are equivalent to vertices in graph theory.
% \end{definition}

% \begin{definition}[Link]
% Links are equivalent to directed edges from origin node $n_o$ to destination node $o_d$.
% \end{definition}

% \begin{definition}[Graph]
% Graph $\G$ is the relationship of a set of nodes $N$ described by a set of links $L$. In our case, we consider only directed graphs. The nodes represent the intersections, and the links represent the roads and the direction they go.
% \end{definition}

% \begin{remark}[Graph]
% The terms graph and network will be used interchangeably.
% \end{remark}


\todo[inline]{See if everything below is needed. Try to put as much references to literature as possible.}

\begin{definition}[Transition probability \cite{langville2011google}] 
For nodes $i, j, X_i, X_{t - 1} \in \N$ and time $t \in \mathbb{N}_0$, the transition probability $p_{ij}(t)$ is:
\begin{equation}
p_{ij}(t) = P(X_t = j | X_{t-1} = i) 
\end{equation}
\end{definition}

\begin{remark}[Transition probability \cite{langville2011google}]
In this article, transition probabilities do not vary with time, so we define $p_{ij} := p_{ij}(t) \quad \forall t \in \mathbb{N}_0$. This is known as a stationary Markov chain \cite{langville2011google}.  
\end{remark}

\begin{definition}[Aperiodic Markov chains \cite{bertsekas2008introduction}]
A Markov chain is aperiodic if and only if there exists a time $t\in \mathbb{N}_0$ such that:
\begin{equation}
    P(X_t = j | X_0 = i) > 0 \quad \forall i, j \in \N
\end{equation}
\end{definition}

%\begin{remark}[Strongly connected graph]
%We will only explore strongly connected graphs in this article.
%\end{remark}

% \begin{definition}[Demand]
% Demand $d_{ij}$ is a nonnegative number of commuters entering the network at node $n_i \in \N$ and exiting the network at node $n_j \in \N$.  
% \end{definition}

% \begin{definition}[Demand matrix]
% The demand matrix $\mathbf{M}$ is a matrix containing the demand $d_{ij}$ for all node pairs $(n_i, n_j)$ for a network where $n_i \in \N$ is the entrance and $n_j \in \N$ is the exit.
% \begin{equation}
%     \mathbf{M} := [dij]
% \end{equation}
% \end{definition}

% \begin{definition}[Flow]
% Flow is the nonnegative number of commuters on a link. The flow on all links is compiled into the vector $\vec{f}$.
% \end{definition}

\begin{definition}[Adjacency matrix of a directed graph \cite{Godsil2001algebraic}]
\begin{equation}
    A = [a_{ij}] \text{ where  } 
    a_{ij} = 
    \begin{cases} 
      1 & \text{if there is a link from node $i \in \N$ to node $j \in \N$} \\
      0 & \text{else} 
  \end{cases}
\end{equation}
\end{definition}

\begin{definition}[Origin matrix]
\begin{equation}
    O = [\omega_{li}] \text{ where  } 
    \omega_{li} = 
    \begin{cases} 
      1 & \text{if node $i \in \N$ is the origin of link $\l \in \L$} \\
      0 & \text{else} 
  \end{cases}
\end{equation}
\end{definition}

\begin{definition}[Transition matrix \cite{Godsil2001algebraic}]
The transition matrix $P_{|\N|\times|\N|}$ of a graph $\G$ is a  matrix that contains information of all nodes, all links, and all transition probabilities of $\G$. 
All entries in $P$ are nonnegative, and entries of each row sum to 1 i.e. $P \mathbbm{1} = \mathbbm{1}$. 
Rows represent the nodes where links begin, and columns represent the nodes where links end. 

\begin{equation}
    P :=[p_{ij}] \quad \forall i, \forall j \in\N
\end{equation}
\end{definition}

\begin{remark} [Transition matrix]
Transition matrices are sometimes called stochastic matrices or probability transition matrices.
\end{remark}

\begin{remark} [Transition matrix]
Note that $P$ is similar to $A$ in that instead of entries being 0 or 1, each 1 is replaced by a probability of traveling on that link. 
\end{remark}

\begin{definition}[Strongly connected graph \cite{Godsil2001algebraic}]
$\G$ is a strongly connected graph if and only if for all $n_i,n_j \in \N$,  $n_i$ is reachable from $n_j$ and vice versa.
\end{definition}

\begin{remark}[Strongly connected graph \cite{langville2011google}]
Irreducible Markov chains can be represented as strongly connected graphs.
\end{remark}

\begin{definition}[Line graph \cite{Godsil2001algebraic}]
The line graph $L(\G)$ is the graph formed from swapping the roles of nodes and links in $\G$. Each link in $\G$ is represented as a node in $L(\G)$, and each intersection of two links in $\G$ is a link in $L(\G)$. The above definitions apply in a similar way, and the following are notations we give to line graphs:

\begin{itemize}
    \item Nodes: $L(\N)$
    \item Links: $L(\L)$
    \item Adjacency matrix: 
        \begin{equation}
            L(A) = [a_{ij}] \quad \forall i, \forall j \in L(\N)
        \end{equation}
    \item Origin Matrix:
        \begin{equation}
            L(O) = [\omega_{li}] \quad \forall l \in L(\L), \forall i \in L(\N)
        \end{equation}
    \item Transition matrix:
        \begin{equation}
            L(P) := [p_{kl}] \quad \forall k, \forall l \in L(\N)
        \end{equation}
\end{itemize}
\end{definition}

\begin{remark}[Line graph]
Note that $L(\N) = \L$.
In addition, the probability associated with each link in $L(\G)$ is the probability of traveling on the destination link in $\G$. 
\end{remark}

\begin{remark}[Line graph]
The formal name is line graph, but some articles such as \cite{crisostomi2011google} and \cite{porta2006network} use the term dual graph instead. Note that the definition of the dual graph (in \cite{crisostomi2011google} and \cite{porta2006network}) is not equivalent to the notion of dual graph from a graph theory point of view where the faces in the original graphs are nodes in the dual graph.
\end{remark}

%In other words, each link in $\G$ is represented as a node in $L(\G)$, and each link in $L(\G)$ is represented as a node in $\G$. 
%However, the number of links $L(\G)$ do not match the number of nodes in $\G$.


\begin{definition}[Probability vector]
The probability vector $\mathbf{p} \in \mathbb{R}^{|\L|}$ is defined as follows:
\begin{equation}
    \mathbf{p} = [p_{ij}]_{i,j \in \N}
    \text{ such that $p_{ij} > 0$}
\end{equation}
\end{definition}

\begin{remark}[Probability vector]
The order of the transition probabilities should be in the same order as the rows of $O$.
\end{remark}

\begin{definition}[$diag(\cdot)$]
Let $\mathbf{v} = \begin{bmatrix}
        v_1 \\
        \vdots \\ 
        v_{k} 
    \end{bmatrix}$. Then,
    \begin{equation}
        diag(\mathbf{v}):=\begin{bmatrix}
        v_1    &0       &\dots  &0\\
        0      &\ddots  &       &\vdots\\
        \vdots &        &\ddots &0\\ 
        0      &\dots   &0      &v_{k}
        \end{bmatrix}
    \end{equation}
\end{definition}

\begin{definition}[$A_{ln}$]
$A_{ln}$ is equivalent to replacing all positive entries in $A$ with the natural log of each entry. Let $A = [a_{ij}]$, then:
\begin{equation}
    A_{ln} := [a_{ij}'] \text{ where } 
    a_{ij}' = \begin{cases} 
      ln(a_{ij}) & \text{if $a_{ij} > 0$} \\
      0 & \text{else} 
  \end{cases}
\end{equation}
\end{definition}

\begin{remark}[$A_{ln}$]
This is not to be confused with $ln(A)$ which is a different operation in linear algebra.
\end{remark}

\begin{definition}[$A_{e}$]
$A_{e}$ is equivalent to replacing all entries in $A$ with the exponential of each entry. Let $A = [a_{ij}]$, then:
\begin{equation}
    A_{e} := [e^{a_{ij}}]
\end{equation}
\end{definition}

\begin{remark}[$A_e$]
This is not to be confused with $e^A$ which is a different operation in linear algebra.
\end{remark}

\begin{definition}[Mean first passage time \cite{bertsekas2008introduction}]
The mean first passage time $t_{i}$ from node i to node s is solution to the following system of equations:
\begin{equation}
    \begin{split}
        t_{s} &= 0 \\
        t_{i} &= 1 + \sum_{j \in \N} p_{ij}t_j
    \end{split}
\end{equation}
\end{definition}

%\begin{definition}[Kemeny constant \cite{crisostomi2011google}]
%Let $t_{ij}$ be the mean first passage time from node i to node s, and let $\vec{f}$ be the distribution of flow at equilibrium, then:
%\begin{equation}
%    K = 
%\end{equation}
%\end{definition}


%\begin{definition}[Inverse multiplicity matrix]
%Inverse multiplicity matrix $M$ is a diagonal matrix whose entries are the multiplicative inverse of the in-degree of each node in the line graph. Let $m_l$ be the in-degree of node $l$ in the line graph.
%\begin{equation}
%    M :=\begin{bmatrix}
%        \frac{1}{m_1}    &0       &\dots  &0\\
%        0      &\ddots  &       &\vdots\\
%        \vdots &        &\ddots &0\\ 
%        0      &\dots   &0      &\frac{1}{m_{k}} 
%        \end{bmatrix}
%\end{equation}
%\end{definition}


% \begin{definition}[line graph \cite{porta2006network}]
% The line graph $L(\G)$ is the graph formed from swapping the roles of nodes and links in $\G$. 
% \end{definition}

% In other words, each link in $\G$ is represented as a node in $L(\G)$, and each link in $L(\G)$ is represented as a node in $\G$. However, the number of links $L(\G)$ do not match the number of nodes in $\G$. The probability associated with each link in $L(\G)$ is the probability of traveling on the destination link in $\G$. We define $L(\mathbf{P})$ as the transition matrix associated with $L(\G)$. Let $L$ be the set of links in $\G$, which is also the set of nodes in $L(\G)$.

% \begin{equation}
%     L(\mathbf{P}) := [\tilde{p}_{kl}] \text{, where $\tilde{p}_{kl}$ is the probability of traveling on link $l$ from link $k$ } \forall k, l \in L
% \end{equation}

% \begin{remark}[line graph]
% Note that the definition of the line graph (in \cite{porta2006network}) is not equivalent to the notion of line graph from a graph theory point of view where the faces in the original graphs are nodes in the line.
% \end{remark}

\subsection{The Diamond Example}
We will continuously use the diamond graph as examples for concepts. This network is shown below.

\begin{figure}[h]
    \centering
    \begin{tikzpicture}
    \tikzset{vertex/.style = {shape=circle,draw,minimum size=1.5em}}
    \tikzset{edge/.style = {->,> = latex'}}
    % vertices
    \node[vertex] (A) at  (0,0) {A};
    \node[vertex] (B) at  (3,1.5) {B};
    \node[vertex] (D) at  (6,0) {D};
    \node[vertex] (C) at  (3,-1.5) {C};
    %edges
    \path[->] (A) edge node[above] {$p_{AB}$} (B);
    \path[->] (A) edge node[below] {$p_{AC}$} (C);
    \path[->] (B) edge node[left] {$p_{BC}$} (C);
    \path[->] (B) edge node[above] {$p_{BD}$} (D);
    \path[->] (C) edge node[below] {$p_{CD}$} (D);
    \path[->] (D) edge [bend left = 100] node[below] {$p_{DA}$} (A);
    \end{tikzpicture}
    \caption{To do}
    \label{fig:diamond_network}
\end{figure}



Applying several relevant previous definitions to the diamond example, we get the following equations:

\begin{equation}
  \N = \{A, B, C, D\}
\end{equation}

\begin{equation}
  \L = \{DA, AB, AC, BC, BD, CD\}
\end{equation}

\begin{equation}
    O = \begin{bmatrix}
        0 &0 &0 &1 \\
        1 &0 &0 &0 \\
        1 &0 &0 &0 \\
        0 &1 &0 &0 \\
        0 &1 &0 &0 \\
        0 &0 &1 &0 
    \end{bmatrix}
\end{equation}

\begin{equation}
    P = \begin{bmatrix}
        0 &p_{AB} &p_{AC} &0 \\
        0 &0 &p_{BC} &p_{BD} \\
        0 &0 &0 &p_{CD} \\
        p_{DA} &0 &0 &0  
    \end{bmatrix}
\end{equation}

\begin{equation}
    \vec{p} = \begin{bmatrix}
        p_{DA} \\
        p_{AB}  \\
        p_{AC}  \\
        p_{BC} \\
        p_{BD} \\
        p_{CD} 
    \end{bmatrix}
\end{equation}

The line graph of the diamond graph and the corresponding transition matrix are shown below where nodes are in the approximate positions of the links in the diamond graph.

\begin{figure} [h]
    \centering
    \begin{tikzpicture}
    \tikzset{vertex/.style = {shape=circle,draw,minimum size=1.5em}}
    \tikzset{edge/.style = {->,> = latex'}}
    % vertices
    \node[vertex] (a) at  (3, -2.5) {a};
    \node[vertex] (b) at  (1.5,1) {b};
    \node[vertex] (c) at  (1.5,-1) {c};
    \node[vertex] (d) at  (3,0) {d};
    \node[vertex] (e) at  (4.5,1) {e};
    \node[vertex] (f) at  (4.5,-1) {f};
    %edges
    \path[->] (a) edge [bend left = 100] node[left] {$p_{AB}$} (b);
    \path[->] (a) edge node[above] {$p_{AC}$} (c);
    \path[->] (b) edge node[below] {$p_{BC}$} (d);
    \path[->] (b) edge node[above] {$p_{BD}$} (e);
    \path[->] (c) edge node[above] {$p_{CD}$} (f);
    \path[->] (d) edge node[above] {$p_{CD}$} (f);
    \path[->] (e) edge [bend left = 100] node[right] {$p_{DA}$} (a);
    \path[->] (f) edge node[above] {$p_{DA}$} (a);
    \end{tikzpicture}
    \caption{The network considered as an example}
    \label{fig:network}
\end{figure}

\begin{equation}
    L(P) = \begin{bmatrix}
        0 &p_{AB} &p_{AC} &0 &0 &0\\
        0 &0 &0 &p_{BC} &p_{BD} &0\\
        0 &0 &0 &0 &0 &p_{CD}\\
        0 &0 &0 &0 &0 &p_{CD}\\
        p_{DA} &0 &0 &0 &0 &0\\
        p_{DA} &0 &0 &0 &0 &0
    \end{bmatrix}
\end{equation}


% \subsection{STA Framework}

\subsubsection{Flow dynamics as a Markov chain}

Both $\G$ and $L(\G)$ can be viewed as Markov chains.
In $\G$, the nodes are intersections and links are roads between intersections with transition probabilities determining the likelihood that a commuter chooses one road over others at an intersection. 
In $L(\G)$, the nodes are links in $\G$ and links are every possible intersection of two roads.
Thus, transition probabilities determine the likelihood of going from one road to another.
In fact, transition probabilities in $L(\G)$ come from transition probabilities in $\G$.
The transition probability of a link in $L(\G)$ is the same as the probability going from the previous road to the current road.
To make this more concrete, let us use the diamond example.
The probability associated with link $l \in L(\L)$ that joins nodes $b$ and $d$ is the probability of going from the road represented by $b$ in $\G$ to the road represented by $d$ in $\G$.
This probability is the same as the probability of taking road $d$ after reaching the intersection from taking road $b$.

Another point of clarification is the demand matrix $\de$. 
In our model, there are no commuters in the network at the beginning.
Then, the demand $\sum_{j \in \N}d_{ij}$ enters the network at node $i \in \N$ at each timestep.
Demand leaving the network is slightly different.
A maximum of $\sum_{i \in \N}d_{ij}$ leaves the network from node $j \in \N$ at  at each timestep.
However, since there cannot be a negative number of commuters, the demand leaving the network never exceeds the total flow into $j$.
More formally, the demand that that leaves the network at node $j$ is $min\{ \sum_{i \in \N}d_{ij}, \sum_{i \in \N}f_{ij} \}$.
Consequently, the number of commuters in the network monotonically increases until $\sum_{i \in \N}f_{ij} \geq \sum_{i \in \N}d_{ij}$ for all $j$.
At equilibrium, the flows on all roads do not change with time, implying demand entering the network is equal to the demand leaving the network.

The reason $L(\G)$ is useful is that by representing roads as nodes rather than links, we can use Markov chains to calculate how flow shifts from one node to the next, or from one road to the next, instead of flow of an intersection which is captured in $\G$.

There are several advantages of using Markov chains.
Under this model, we can use properties of Markov chains which will be handy in the next several sections, most notably, the properties of irreducibility and periodicity.
Additionally, this model allows us to combine different modes of transportation   into one network \cite{faizrahnemoon2016real}.
For instance, cars, trains, and other forms of travel can be placed in the same network without having to treat them differently.
Markov chains can also extend to larger networks, so scaling is not a significant issue \cite{crisostomi2011google}.
Furthermore, another benefit is the transition matrix, which captures a nontrivial amount of information about the network which we will explore.

The limitations of this model are that we make time discrete and that we assume that at each timestep, commuters travel from one node to the next. 
Additionally, we assume that each commuter acts independently, meaning commuters choose routes without considering other commuters' choices and without considering previous road choices \cite{crisostomi2011google}.
Another limitation is that we treat demand and transition probabilities as constants, an inherent weakness with the static traffic assignment model.

\todo[inline]{Explain this a little bit more. Refer to dynamical system evolution modeled as Markov Chain (for the $\fv=\T^\top\fv$). And refer to fluid mechanism for the $\fv=diag(p)\mathbf{O}(\de-\de^\top)$}

Assuming that the network is strongly connected, the equilibrium flow $\mathbf{f}_{eq}$ is:
\begin{equation}
    \mathbf{f}_{eq} = L(P)^\top \mathbf{f}_{eq} + diag(\mathbf{p}) O [\de-\de^\top]\mathbbm{1}
\end{equation}

The $L(P)^\top \mathbf{f}_{eq}$ term comes directly from the property of Markov chains in which the transition matrix is used to advance one timestep \cite{langville2011google}. 
In other words, multiplication of $L(P)$ shifts the commuters from one node to the next.
Before addressing the next part of the equation, there are some conventions of Markov chains that we must address:

\begin{remark}[Transition matrices conventions]
In some texts using Markov chains, row vectors are used, so if $P$ is the transition matrix and $\mathbf{x}_t$ is the distribution of commuters in the network at time $t$ organized in a row vector, then $\mathbf{x}_{t+1} = \mathbf{x}_t P$. 
However, for column vectors, we can take the transpose of both sides to get $\mathbf{y}_{t+1} = P^\top \mathbf{y}_t$ for $\mathbf{y}_t := \mathbf{x}_t^\top$ and $\mathbf{y}_{t+1} := \mathbf{x}_{t+1}^\top$.
\end{remark}

The $diag(\mathbf{p})O[\de-\de^\top]\mathbbm{1}$ term is a bit more complicated.
This stems from the flow conservation law which states that assuming no commuters entering the network, $f_{v_{in}, t} = f_{v_{out}, t + 1}$ where $f_{v_{in}, t} = \sum_{u \in \N} f_{uv, t}$, $f_{v_{out}, t+1} = \sum_{w \in \N} f_{vw, t+1}$, and $t \in \mathbb{N}_0$ is the timestep \cite{patriksson}. 
In other words, the flow into node $v$ is equal to the flow out of $v$ at the next timestep for all $v \in\N$ \cite{patriksson}. 
However, we know that at equilibrium, $\mathbf{f}_{eq}$ does not change with time.
As a result, we can simplify the notation of $f_{v_{in}, t}$ to $f_{v_{in}}$ and $f_{v_{out}, t + 1}$ to $f_{v_{out}}$, as long as the equilibrium state is being studied.
With demand, $f_{v_{in}} = \sum_{u}f_{uv} + \sum_{\tilde{u}}d_{v \tilde{u}}$ and $f_{v_{out}} = \sum_{w}f_{vw} + \sum_{\tilde{w}}d_{\tilde{w} v}$ for $v, w, \tilde{v}, \tilde{w} \in\N$. 
This can be summarized into one equality:

\begin{equation}
    \sum_{u}f_{uv} + \sum_{\tilde{u}}d_{v\tilde{u}} = \sum_{w}f_{vw} + \sum_{\tilde{w}}d_{\tilde{w}v}
\end{equation}

If we want the flow $f_{vn}$ of the link from $v$ to $n \in\N$, we can rearrange the above equation and use a probability fact to find $f_{vn}$:

\begin{equation}
\begin{split}
\sum_{u}f_{uv} + \sum_{\tilde{u}}d_{v\tilde{u}} &= \sum_{w}f_{vw} + \sum_{\tilde{w}}d_{\tilde{w}v} \\
p_{vn}\sum_{w}f_{vw} &= p_{vn}\left[\sum_{u}f_{uv} + \sum_{\tilde{u}}d_{v\tilde{u}} - \sum_{\tilde{w}}d_{\tilde{w}v}\right] \\
f_{vn} &= p_{vn}\left[\sum_{u}f_{uv} + \sum_{\tilde{u}}d_{v\tilde{u}} - \sum_{\tilde{w}}d_{\tilde{w}v}\right] &\text{since $p_{vn} = \frac{f_{vn}}{\sum_{w}f_{vw}}$}\\
\end{split}
\end{equation}

Notice that $L(\mathbf{P})^\top\vec{f}$ is represented by $p_{vn}\sum_{u}f_{uv} \forall v \in \L$ since this is a transfer of flow in one timestep. 
Similarly, we can make a connection to $p_{vn}\left[\sum_{\tilde{u}}d_{v\tilde{u}} - \sum_{\tilde{w}}d_{\tilde{w}v}\right]$ as $diag(\vec{p})\mathbf{O}[\de-\de^\top]\mathbbm{1}$.
The connection is made more clear below. 
Note that entries equal to 1 in $\mathbf{O}$ are not all lined up (refer to the definition of the origin matrix). 
Let $a, b, \dots,\epsilon$ represent links, $n$ be the number of nodes, and $k_a, k_b, \dots, k_\epsilon$ are origin nodes of links $a, b, \dots,\epsilon$ where $1 \leq k_a, k_b, \dots, k_\epsilon \leq n$:
%Suppose entries of $\vec{p}$ is organized such that all links are grouped by their origin node in ascending order. Although this is not necessary in practice, it gives

\begin{equation}
\begin{split}
    diag(\vec{p})\mathbf{O}
    &= \begin{bmatrix}
        p_a    &0       &\dots  &0\\
        0      &p_b     &       &\vdots\\
        \vdots &        &\ddots &0\\ 
        0      &\dots   &0      &p_{\epsilon} 
    \end{bmatrix}
    \begin{bmatrix}
        0 &\dots &1 &\dots &0 \\
        0 &\dots &1 &\dots &0 \\
        & &\vdots \\
        0 &\dots &1 &\dots &0
    \end{bmatrix} 
    = \begin{bmatrix}
        0 &\dots &p_a &\dots &0 \\
        0 &\dots &p_b &\dots &0 \\
        & &\vdots \\
        0 &\dots &p_{\epsilon} &\dots &0
    \end{bmatrix}
\end{split}
\end{equation}

\begin{equation}
\begin{split}
    \de-\de^\top 
    &= \begin{bmatrix}
        0       &d_{12} &\dots  &d_{1n} \\
        d_{21}  &\ddots &     &\vdots \\
        \vdots  &       &\ddots &d_{[n-1]n}\\
        d_{n1}  &\dots  &d_{n[n-1]} &0
    \end{bmatrix}
    -
    \begin{bmatrix}
        0       &d_{21} &\dots  &d_{n1} \\
        d_{12}  &\ddots &     &\vdots \\
        \vdots  &       &\ddots &d_{n[n-1]}\\
        d_{1n}  &\dots  &d_{[n-1]n} &0
    \end{bmatrix} \\
    &= \begin{bmatrix}
        0               &d_{12} - d_{21}    &\dots                      &d_{1n} - d_{n1} \\
        d_{21} - d_{12} &\ddots             &                           &\vdots \\
        \vdots          &                   &\ddots                     &d_{[n-1]n} - d_{n[n-1]} \\
        d_{n1} - d_{1n} &\dots              &d_{n[n-1]} - d_{[n-1]n}    &0
    \end{bmatrix}
\end{split}
\end{equation}

\begin{equation}
\begin{split}
    diag(\vec{p})\mathbf{O}[\de-\de^\top]\mathbbm{1} &= \begin{bmatrix}
        p_a\sum_{\tilde{u}\in\N}\left(d_{k_a\tilde{u}} - d_{\tilde{u}k_a}\right) \\
        p_b\sum_{\tilde{u}\in\N}\left(d_{k_b\tilde{u}} - d_{\tilde{u}k_b}\right) \\
        \vdots \\
        p_\epsilon\sum_{\tilde{u}\in\N}\left(d_{k_\epsilon\tilde{u}} - d_{\tilde{u}k_\epsilon}\right)
    \end{bmatrix}  = \begin{bmatrix}
        p_a\left[\sum_{\tilde{u}\in\N}d_{k_a\tilde{u}} - \sum_{\tilde{w}\in\N}d_{\tilde{w}k_a}\right] \\
        p_b\left[\sum_{\tilde{u}\in\N}d_{k_b\tilde{u}} - \sum_{\tilde{w}\in\N}d_{\tilde{w}k_b}\right] \\
        \vdots \\
        p_\epsilon\left[\sum_{\tilde{u}\in \N}d_{k_\epsilon\tilde{u}} - \sum_{\tilde{w}\in \N}d_{\tilde{w}k_\epsilon}\right]
    \end{bmatrix}
\end{split}
\end{equation}

Now, let us make sure that entries in the above vector sum to zero:
\begin{equation}
\begin{split}
    \begin{bmatrix}
        1 &1 &\dots &1
    \end{bmatrix}
    \begin{bmatrix}
        p_a\left[\sum_{\tilde{u}\in \N}d_{k_a\tilde{u}} - \sum_{\tilde{w}\in \N}d_{\tilde{w}k_a}\right] \\
        p_b\left[\sum_{\tilde{u}\in \N}d_{k_b\tilde{u}} - \sum_{\tilde{w}\in \N}d_{\tilde{w}k_b}\right] \\
        \vdots \\
        p_\epsilon\left[\sum_{\tilde{u}\in \N}d_{k_\epsilon\tilde{u}} - \sum_{\tilde{w}\in \N}d_{\tilde{w}k_\epsilon}\right]
    \end{bmatrix}
    %&= \sum_{l \in\L} \sum_{\tilde{u}\in \N}p_ld_{k_l\tilde{u}} - \sum_{m \in\L} \sum_{\tilde{w} \in \N} p_ld_{\tilde{w}k_l} \\
    &= \sum_{\tilde{u}\in \N}\sum_{l \in\L} p_ld_{k_l\tilde{u}} - \sum_{\tilde{w} \in \N}\sum_{m \in\L}  p_ld_{\tilde{w}k_l} \\
    &= \sum_{\tilde{u}\in \N}\sum_{\tilde{v}\in \N} d_{\tilde{v}\tilde{u}} - \sum_{\tilde{w} \in \N}\sum_{\tilde{x}\in \N} d_{\tilde{x}\tilde{w}} = 0
\end{split}
\end{equation}

The third equality comes from the fact that the sum of outgoing probabilities of any node equals 1:

\begin{equation}
\begin{split}
    \sum_{\tilde{u}\in \N}\sum_{l \in\L} p_ld_{k_l\tilde{u}} &= \sum_{\tilde{u}\in \N}\sum_{\tilde{v} \in \N}\sum_{\tilde{w} \in \N} p_{\tilde{v}\tilde{w}}d_{\tilde{v}\tilde{u}} = \sum_{\tilde{u}\in \N}\sum_{\tilde{v} \in \N}\left[d_{\tilde{v}\tilde{u}}\sum_{\tilde{w} \in \N} p_{\tilde{v}\tilde{w}}\right] = \sum_{\tilde{u}\in \N}\sum_{\tilde{v} \in \N}d_{\tilde{v}\tilde{u}}
\end{split}
\end{equation}

\subsubsection{Perron-Frobenius Theorem}
First, we need to show that if $\G$ is strongly connected, then $L(\G)$ is strongly connected.
We do this by proving the contrapositive.

\begin{align*}
\text{$L(\G)$ is not strongly connected} 
&\text{$\implies \exists$ nodes in $L(\G): l_1, l_2 \in\L$ s.t. there is no path from $l_1$ to $l_2$} \\
&\text{$\implies \exists$ links in $\G: l_1, l_2 \in\L$ s.t. there is no path from $l_1$ to $l_2$ } \\
&\text{$\implies$ there is no path from $n_1$ to $n_2$ s.t. $n_1, n_2$ are origins of $l_1, l_2$} \\
&\text{$\implies$ $\G$ is not strongly connected}
\end{align*}


Since $L(\G)$ is strongly connected, $L(\G)$ is an irreducible Markov chain. 
Thus, $L(\mathbf{P})$ has only nonnegative entries and is irreducible. 
With these properties, we can use the Perron-Frobenius Theorem to show that $L(\mathbf{P})^\top$ has an eigenvalue of 1. 
The importance of an eigenvalue of 1 is that it shows the existence of equilibria where at each timestep, the flow on each link does not change. 
Additionally, the Perron-Frobenius Theorem allows us to show that the eigenspace corresponding to the eigenvalue of 1 is one-dimensional, and all entries have the same sign. 
In other words, there exists an $\vec{f}$ such that $\vec{f} = L(\mathbf{P})^\top\vec{f}$ where all entries of $\vec{f}$ is nonnegative. 

The proof is shown below. Let $r$ be the spectral radius of $L(\mathbf{P})$.

\begin{align*}
\text{$\G$ is strongly connected} 
&\text{$\implies L(\G)$ is strongly connected} \\
&\text{$\implies r = 1$ and $r$ is the largest real eigenvalue of $L(\mathbf{P})$ \cite{langville2011google}}\\
&\text{$\implies$ 1 is the spectral radius and the largest real eigenvalue of $L(\mathbf{P})^\top$} \\
&\text{$\implies \exists \vec{f}$ s.t. $\vec{f} = L(\mathbf{P})^\top\vec{f}$}
\end{align*}


Additionally, by the Perron-Frobenius Theorem, the left and right eigenspaces of $L(\mathbf{P})$ corresponding to $r = 1$ are one-dimensional. 
The right eigenvector of $L(\mathbf{P})^\top$ corresponding to the eigenvalue 1 is the called the stationary distribution \cite{langville2011google}.
Let us establish the relationship of eigenvectors between a square matrix $M$ and its transpose $M^\top$. Suppose $\vec{v}$ is the eigenvector corresponding to the eigenvalue $\lambda$ for $M$:

\begin{equation}
    \vec{v}^\top M^\top = (M\vec{v})^\top = (\lambda \vec{v})^\top = \lambda \vec{v}^\top
\end{equation}

Thus, the right eigenvector of $M$ is the transpose of the left eigenvector of $M^\top$.
Since we also know $\vec{f}$ s.t. $\vec{f} = L(\mathbf{P})^\top\vec{f}$, $span(\vec{f})$ is the right eigenspace of $L(\mathbf{P})^\top\vec{f}$ corresponding to $r$.
In fact, by the property of transition matrices, $L(\mathbf{P})\mathbbm{1} = \mathbbm{1}$, so $span(\mathbbm{1})$ is the right eigenspace corresponding to $r$.
In turn, $span(\mathbbm{1}^\top)$ is the left eigenspace corresponding to $r$ for $L(\mathbf{P})^\top$.

Let the simplified form of the flow equation be:

\begin{equation}
    \vec{f} = L(\mathbf{P})^\top\vec{f} + \vec{b}
\end{equation}

This can be rewritten as

\begin{equation}
\begin{split}
    (\mathbf{I}-L(\mathbf{P})^\top)\vec{f} &= \vec{b}\\ 
    A\vec{f} &= \vec{b} \text{ where $A := \mathbf{I}-L(\mathbf{P})^\top$}
\end{split}
\end{equation}

Let $S$ be the solutions to $A\vec{f} = \vec{b}$, then $S=\{\vec{x}^* + Null(A):A\vec{x}^*=\vec{b}\}$ which we will now prove. 
Since there is some flow $\vec{f_0}$ such that $L(\mathbf{P})^\top\vec{f_0} = \vec{f_0}$, then $(I-L(\mathbf{P})^\top)\vec{f_0} = \vec{0}$. 
This means $Null(A) = Span(\vec{f_0})$ by the one-dimensional argument from the Perron-Frobenius Theorem. 
We know that $\vec{b}\perp Null(A^\top)$ since $\mathbbm{1}^\top\vec{b} = 0$ as shown before, so $\vec{b}\in Im(A)$ because $Im(A)  \bigoplus^\perp Null(A^\top)$. 
As a result, we know that there exists is an $\vec{x}^*$ such that $A\vec{x}^* = \vec{b}$.
Thus, $\vec{x}^*\in S$.

Take $\vec{x}\in S$. 
Then, $A\vec{x} = \vec{b}$, but we also know that $A\vec{x}^*=\vec{b}$.
As a result, $A(\vec{x}-\vec{x}^*) = A\vec{x} - A\vec{x}^* = \vec{b} - \vec{b} = \vec{0}$. 
Since $(\vec{x}-\vec{x}^*)\in Null(A)$, $\vec{x} \in S \implies (\vec{x}-\vec{x}^*) \in Null(A)$. 
Thus, $S\subset (\vec{x}^* + Null(A))$.

Now, let's take $\vec{x}\in (\vec{x}^* + Null(A))$. 
$\vec{x} = \vec{x}^* + \vec{v}$ with $\vec{v} \in Null(A)$. 
$A\vec{x} = A(\vec{x}^* + \vec{v}) = A\vec{x}^* + A\vec{v} = A\vec{x}^* + \vec{0} = \vec{b}$. So $(\vec{x}^* + Null(A))\subset S$.

Therefore: $S=\{\vec{x}^* + Null(A):A\vec{x}^*=\vec{b}\}$.

%To show that $Im(A)  \bigoplus^\perp N(A^\top)$: let $x\in Im(A)$, therefore $x=Ab$ and for all $v\in N(A^\top)$: $x^\top v = (Ab)^\top v = (b^\top A^\top) v = (b^\top) (A^\top v) = b^\top 0 = 0$.
%Definition of $A^\top$: is $A^\top = M$ such that for every $x, y$, $<Ax, y> = <x , My>$.

%Solve $Ax=b$. Set of solution is denoted $S$.
%\begin{enumerate}
%    \item find that $b\perp N(A^\top)$.
%    \item find $N(A)$.
%\end{enumerate}

%Because $b\perp N(A^\top)$ and $Im(A)  \bigoplus^\perp N(A^\top)$, then $b\in Im(A)$: $\exists x^*$ such that $A x^* = b$.
%This gives you $x^*\in S$, therefore $S\neq \empty$.




\ 
 
In our case: PF gives that $N(A^\top) = span (\mathbf{1})$. So 1. is equivalent to show that $\mathbf{1}^\top b = 0$ \todo[inline]{To do Harry} (this is actually the flow conservation law for the demand).

PF gives that $N(A) = Span (f_0)$ with $f_0>0$.

This gives you that the set of solution of $\vec{f} = L(\mathbf{P})^\top\vec{f} + diag(\vec{p})\mathbf{O}[\de-\de^\top]\mathbbm{1}$ is $f^* + \alpha f_0$. Because $f_0 > 0$, there exist $f\geq 0$, such that $\vec{f} = L(\mathbf{P})^\top\vec{f} + diag(\vec{p})\mathbf{O}[\de-\de^\top]\mathbbm{1}$. Now the one that correspond to the solution is the smallest one (e.g. $\min \|f\|_2$).

\subsubsection{Periodicity}
\todo[inline]{define period and irreducibility}
For each network, we can represent it as an irreducible Markov chain since the network is strongly connected. 
For irreducible Markov chains, we can categorize them as aperiodic or periodic. 
Aperiodic graphs have the property the length of every cycle for each state has a greatest common divisor of 1, whereas for periodic graphs, the greatest common divisor of the length of all cycles for each state is greater than 1.

Aperiodic graphs have the property that as the number of timesteps approaches infinity, the distribution of flow at each node converges \cite{langville2011google}.
This is called the stationary distribution, and this is the eigenvector corresponding to the eigenvalue of one discussed earlier \cite{langville2011google}. 
In fact, regardless of the initial distribution, the Markov chain will always converge to the stationary distribution \cite{langville2011google}. 
Aperiodic Markov chains have transition matrices that are primitive \cite{langville2011google}.

For periodic graphs, this is not the case. 
These have imprimitive transition matrices \cite{langville2011google}.
There is a stationary distribution (by the Perron-Frobenius Theorem), but it does not generally converge to the stationary distribution. 
This reveals some properties of $\T$ according to the Perron- Frobenius Theorem relating to imaginary eigenvalues.

\todo[inline]{Show that $\fv(\T)$ exists}

\todo[inline]{Show that $\forall \T,\ \fv(\T)\in\Fd$}

\todo[inline]{Show that $\{\fv(\T), \T\} = \Fd$}

\todo[inline]{Show that $T \rightarrow \fv(\T)$ is a convex function}

\subsubsection{Path flows}

Instead of link flows, we can choose to focus on path flows as well. We first define the path probabilities $\vec{\rho}$ as:
\begin{equation}
    \vec{\rho} := \left[[\mathbf{\tilde{T}_{ln}}M\Delta] ^\top \mathbbm{1}\right]_e
    = [\Delta^\top M^\top \mathbf{\tilde{T}_{ln}}^\top \mathbbm{1}]_e
\end{equation}

\[ \rho = [\Delta^\top diag(p)_{ln}^\top \mathbbm{1}]_e  \]

\todo[inline]{Try to show that $\mathbf{1}^\top \rho = 1$ when there is only one origin destination pair.}
\[ h = (\rho_p d)_p\]

. Let $\delta_k$ be row in the incidence matrix corresponding to link $k$, $P_j$ be the set of links in path $j$, and $\beta$ be number of paths:

\begin{equation}
\begin{split}
    \rho &= 
    \left[
    \begin{bmatrix}
        \delta_a^\top &\delta_b^\top &\dots &\delta_\epsilon^\top
    \end{bmatrix}
    \begin{bmatrix}
        ln(p_a)    &0       &\dots  &0\\
        0      &ln(p_b)     &       &\vdots\\
        \vdots &        &\ddots &0\\ 
        0      &\dots   &0      &ln(p_{\epsilon}) 
    \end{bmatrix}
    \begin{bmatrix}
        1 \\
        \vdots \\
        1
    \end{bmatrix}
    \right]_e \\
    &= \left[\begin{bmatrix}
        ln(p_a)\delta_a^\top &ln(p_b)\delta_b^\top &\dots &ln(p_\epsilon)\delta_\epsilon^\top
    \end{bmatrix}
    \begin{bmatrix}
        1 \\
        \vdots \\
        1
    \end{bmatrix}\right]_e \\
    &= \begin{bmatrix}
        ln(p_a)\delta_a^\top + ln(p_b)\delta_b^\top + \dots + ln(p_\epsilon)\delta_\epsilon^\top
    \end{bmatrix}_e \\
    &= \begin{bmatrix}
        \sum_{l \in P_1}ln(p_l) \\
        \vdots \\
        \sum_{l \in P_\beta}ln(p_l)
    \end{bmatrix}_e \\
    &= \begin{bmatrix}
        ln(\prod_{l \in P_1}p_l) \\
        \vdots \\
        ln(\prod_{l \in P_\beta}p_l)
    \end{bmatrix}_e \\
    &= \begin{bmatrix}
        e^{ln(\prod_{l \in P_1}p_l)} \\
        \vdots \\
        e^{ln(\prod_{l \in P_\beta}p_l)}
    \end{bmatrix} \\
    &= \begin{bmatrix}
        \prod_{l \in P_1}p_l \\
        \vdots \\
        \prod_{l \in P_\beta}p_l
        \end{bmatrix}
\end{split}
\end{equation}

For one origin-destination pair, we can show that $\mathbf{1}^\top \rho = 1$:

\begin{equation}
    \begin{split}
        \mathbf{1}^\top \vec{\rho} &=
        \begin{bmatrix}
            1 &\dots &1
        \end{bmatrix}
        \begin{bmatrix}
            \prod_{l \in P_1}p_l \\
            \vdots \\
            \prod_{l \in P_\beta}p_l
        \end{bmatrix} \\ 
        &= \sum_{j = 1}^\beta \prod_{l \in P_j}p_l 
    \end{split}
\end{equation}

\todo[inline]{If there is a cycle then $s_{od}=\infty$ (which is not well defined)}

We can prove that $\sum_{j = 1}^\beta \prod_{l \in P_j}p_l$ sums to 1 using strong induction. 
Let distance be defined as the max number of links between two nodes, and let $s_{od}$ be the distance between the origin to the destination.

\textbf{Base case:} When $s_{od}=1$, we know that there is only one link from the origin to the destination. 
Thus, there is one path and the probability of traveling on that path is 1.

\textbf{Inductive hypothesis:} Assume this is true for $s_{od} = k$.

\textbf{Induction step:} Let $s_{od} = k+1$, $n$ be the origin node, $n_1, \dots, n_m$ be the nodes that can be reached from the origin in one step, $p_1, \dots, p_m$ be the probabilities from the origin to the respective nodes, $\beta_1, \dots, \beta_m$ as the number of paths for the respective nodes to the destination, $\beta$ be the number of paths for the entire graph, and $P_{n_i d, j}$ be path $j$ from node $n_i$ to the destination.
We know that the distance from nodes $n_1, \dots, n_m$ to the destination is at most $k$ which we know $\sum_{j = 1}^{\beta_i} \prod_{l \in P_{n_i d, j}}p_l = 1$ is true for $1\leq i \leq m$ by the inductive hypothesis.
Thus, we can rewrite $\sum_{j = 1}^\beta \prod_{l \in P_{n d, j}}p_l$ as:
\begin{equation}
    \sum_{i=1}^m p_i  \sum_{j = 1}^{\beta_i} \prod_{l \in P_{n_i d, j}}p_l = \sum_{i=1}^m p_i = 1 
\end{equation}



%Suppose the above equation does not equal 1. Since the sum of path probabilities should be 1 since all commuters must be on one of those paths. 
%This means that there is at least one path that is not included in the summation above. 
%However, we sum over all paths, so this is a contradiction. Thus, $\sum_{j = 1}^\beta \prod_{l \in P_j}p_l$ = 1. 
We can define the path flows as 

\begin{equation}
    \vec{h}_p = d_{o,d}\vec{\rho}
\end{equation}

\subsection{STA Equilibrium}
Recall that at user equilibrium, no user can switch to a different route and reduce his or her travel cost \cite{perederieieva2013computational}.
The Wardrop condition of user equilibrium is formulated below \cite{patriksson}:

\begin{equation}
    \begin{split}
        h_{pqr} > 0 &\implies c_{pqr} = \pi_{pq} \quad \forall r \in \P_{pq} \\
        h_{pqr} = 0 &\implies c_{pqr} \geq \pi_{pq} \quad \forall r \in \P_{pq} 
    \end{split}
\end{equation}

However, to account for flow and demand, user equilibrium conditions can be modified \cite{patriksson}:

\begin{equation}
    \begin{split}
        h_{pqr}(c_{pqr} - \pi_{pq}) &= 0, \quad \forall r \in \P_{pq}, \; \forall (p, q) \in C \\
        c_{pqr} - \pi_{pq} &\geq 0, \quad \forall r \in \P_{pq}, \; \forall (p, q) \in C \\
        \sum_{r \in \P_{pq}} h_{pqr} &= d_{pq} \quad \forall (p, q) \in C \\
        h_{pqr} &\geq 0 \quad \forall r \in \P_{pq}, \; \forall (p, q) \in C \\
        \pi_{pq} &\geq 0 \quad \forall (p, q) \in C
    \end{split}
\end{equation}

The above set of equations can be formulated into the following optimization problem \cite{patriksson}:

\begin{equation}
\begin{split}
    \min \sum_{e\in \L}\int_0^{f_a}t_a(s) ds, \\ 
    \text{ subject to }  \quad \sum_{r \in \P} h_{pqr} &= d_{pq} \quad \forall (p,q) \in C \\
    h_{pqr} &\geq 0 \quad \forall r \in \P_{pq}, \forall (p,q) \in C \\
    \sum_{(p,q) \in C} \sum_{r \in \P_{pq}} \delta_{pqra} h_{pqr} &= f_a \quad \forall a \in \L
\end{split} 
\end{equation}

\subsection{Transition Equilibrium}

We know that $\vec{f}$ is the equilibrium flow such that $\vec{f} = L(\mathbf{P})^\top\vec{f} + diag(\vec{p})\mathbf{O}[\de-\de^\top]\mathbbm{1}$.
In fact, we proved that $\vec{f}$ exists by the Perron-Frobenius Theorem. 
This is equivalent to the optimization problem:

%\begin{equation}
%    \begin{split}
%    \min \| \vec{f} \|_2, \\ 
%    \text{such that} \quad \vec{f} &= L(\mathbf{P})^\top\vec{f} + diag(\vec{p})\mathbf{O}[\de-\de^\top]\mathbbm{1} \\
%    \mathbf{P} \mathbbm{1} &= \mathbbm{1} \\
%    d_{pq} &\geq 0 \quad \forall p, q \in \N \\
%    f_{pq} &\geq 0 \quad \forall p, q \in \N \\
%    \vec{f}^\top \mathbbm{1} &\geq \mathbbm{1}^\top \de \mathbbm{1} \\
%    \mathbbm{1}^\top \de \mathbbm{1} &> 0 \\
%    \text{no infinite loops}
%    \end{split}
%\end{equation}
\todo[inline]{infinite loops}

We can ensure that all entries in $\vec{f}$ are nonnegative because the null space of $I-L(\mathbf{P})^\top$ is nonnegative, so we can add a vector from the null space to satify the above conditions.

\subsection{Applications}
\subsubsection{Critical roads}
We can identify critical roads from the equilibrium flow vector, solely based on the magnitude of each entry.
Naturally, links with greater flow at equilibrium implies that they are busier roads in the long run.
Since working with Markov chains are a simplified representation of real-world networks, one can observe how closing a road or multiple roads (while mainly the strongly connected nature of the Markov chain) would affect the network fairly easily.
This could show the impact on travel time if a road were closed due to construction, an accident, or a similar event.

This is analogous to the concept of node criticality in graph theory which identifies certain roads as critical if removing it would increase average travel times in the network \cite{crisostomi2011google}.
This can be represented using Kemeny's constant $K$ which is, for the purpose of this article \cite{crisostomi2011google}:
\begin{equation}
    K = \sum_{j \in L(\N)} f_j t_{ij} \quad \forall i \in L(\N)
\end{equation}
where $t_{ij}$ is the mean first passage time form link $i$ to link $j$, and $f_j$ is the equilibrium flow on link $j$.
Notice that $K$ does not depend on $i$.
Comparing Kemeny's constant in the original network and after removing a road will show how critical that road is, as an increase in Kemeny's constant will imply that the road is critical to reducing average travel time \cite{crisostomi2011google}.
Likewise, a negative change implies that the existence of that road increases average travel time.
Such a scenario is known as Braess's Paradox, in which adding roads harms the network \cite{braess2005paradox}.
Indeed, the greater the change, the bigger the impact of the road on the network \cite{crisostomi2011google}.
Thus, this creates a measure of how well a network functions to improve existing networks and optimize future networks.


%Since $\vec{f} = \Delta \vec{h}$, $A\Delta d_{ab}\vec{\rho} = \vec{b}$ 


\subsubsection{Optimal Dynamic Flow Allocation Using SUMO}

\paragraph{Why Dynamic Traffic Assignment?}
\newline

Recognizing that traffic networks are generally not in the steady state, researchers have extended the notion of user equilibrium from Static Traffic Assignment (STA) in two ways\cite{TRB2011dta}: 
\begin{enumerate}
    \item It's required to develop efficient ways of describing time-varying network traffic conditions and finding route with shortest travel time considering that link travel time changes over time.
    \item It's required to establish new equilibrium for each departure time. 
\end{enumerate}
Compared with STA models, DTA models are able to capture more realistic traffic flow characteristics such as queue spillback, expansion waves and changing demand\cite{Szeto2006dynamic}. Moreover, the traditional travel forecasting models perform simulation on static regional traffic flow while microscopic traffic simulation models focus on dynamic corridor-level traffic analysis. DTA models' ability to model at a wide range of scales from corridor-level to regional-level actually fills the gap between travel forecasting model and microscopic traffic simulation mode\cite{TRB2011dta}. This can significantly improve the accuracy of traffic estimation. 

\newline


\paragraph{Optimization Framework for Dynamic Traffic Assignment}

For this article, we are considering a simulation-based DTA model using a traffic simulator to imitate the flow dynamics in urban road traffic system and to optimize certain objective functions. \cite{Peeta2001foundation}. A microscopic and open-source simulator SUMO is used to in a descriptive mode to simulate the traffic flow propagation and spatial-temporal interaction. SUMO is able to handle easy query and traffic control with Python API traci. 

In order to find the optimal objective function, we experimented with three reward function: 
\begin{enumerate}\label{rewards}
    \item maximizing the number of vehicles on outflow
    \begin{equation}\label{eq:reward1}
        r_{out} = \frac{f_D + 1}{f_A + 1}
    \end{equation}
    \item minimizing the sum of amount of vehicle weighted by average travel time of the edge
    \begin{equation}\label{eq:reward2}
        r_{sum} = \frac{\sum_{e \in E}{(f_e + 1)l_e/(v_e + 0.1 \cdot v_{e(max)})}}{\sum_{e \in E}{f_e + 1}}
    \end{equation}
    \item Minimizing the total travel time difference between any path and the path with shortest travel time.
    \begin{equation}\label{eq:reward3}
        r_{nas} = \frac{\sum_{e \in {upper, middle, lower}} {(f_e + 1) (t_e - t_{min})}}{\sum_{e \in {upper, middle, lower}} {f_e + 1}}
    \end{equation}
\end{enumerate}



\subsubsection{SUMO Setup}
The road network in figure \ref{fig:diamond_network} is simulated in SUMO and the data is collected from repeated simulation with different random seeds. The objective of using SUMO is to simulate the traffic states at different split ratios and to learn the optimal split ratio that maximizes the reward function. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{SUMO_setup.png}
    \caption{SUMO Setup}
    \label{fig:sumo_setup}
\end{figure}

In order to run simulation in SUMO, we need to perform the following setups, as demonstrated in figure  \ref{fig:sumo_setup}:
\begin{enumerate}
    \item Fixing the position of nodes and edges in desired network in figure \ref{fig:diamond_network}.
    \item Handling merge at \node[C] and \node[D] using buffer space with the help of \node[E] and \node[F] to prevent congestion from forming due to bottleneck capacity at merge. 
    \item Smoothing the two-lane buffer zone back to one lane for consistency with other lanes.
    \item At timestep i, iteratively generating a \Pod with \rhop of 0.5 starting from \node[Enter] and splitting at each node depending on transition matrix.
    \item Adding a vehicle to the network following route i.
\end{enumerate}




% \Fangyu{We experimented with three reward functions: (1) outflow, (2) weighted sum, and (3) Nash.
% \begin{align}
%     r_{out} &= \frac{f_D + 1}{f_A + 1}\\
%     r_{sum} &= \frac{\sum_{e \in E}{(f_e + 1)l_e/(v_e + 0.1 \cdot v_{e(max)})}}{\sum_{e \in E}{f_e + 1}} \\
%     r_{nas} &= \frac{\sum_{e \in {upper, middle, lower}} {(f_e + 1) (t_e - t_{min})}}{\sum_{e \in {upper, middle, lower}} {f_e + 1}}
% \end{align}}

\subsubsection{grid search Method}

As demonstrated in figure \ref{fig:diamond_network}, the example diagram only has two splits: at N\node[A] and N\node[B]. As each of the split is binary and the summation of split ratios at each intersection is 1, we only have two variables to be optimized: $P_{AB}$ and $P_{BC}$. Therefore, we attempted brute-force method first by experimenting all different combination of ($P_{AB}$, $P_{BC}$). The exhaustive search is also a good benchmark to be compared with the results using gradient descent method and random search. 

In order to understand the property of problems and check the efficacy of reward functions, we plot the heatmap of each reward distribution on meshgrid    of $P_{12}$ and $P_{23}$ with each axis incrementing from 0 to 1 at stepsize of 0.1. The figure in shown in fig \ref{fig:brute_force}.


\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{rewards_1000step_average.png}
    \caption{grid search Solution}
    \label{fig:brute_force}
\end{figure}

Each simulation is designed to be 1000 timesteps (500 seconds) and each column of fig\ref{fig:brute_force} shows the progression of heatmaps for each reward function throughout the simulation timestamped at [37.5s, 87.5s, 287.5s and 487.5s]. 



The plot for reward function 1 makes sense because in order to maximize the the exit flow,  we want to minimize congestion in every path. As illustrated in figure \ref{fig:sumo_setup}, there is a merge at \node[C]. When a vehicle is about to turn at certain radius, there is a speed reduction for all the cars in the area, which increases the path travel time. When the amount of vehicles from trying to merge at N\node[C] exceeds certain capacity, the speed reduction would result in spillbacks in AC or BC and therefore decrease the flow rate at exit. In consideration of the merge, when $\pr{12} >= 0.6$ and $\pr{23} <= 0.4$, the exist flow would be maximized. 
\subsubsection{Convex optimization methods}



\subsubsection{Optimal control methods}

\subsubsection{Reinforcement learning method}


\newpage
\bibliographystyle{trb}
\bibliography{trb_template}
